Analyzing the Evolution of Graphs and Texts

With the recent advance of representation learning algorithms on graphs (e.g., DeepWalk/GraphSage) and natural languages (e.g., Word2Vec/BERT) , the state-of-the art models can even achieve human-level performance over many downstream tasks, particularly for the task of node and sentence classification. However, most algorithms focus on large-scale models for static graphs and text corpus without considering the inherent dynamic characteristics or discovering the reasons behind the changes. This dissertation aims to efficiently model the dynamics in graphs (such as social networks and citation graphs) and understand the changes in texts (specifically news titles and personal biographies). To achieve this goal, we utilize the renowned Personalized PageRank algorithm to create effective dynamic network embeddings for evolving graphs. Our proposed approaches significantly improve the running time and accuracy for both detecting network abnormal intruders and discovering entity meaning shifts over large-scale dynamic graphs. For text changes, we analyze the post-publication changes in news titles to understand the intents behind the edits and discuss the potential impact of titles changes from information integrity perspective. Moreover, we investigate self-presented occupational identities in Twitter users' biographies over five years, investigating job prestige and demographics effects in how people disclose jobs, quantifying over-represented jobs and their transitions over time.

==> chapter2-DynAnom/cut-offs.tex <==
% general node/graph  monitoring

%(e.g., keeping track of suspicious nodes in a large social network, watching nodes of specific types in a massive heterogeneous graph)[\textcolor{red}{BJ: Examples could be put into intro.}].
% New problem: subset node monitoring 

% an instance of the application
% \footnote{For example, when analyze how \textit{Donald Trump} changes in Wikipedia hyperlink graph (about 6.4M nodes in total) over time, we are only interested in a subset of node $S = \{"\text{Donald-Trump}"\}$ and $|S|$ =1. We may want to avoid the computation of the other non-targeted nodes (places, food, events, ...) for efficiency purpose.}

% propose the problem

However, most of the computational time is used for small values as the iteration continues. In practice, those small values are less important than the large values (e.g., Top-k PPR values), thus neglected.



% To obtain dynamic embedding vectors, the general idea is to obtaindynamic PPVs and then project these PPVs into embedding spaceby using two kernel functions [30,42]. In this section, we presentour proposed methodDynamicPPEwhere it contains two maincomponents: 1) an adaptive precision strategy to control the esti-mation error of PPVs. We then prove that the time complexity ofthis dynamic strategy is still independent on��. With this qualityguarantee, learned PPVs will be used as proximity vectors and be"projected" into lower dimensional space based on ideas ofVerse[39] andInstantEmbedding[30]. We first show how can we get highquality PPVs and then present how use PPVs to obtain dynamicembeddings. Finally, we give the complexity analysis.

% \red{The proposed method should (or maybe) split into 3 parts. The first part is theoretical foundations of dynamic anomaly detection based on PPVs. Maybe give a chance to unify previous works. The second section is to analyze and present our proposed method. The third section is to analyze the theoretical guarantees w.r.t anomaly scores and qualities and also the run time complexity analysis. This part should finish as we argue the efficiency compared with previous methods.}


% \red{XZ: add a table talking about time complexity, and could the method handle individual anomaly tracking }
% \subsection{DynamicPPE} 
% \textcolor{red}{should we put it in method or related work} 

%\subsection{DynamicPPE with Weighted Push} Extend DynamicPPE with weighted adjacent matrix, and incremental push (with adjusted transition weights). We prove the incrementally PPR in Appendix \ref{appendix:unweighted-ppr-update}.

% \footnote{\url{https://www.aberdeennews.com/story/opinion/columns/2021/10/11/al-franken-makes-comeback-include-run-office/6053193001/}}

% Arnold Schwarzenegger:
% \begin{itemize}
%     \item In 2003, Arnold Schwarzenegger won the California gubernatorial election as his first politician role.
%     \item In 2008, Arnold began campaigning with McCain as the key endorsement for McCain's presidential campaign.  
%     \item In 2010, mid-term election.
%     \item After 2011, Arnold reached his term limit as Governor and returned to acting.
% % \end{itemize}

% Al Franken:
% \begin{itemize}
%     \item In 2002, Al Franken consider his first race for office due to the tragedy of Minnesota Sen. Paul Wellstone.\footnote{\url{https://www.aberdeennews.com/story/opinion/columns/2021/10/11/al-franken-makes-comeback-include-run-office/6053193001/}}
%     \item In 2004, The Al Franken Show aired.
%     \item In 2007, Al Franken announced for candidacy for Senate.
%     \item In 2008, Al Franken won election.
%     \item In 2012, Al Franken won re-election.
%     \item In 2018, Al Franken resigned.
% \end{itemize}

\clearpage


\xingzhiswallow{
\subsection{Issue with edge anomaly detection}
The edge anomaly detection algorithm assign anomaly score to each edge, however, it can not measure the node-level anomaly since if there is only a few edge associated with a node across snapshot, the node does not change in the snapshot without edges involving this node, regardless of its neighbors' evolution.
}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.

% \begin{acks}
% %add fundings

% \end{acks}

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.


% \red{we use max changes happen in top degree nodes $\pi_{\alpha}$ as grpah-level anomaly score}
% \paragraph{All-Tracking} Tracks all nodes once the node emerged in the graph.
% \paragraph{Top Node Tracking}: Incrementally add top-degree nodes into the tracking list from each snapshots. 

% \paragraph{Def-Tracking} Track the pre-defined nodes in the graph.

% \begin{algorithm}[ht]
% \caption{$\textsc{DynAnom}_{graph}(p_s^0, ... ,P_s^T)$}
% \begin{algorithmic}[1]
% \State $\delta_{\mathcal{G}} = \bm 0 \in \mathbb{R}^T$

% \State \textbf{return} $\bm W_s^t = [\bm w_s^1,\bm w_s^2,\ldots, \bm w_s^T], \forall s\in S$. 
% \end{algorithmic}
% \label{algo:dynanom-node}
% \end{algorithm}

% \paragraph{Active-Tracking} Tracks all nodes, but selectively update PPV based on the significant edge update, in terms of degree and $\Delta_{\{ p_s,r_s \}}$ changes.

%Focus on nodes, tracking the changes of a node across different snapshots and calculate the PPV changes.



% Given the node heterogeneity and size in the real-world graphs (), we may only interested 
% Such anomalies may constantly happen across different parts of graph, given that the real-world graphs are large-scale and fast-growing.  

% those methods may fail to monitor a subset nodes of interest (e.g., suspicious grey-list nodes). 

% but fail to further localize the specific anomalies nodes, or efficiently quantify the anomaly score of individually interesting nodes due to expensive re-training or fine-tuning.

% Additionally, given that the anomalies are constantly occurring, a global anomaly detector may always signify as positive, and becomes pointless unless it could localize where the anomalies actually happen. 
% Meanwhile, the scale and dynamics of graph also requires high efficiency. Thus, the following two important problems still remain unsolved : 
% 1). How to localize anomalous nodes in dynamic graphs?  
% 2). How to efficiently quantify the anomaly scores of individual nodes as the graph evolves? 

% In this paper, we propose a scalable and efficient PageRank-based anomaly detection algorithms over dynamic graphs. 
% In this paper, we propose an unifying algorithm to solve both aforementioned problems, which can effectively localize anomalies at the finest node level, and be capable of efficiently processing large dynamic graphs in an incremental fashion. 




% \textbf{1:} Coarse anomalous node candidates selection based on heuristics (e.g., the most active nodes in each time period). 
% \textbf{2:} Finer anomalous node selection based on the score derived from the highly efficient dynamic node embedding of time complexity ($\frac{\Delta m}{\epsilon \alpha}$), regardless of graph node size.   




%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.


% BJ: (e.g., grey-listed nodes), searched Google scholar, only one paper used this term.
% Monitoring a targeted subset of nodes (e.g., grey-listed nodes) in an evolving graph is critical for many real-world applications.



% We argue that the node-level anomaly could also capture the global anomaly given the fact that global anomaly could be decomposed to many node-level anomalies. Additionally, to describe the node in a graph, a well-known measure is Single-Source Personalized PageRank (SS-PPR). Following the recent advances in efficient local algorithms for SS-PPR in dynamic setting, we integrate SS-PPR for anomaly detection, and introduce in Section \ref{sec:ppr}.

% We believe that the graph-level anomaly consists of node and edge anomalies, reflecting the global properties, thus could be represented by finer-level anomalies.  
% In contrast, edge-level anomaly measures the fitness of two local nodes it connected with, but makes the scope too narrow and unavailable to the nodes without direct link. In other words, it may ignore the local community information when deciding if the edge-level anomaly occurs. 
% Node level as the intermediate, consisting the node-level community properties and fine-level local structure, could better capture the anomaly for both macro and micro anomalies. 



% In this paper, we restrict out attention on node-level anomaly detection and extend the node anomaly to graph anomaly.
%Therefore, focusing more on local perturbations, personalized PageRank is favored on the anomaly node identification.


\xingzhiswallow{
\sout{\red{Instead,} Node representation-based methods are the most satisfying approaches, but most of them \cite{perozzi2014deepwalk,grover2016node2vec,yu2018netwalk} may computationally suffer from large node size, \red{e.g., the size of our motivating example}, and waste computations on the nodes falling out of the target subset. In our example where we have million-scale graph over thousands of snapshots, those methods may fail to finish.}
}

 %, causing extra overhead for re-alignment (e.g., $\mathcal{O}(n^3 T) $ for Procrustes analysis \cite{gower1975generalized, wang2008manifold}, $T$ is the number of snapshots and $n$ is the number of nodes). 

%\cite{tsitsulin2021frede}
% recent local methods could save 
% but anomaly for local methods was not explored.
% our paper extend local method to weighted graph and explore the anomaly 

% \item \textcolor{red}{Copied from abstract: Our three major contributions are:
% \textit{ \textbf{1.}} A more applicable efficient local node representation based on incremental PPVs over evolving graphs, whose per-node time complexity is bounded by edge events ($\Delta m$) and error parameter($\epsilon$) regardless of graph node size.  \textit{ \textbf{2.}} An unified framework for both node-level anomaly localization and global snapshot-level anomaly detection with theoretical guarantees.
% \textit{ \textbf{3.}} Analysis on two new, large, real-world dynamic graphs of people and countries across 30 years. With the scarcity of annotated-\textit{anomaly} graphs, these resources provide fresh opportunities for human-interpretable anomaly detection in graph mining community.}


%2. The are all sudden changes from original patterns, either in global or local resolution, and we define the anomaly as the sudden changes in feature space.\\

% 3.1 How to construct features?  PageRank as global graph-level features. Node embeddings as local node-level features.  \\

% 3.2 How to efficiently construct features for evolving graphs?  \\

% 3.2.1. Embedding Space consistency\\

% 3.2.2. Algorithm Efficiency \\

% 4. How to define anomaly over feature space? \\

% 4.1 $l_1$ distance, \\

% 4.2 Derivatives of changes.\\

% 4.3 Difference in clustering.\\



% Many real-world networks (e.g., online transaction, social network interaction) are large-scale and evolving at a fast pace, involving nodes and edges being added or deleted.
%Monitoring anomalies over a fast-growing graph is critical to detect online transaction fraud, social spam, malware, etc. 

% static graph
%In a static graph consisting of a fix number of vertices and edges, graph-level anomaly considers the global properties of graph, and measure the deviation of the selected properties against the \textit{norm}, which are observed from the other instances in the same graph-family. For example, the power-law node degree distribution, betweenness, etc.

% \citet{beutel2013copycatch} 
%We notices that many PageRank-based methods \cite{yoon2019fast} were developed. 


%It neither has ability to track changes of suspicious nodes, nor to determine which edges are unwelcome.  
% In practice, the local subtle anomalies may constantly occur (e.g., online frauds are always going on in a large transaction network), spotting local anomalies is critically useful to inspect and understand the problem, instead of flagging the whole snapshot as anomaly.  
% From theoretical perspective, \citet{lee2003perturbation} suggests that the global PageRank is rather stable w.r.t. the edge perturbation, so the global PageRank may not be sensitive to the local malicious changes, resulting in many false negative.
%\todo{We may need to highlight local (subtle) changes are important if our assumption is true.}

%Many streaming based methods \cite{chang2021f,eswaran2018sedanspot} were proposed. 
%Many edge streaming anomaly detection algorithms \cite{bhatia2020midas, eswaran2018spotlight} were proposed.


%thus unable to monitor the node status change resulted from the community evolution as the Trump-Melania example shows.

% Similarly, edge-level anomaly detection identifies the unexpected edges. The fitness of an existing edge could be determined by the node properties (either node embeddings or hand-crafted features) of the nodes on the edge's endpoints. 

% node anomaly 
% Node-level anomaly detection is equivalent to identify the outliers w.r.t. node properties, that is - the nodes belonging to neither community or those of unexpected high degrees \textcolor{red}{CITE}. The definition of anomaly is hueristic and application-dependant, the most recent works use powerful network embeddings as the node representation for outlier detection. 


%Compare to the global anomaly, local changes are more subtle, thus it might not be significant enough to affect global graph property.


%For example, we may want to quantify the anomaly of a single persons in a million-scale dynamic graph. A straightforward pruning of irrelevant nodes from the graph may remove useful network structure information and dramatically change the graph topology. 
%And calculating all node embeddings across times then extract the node subset may less computationally-budgeted, even becomes impractical if the graph size is large (millions of nodes) and time horizon is long (thousands of snapshots). Therefore, an efficient subset node representation over large dynamic graph is critical.


% \red{not scalable} 
%However, since there is no embedding space alignment across time, the outliers can be only identified within each snapshot, which is more like a static node anomaly detection. Moreover, This method is inapplicable to large graph with upcoming new nodes because the used AutoEncoder  is not scalable and expandable. % \red{not scalable} 

%Likewise, JODIE \cite{kumar2019predicting} leverages Recurrent Neural Networks (RNNs) to model the node embedding trajectories changes as the graph evolves. 
%This model aims to predict the future node embeddings based on the previous interaction history, and model the node state based on the learnt latent representation.

% shortcomings of above methods
% However, considering the large-scale and fast-grow property of real-world graph, efficiently updating node representation becomes the bottleneck. 
% Moreover, in order to compare the node representation across different time, it needs a consistent embedding space alignment, which imposes extra overhead when calculating the node-level anomaly score. 
% Most importantly, the above methods are not good fit for the task of \textit{Local node-level anomaly by queried nodes} where we only care about a subset nodes of interest, as described in Definition \ref{def:node-track-def}. 
% For example, we may want to quantify the anomaly of persons in a heterogeneous graph containing the interactions both people, events, locations, etc. 
% A straightforward pruning of irrelevant nodes from the graph may remove useful network structure information and dramatically change the graph topology. 
% And calculating all node embeddings across times then extract the node subset may less computationally-budgeted, even becomes impractical if the graph size is large (millions of nodes) and time horizon is long (thousands of snapshots). Therefore, an efficient subset node representation over large dynamic graph is critical.

%Single-Source Personalized PageRank (SS-PPR) \cite{page1999pagerank}, could be leveraged for node representation. 
%for Single-Source Personalized PageRank (SS-PPR)

% We generalize the PPV approximation for incorporating node interaction frequency, which will be detailed in Section \ref{sec:notation-prelim} and Section \ref{sec:ppr}. We summarize the properties of algorithms in Table \ref{tab:algo-comparison}.






% \begin{table}[ht]
% \caption{The comparison of supported features between DynAnom and other methods.}
% \centering
% \begin{tabular}{p{0.15\textwidth}|rrrr|r}
% \toprule
%   \diaghead{\hskip 25mm }%
% {Feature}{Method} & \rotatebox[origin=c]{75}{SedanSpot\cite{eswaran2018sedanspot}} & \rotatebox[origin=c]{75}{AnomRank\cite{yoon2019fast}} & \rotatebox[origin=c]{75}{NetWalk\cite{yu2018netwalk}}  & \rotatebox[origin=c]{75}{DynPPE\cite{xingzhi2021subset}}  & \rotatebox[origin=c]{75}{\textbf{DynAnom}}  \\
% \midrule 
% Node-level Rep. &  \redxmark &  \redxmark & \bluecheck  & \bluecheck  & \bluecheck  \\
% Node Tracking &  \redxmark &  \redxmark &  \redxmark &  \bluecheck &  \bluecheck \\
% Multi-Edge & \bluecheck &  \bluecheck&  \bluecheck &  \redxmark&  \bluecheck\\
% Edge Add/Delete & \redxmark  & \bluecheck & \redxmark & \bluecheck &  \bluecheck \\
% Edge-stream & \bluecheck & \bluecheck & \redxmark  &  \bluecheck&  \bluecheck\\
% Score function-based & \bluecheck & \bluecheck & \bluecheck  &  \redxmark &  \bluecheck\\
% \bottomrule
% \end{tabular}
% \label{tab:algo-comparison}
% \end{table}

\xingzhiswallow{
\subsubsection{Selective Lazy Push}
Since our goal is to signify the changes in node status by comparing the PPVs before and after edge events, we may want to skip the edges causing minor PPV changes until it accumulates to invoke the push subroutine.

\red{[BJ: The following theorem should be move to preliminary part. Or we can present here as a generalized version.]}

\begin{theorem} \cite{lee2003perturbation} The bounds on difference between the old PPR vector  $\pi^{t-1}$ and new PPR vector $\pi^t $ is :
\begin{equation}
    || \pi_s^{t-1} -  \pi_s^t  ||_1 \leq \frac{2(1-\alpha)}{\alpha} \sum_ {i \in U} \pi_s^{t-1}(i), 
\end{equation}
 $U$ is the set of the updated nodes. The proof is in \cite{lee2003perturbation}.
 \label{theorem:alpha-bound-ppr}
\end{theorem}

From theorem \ref{theorem:alpha-bound-ppr}, we observe that a larger $\alpha$ (more chance to restart/teleport from/to the source node) would make smaller changes in PPR. 
If a node $v_i$ with large $\pi^{t-1}_i$ involved in edge changes, then, the upper bound also increases, leading to significant difference in the updated $\pi^{t}$.
It gives us a clue of when to actually need update PPR. In order to save time, we derived a selective lazy push procedure.

}

The most commonly used method is \textit{Power Iteration} \cite{page1999pagerank}, which approximates $\bm \pi_{s}$ iteratively:
\begin{align}
\bm \pi_{s}^{(t)} &= (1-\alpha)  \bm P^\top \bm \pi_{s}^{(t-1)} + \alpha \bm 1_s \textbf{ // Power Iteration}  \allowdisplaybreaks \nonumber\\
% &= (1-\alpha)^{t}  (\bm P^\top)^{t} \bm \pi_{s}^{(0)} + \alpha \sum_{i = 0}^{t-1}(1-\alpha)^{i} (\bm P^\top)^{i}\bm 1_s \nonumber  \allowdisplaybreaks\\
&= \alpha \bm 1_s \sum_{i = 0}^{t-1}(1-\alpha)^{i} (\bm P^\top)^{i} \text{ // assuming that }  \bm \pi_{s}^{(0)} = \bm 0.  \allowdisplaybreaks \label{eq:ppr-2} 
\end{align}


% The root reason of OOM is that the parameter size of NetWalk's AutoEncoder is related to $|\mathcal{V}|$ due to the 

% . Specifically, due to the reconstruction loss function in AE, the length of input/output one-hot vector is $|\mathcal{V}|$, making it computationally prohibitive when dealing with massive graph of large node set.  



% \textbf{DynPPE}, considering to be the unweighted version of \textbf{DynAnom} is always worse than its weighted counterpart. 





% \red{overall time complexity analysis here}


% \subsection{Node Vector Dynamically Maintenance} Instead of using the most up-to-date PPV for every update, we can maintain a temporal vectors with partially dimensions being updated every time.





%\subsection{Score functions ?}

% \subsection{Overall Proposed algorithm}
% \red{In the specific presentation style, union all these algorithms into one algorithm so that the proposed method looks novel and beauty.}

%We introduce the dataset, baseline methods, and experiment settings as following.


\xingzhiswallow{
\paragraph{Country Knowledge Graph (COUNTRY)}: We construct this country-level interaction graph from GDelta Project\cite{leetaru2013gdelt} \footnote{GDelta Homepage: \url{https://www.gdeltproject.org/}}. Each node is a country entity.
Each edge represent a inter-country \textit{conflict} interaction with Goldstein score \cite{goldstein1992conflict} smaller than -7.0\footnote{ Goldstein score ranges from -10.0 to 8.3,  measuring the intensity of conflict(negative) or cooperation(positive) inherent in different types of international events: e.g., -10.0: Military attack; -7.0: Threat with force specified; -3.0: Give warning, etc.}. Similarly, we study when did the countries shift foreign conflict focus as the global tension develop.  

}

%and use cluster-based measure to detect node-level anomaly. 
%However, in the original paper, the definition of anomaly is the edges that are not in the graph, making the task more similar to link prediction instead of anomaly detection.



%Its core PPV calculation module is equivalent to our proposed 

% \textcolor{red}{NetWalk does not finish in 10 hours.}


% \paragraph{F-Fade\cite{chang2021f}} factorizes the frequency of nodes-wise interactions in a edge stream, and use the likelihood of the observed interaction frequency as the anomaly score.

%shows one application using our proposed algorithm \textsc{DynAnom} over the Person-EventKG (3.1 million nodes and 6.7 million edges).

Note that the complexity is independent of the total node size. 

% \item Two large-scale real-world graphs for node level tracking: Person-EventKG and Country-EventKG are constructed as more human-interpretable resources for graph anomaly detection community. It brings more research opportunities for both algorithm benchmarking and data science discovery.  


\xingzhiswallow{
\subsection{Proof of PPV maintenance}
\label{sec:appendix-ppv-adjust-proof}
\begin{proof}
This proof follows the paradigm used in \cite{zhang2016approximate}. We start from the invariant property in Lemma \ref{lemma:ppr-invar}:
\begin{align}
p_s(i) + \alpha r_s(i) = (1-\alpha)\sum_{x \in N^{in}(i)}  \frac{ w_{(x,i)} p_s(x)}{d(x)} + \alpha \times 1_{t=s}, \forall i \in \mathcal{V}  
\end{align}

% Initially, this invariant holds and keeps $ \frac{r_s(i)}{d(i)} \leq \epsilon$ after applying Algo.\ref{algo:forward-local-push-weighted}. 
% When the new edge $(u,v,\Delta w_{(u,v)})$ arrives, it changes the out-degree of $u$, breaking up the balance for all invariant involving $d(u)$. Our goal is to recover such invariant by adjusting small amount of $p_s, r_s$. While such adjustments may compromise the quality of PPVs, we could incrementally invoke Algo.\ref{algo:forward-local-push-weighted} to update $p_s$ and $r_s$ for better accuracy afterwards. We denote the initial vectors as $p_s, r_s, d$ and post-change vectors as $p'_s, r'_s, d'$. 
When the new edge $(u,v,\Delta w_{(u,v)})$ arrives, we denote the initial vectors as $p_s, r_s, d$ and post-change vectors as $p'_s, r'_s, d'$. 

\paragraph{Update $p_s(u)$:}
% First, since $d'(u)$ is involved in $\frac{p_s(u)}{d'(u)}$, we should find an updated $p'_s(u)$ so that  $\frac{p_s(u)}{d(u)} = \frac{p'_s(u)}{d'(u)}$, which makes the invariants still hold for any $p_s(i)$ containing $\frac{p_s(u)}{d}$ in Eq.\ref{eq:u-invaraint-body}:
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \nonumber\\
    %p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\nonumber\\
    p'_s(u) &= (d(u)+\Delta w_{(u,v)}) \frac{p_s(u)}{d(u)},\nonumber\\
            &= p_s(u) \frac{d(u)+\Delta w_{(u,v)}}{d(u)}, 
\end{align}

% Eq. \ref{eq:p-update-weighted-body-2} implies that we should scale up $p_s(u)$ to recover balance. This strategy is the general case of \citet{zhang2016approximate} for unweighted graphs where $\Delta w_{(u,v)} = 1$.

\paragraph{Update $r_s(u)$:} However, once we assign $p'_s(u)$, it breaks the invariant for $u$ since $p_s(u)+\alpha r_s(u) \neq p'_s(u)+\alpha r_s(u)$. Likewise, we maintain this equality by introducing $r'_s(u)$:
\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) \nonumber\\
    % &= \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \text{  from eq. \ref{eq:u-invaraint-body}} \\
    &\text{Substitute $p'_s(u)$ from eq.\ref{eq:p-update-weighted-body}} \nonumber \allowdisplaybreaks\\
    % & = p_s(u)\frac{d(u)+\Delta w_{(u,v)}}{d(u)} + \alpha r_s'(u) ,\nonumber\\
    & = p_s(u) + \frac{\Delta w_{(u,v)} p_s(u)}{d(u)} + \alpha r_s'(u) , \nonumber \allowdisplaybreaks \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{\Delta w_{(u,v)} p_s(u)}{d(u)},\nonumber \allowdisplaybreaks\\
    % \alpha r_s'(u)  &= \alpha r_s(u) -\frac{\Delta w_{(u,v)} p_s(u)}{d(u)},\nonumber\\
    r_s'(u) &=  r_s(u) -\frac{\Delta w_{(u,v)} p_s(u)}{\alpha d(u)} 
\end{align}

% Eq. \ref{eq:r-update-weighted-body-2} implies that we should decrease $r_s(u)$. From a heuristic perspective, it's consistent to the behavior of BCA-algorithm which keeps taking mass from $r_s$ to $p_s$. In this updating case, we artificially create mass for $p'_s$ at the expense of $r_s$'s decrements. When $\Delta w_{(u,v)} = 1$ in case of unweighted graphs, this update rule is also equivalent to \citet{zhang2016approximate}.

% So far, we have the updated $p'_s(u)$ and $r'_s(u)$ so that all nodes (without direct edge update, except for $v$) keep the invariant hold. However, due to the introduction of $\Delta w_{(u,v)}$, the shares of mass pushed to $v$ is changes, breaking the invariant for $v$ as shown below:
% \paragraph{Update $r_s(v)$}
% \begin{align}
%     p_s(v) + \alpha r_s(v) & \neq (1-\alpha) \Bigl( \frac{ (w_{(u,v)} + \Delta w_{(u,v)})  p'_s(u)}{d'(u)} \Bigr. \nonumber\\
%     & \Bigl. + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{w_{(u,x)} p_s(x)}{d(x)} \Bigr) +\alpha \times \mathbbm{1}_{t=s} \nonumber
% \end{align}

% In order to recover the balance with minimal effort, we should update $r_s(v)$ instead of $p_s(v)$. The main reason is that any change in $p_s(v)$ will break the balance for $v$'s neighbors, similar to the breaks incurred by the change of $p_s(u)$. 
\paragraph{Update $r_s(v)$:} We present the updated $r'_s(v) = r_s(v)+\Delta $:
\begin{align}
p_s(v) + \alpha \Bigl(r_s(v)+\Delta \Bigr) &= (1-\alpha) \Bigl( \frac{\Delta w_{(u,v)} p'_s(u)}{d'(u)} + \Bigr. \nonumber\\
&\Bigl. \sum_{x \in N^{in}(v) }  \frac{w_{(u,x)} p_s(x)}{d(x)} \Bigr) +\alpha \times 1_{t=s}   \\
\text{Note that } \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \text{ and}  \nonumber \\
p_s(v) + \alpha r_s(v) &= (1-\alpha)\sum_{x \in N^{in}(v)}  \frac{ w_{(x,v)} p_s(x)}{d(x)} \nonumber  \allowdisplaybreaks \\
&\hspace{-25mm}\text{Reorganize Eq. \ref{eq:invar-v-body} and cancel out $p_s(v), r_s(v)$, we have: } \nonumber \allowdisplaybreaks\\
\Longrightarrow \alpha \Delta &= (1-\alpha) \frac{ \Delta_{w_{(u,v)}} p'_s(u)}{d'(u)} \nonumber \allowdisplaybreaks\\
\Delta &= \frac{(1-\alpha)}{\alpha} \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)} \nonumber \allowdisplaybreaks\\
\text{Recall that } r_s'(v) &=  r_s(v) + \Delta \nonumber\\
&= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{\Delta_{w_{(u,v)}}p_s(u)}{d(u)}
\end{align}
We conclude the proof of Theorem \ref{theorem:dyn-adjust-weighted-graph}.

\end{proof}

}


\xingzhiswallow{
\begin{table}[h!]
    \centering
    \tiny
\begin{tabular}{p{0.1\linewidth} p{0.77\linewidth}}
\toprule
 Marker & Major Conflict Event \\
\midrule 
 \multicolumn{2}{c}{CHN (China)} \\
\midrule 
 CHN-1993 & Criticized the establishment of British Trade and Cultural Office in Taipei City. \\
 CHN-1999 & Belgrade Embassy Bombing: Chinese demonstrators protest throughout the country, attacking official U.S. property \\
 CHN-2008 & China-France over Tibetan sovereignty debate. Sudan violence against Chinese workers \\
 CHN-2009 & China-Australian over Tibetan sovereignty debate \\
 CHN-2010 & China-Japan Senkaku/Diaoyu Island Disputes \\
 CHN-2011 & China-Philippines-Vietnam South China Sea Territorial Disputes \\
 CHN-2014 & Severe Violence against Chinese in Vietnam over South China Sea  Disputes \\
 CHN-2016 & Taiwan-Strait tension. China-Philippines South China Sea Arbitration  \\
\midrule 
 \multicolumn{2}{c}{USA (U.S.)} \\
\midrule 
 USA-1994 & Battle of Mogadishu in Somalia (Black Hawk Down) \\
 USA-1998 & Operation Desert Fox in Iraq \\
 USA-1999 & Kosovo War \\
 USA-2001 & War in Afghanistan since 9-11  \\
 USA-2003 & Iraq War \\
 USA-2006 & Iraq (civil) War intensified \\
 USA-2008 & Pakistan–U.S. skirmishes \\
 USA-2011 & Military intervention in Libya \\
 USA-2016 & Syria Civil War (ISIS)  \\
 \bottomrule
\end{tabular}
    \caption{The global conflict events in China and the U.S.}
    \label{tab:country-events}
\end{table}
}


\xingzhiswallow{
\subsection{Static PPR for unweighted graph}
Given a weighted, but undirected graph $\mathcal{G} = <V,E> ,\{ (v_i, v_j, w_{(i,j)}) \in E, \forall i,j \in V )\}$, a vector $p^\alpha_s(u)$ to approximate the Personalized PageRank $\pi^\alpha_s(u)$ with dampling factor $\alpha$. We elided the constant $\alpha$ for clear notation.  

The recursive and linear definition of PPR tells us:
\begin{align}
    \overrightarrow {\pi}_{\alpha, s} &= \overrightarrow{v_s} \alpha  \sum_{i = 0}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \overrightarrow{v_s} \alpha ( I  + \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i})\\
            &= \overrightarrow{v_s}  \alpha I  + \overrightarrow{v_s} \alpha \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i},\\
    R_\alpha &= \alpha  \sum_{i = 0}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \alpha I + \alpha \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \alpha I + (1-\alpha) \bm P R_\alpha \\
    \overrightarrow {\pi}_{\alpha, s} &= \overrightarrow{v_s}  R_\alpha \\
            &=  \overrightarrow{v_s}  \alpha I  + \overrightarrow{v_s}  (1-\alpha) \bm P R_\alpha \\
            &=  \alpha \overrightarrow{v_s} + (1-\alpha)  \overrightarrow{v_s} \bm P R_\alpha \\
            &=  \alpha \overrightarrow{v_s} + (1-\alpha) \overrightarrow{\pi}_{(\alpha, v_s \bm P)},\\
            &=  \alpha \overrightarrow{v_s} + \overrightarrow{\pi}_{(\alpha, (1-\alpha) v_s \bm P)},\\            
\end{align}


Assign initial $v_s = \bm 1_s$, Eq.\ref{eq:ppv-reursion-recursive} gives the recursive formulation of PPR calculation. Starting from putting $\alpha v_s$ mass into $\pi(s)$, then propagation $(1-\alpha) v_s$ via the network ($ \bm P$) as the input $v_s$ for the next level nodes. The forward push algorithm essentially repeat the above process until there is no significant $v_s$ to be propagate.

The algorithm works for both un/directed or un/weighted graph, based on how to formulate $\bm P$. 


\begin{algorithm}[H]
\caption{$\textsc{ForwardPush}$ \cite{zhang2016approximate}}
\begin{algorithmic}[1]
\State \textbf{Input: }$\bm p_s, \bm r_s, \mathcal{G}, \epsilon, \beta = 0$
\While{$\exists u, r_s(u) > \epsilon d(u)$}
\State $\textsc{Push}(u)$
\EndWhile
\While{$\exists u, r_s(u) < -\epsilon d(u)$} 
\State $\textsc{Push}(u)$
\EndWhile
\State \Return $(\bm p_s, \bm r_s)$
\Procedure{Push}{$u$}
\State $p_s(u) \pluseq \alpha r_s(u)$
\For{$v \in \operatorname{Nei}(u)$}
\State $r_s(v) \pluseq (1-\alpha) r_s(u) (1-\beta) / d(u)$
\EndFor
\State $r_s(u) = (1-\alpha) r_s(u) \beta $
\EndProcedure
\end{algorithmic}
\label{algo:forward-local-push}
\end{algorithm}

\subsection{Dynamic PPR via Forward Push}
\label{appendix:dyn-ppr-push}
Similar to the formulation above, but we add an edge insertion or deletion.  Suppose at time $t+1$we insert an single new edge $(v_u, v_v, w_(u,v))$ to the graph $\bm G^{(t)}$, how to update the parameters?


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt   
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[x=0.4pt,y=0.4pt,yscale=-1,xscale=1]
    %uncomment if require: \path (0,276); %set diagram left start at 0, and has height of 276
    
    
    %Shape: Circle [id:dp6177377526862062] 
    \draw   (246,98) .. controls (246,85.85) and (255.85,76) .. (268,76) .. controls (280.15,76) and (290,85.85) .. (290,98) .. controls (290,110.15) and (280.15,120) .. (268,120) .. controls (255.85,120) and (246,110.15) .. (246,98) -- cycle ;
    %Shape: Circle [id:dp1784403270352245] 
    \draw   (403,93) .. controls (403,80.85) and (412.85,71) .. (425,71) .. controls (437.15,71) and (447,80.85) .. (447,93) .. controls (447,105.15) and (437.15,115) .. (425,115) .. controls (412.85,115) and (403,105.15) .. (403,93) -- cycle ;
    %Shape: Circle [id:dp6416110255517944] 
    \draw   (347,216) .. controls (347,203.85) and (356.85,194) .. (369,194) .. controls (381.15,194) and (391,203.85) .. (391,216) .. controls (391,228.15) and (381.15,238) .. (369,238) .. controls (356.85,238) and (347,228.15) .. (347,216) -- cycle ;
    %Shape: Circle [id:dp3486444110500183] 
    \draw   (240,233) .. controls (240,220.85) and (249.85,211) .. (262,211) .. controls (274.15,211) and (284,220.85) .. (284,233) .. controls (284,245.15) and (274.15,255) .. (262,255) .. controls (249.85,255) and (240,245.15) .. (240,233) -- cycle ;
    %Shape: Circle [id:dp8249186864870216] 
    \draw   (100,177) .. controls (100,164.85) and (109.85,155) .. (122,155) .. controls (134.15,155) and (144,164.85) .. (144,177) .. controls (144,189.15) and (134.15,199) .. (122,199) .. controls (109.85,199) and (100,189.15) .. (100,177) -- cycle ;
    %Shape: Circle [id:dp9360878049566426] 
    \draw   (85,90) .. controls (85,77.85) and (94.85,68) .. (107,68) .. controls (119.15,68) and (129,77.85) .. (129,90) .. controls (129,102.15) and (119.15,112) .. (107,112) .. controls (94.85,112) and (85,102.15) .. (85,90) -- cycle ;
    %Shape: Circle [id:dp7730088104243199] 
    \draw   (174,32) .. controls (174,19.85) and (183.85,10) .. (196,10) .. controls (208.15,10) and (218,19.85) .. (218,32) .. controls (218,44.15) and (208.15,54) .. (196,54) .. controls (183.85,54) and (174,44.15) .. (174,32) -- cycle ;
    %Straight Lines [id:da933198006075885] 
    \draw    (129,90) -- (244,97.86) ;
    \draw [shift={(246,98)}, rotate = 183.91] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da896601842938809] 
    \draw    (141,167) -- (252.18,116.82) ;
    \draw [shift={(254,116)}, rotate = 155.71] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da20344875896867154] 
    \draw    (218,46) -- (253.53,78.65) ;
    \draw [shift={(255,80)}, rotate = 222.58] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6413353007566629] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=3.75]    (290,98) -- (396,98.95) ;
    \draw [shift={(402,99)}, rotate = 180.51] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=3.75]    (35.19,-10.59) .. controls (22.38,-4.5) and (10.65,-0.97) .. (0,0) .. controls (10.65,0.97) and (22.38,4.5) .. (35.19,10.59)   ;
    %Straight Lines [id:da16852402207129602] 
    \draw    (268,120) -- (262.13,209) ;
    \draw [shift={(262,211)}, rotate = 273.77] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6238574957309465] 
    \draw    (287,111) -- (350.86,203.35) ;
    \draw [shift={(352,205)}, rotate = 235.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    
    % Text Node
    \draw (262,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {u};
    % Text Node
    \draw (418,84) node [anchor=north west][inner sep=0.75pt]   [align=left] {v};
    % Text Node
    \draw (257,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {j};
    % Text Node
    \draw (363,211) node [anchor=north west][inner sep=0.75pt]   [align=left] {k};
    
    \end{tikzpicture}
    \caption{The new edge (u,v)}
    \label{fig:new-edge-example-appendix}
\end{figure}

The $p^t_s,r^t_s$ estimation has been converged to the true PPR. The addition of the edge may break the balance, specifically for :

\begin{align}
    p_s(u) + \alpha r_s(u) = (1-\alpha)\sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \label{eq:u-invaraint} \\
    p_s(k) + \alpha r_s(k) = (1-\alpha)\sum_{x \in N^{in}(k)}  \frac{p_s(x)}{d(x)}, \\
    p_s(j) + \alpha r_s(j) = (1-\alpha)\sum_{x \in N^{in}(j)}  \frac{p_s(x)}{d(x)}, \\
    p_s(v) + \alpha r_s(v) = (1-\alpha)\sum_{x \in N^{in}(v)}  \frac{p_s(x)}{d(x)},
\end{align}


Where any equation evolve degree of node u break up (for node $j, k, v$). In order to fix the imbalance, we should adjust estimation $p_s, r_s$ at the expense of PPR value. 

We denote the updated degree is $d'(u)$ and $p'_s(u)$, for any node-u involved calculation, we want to make the value does not change, specifically :
\paragraph{Update $p_s(u)$}
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \\
    p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\\
            &= (d(u)+1) \frac{p_s(u)}{d(u)},\\
            &= p_s(u) \frac{d(u)+1}{d(u)}, \label{eq:p-update}
\end{align}

Eq.\ref{eq:p-update} shows that we could scale $p_s(u)$ by a factor of $\frac{d(u)}{d(u)+1}$, but this adjustment for neighbors of node u further breaks up the invaraiant of node u itself in Eq. \ref{eq:u-invaraint}, thus we should adjust $r_s(u)$ to rebalance but increase the error of ppv.
\paragraph{Update $r_s(u)$}

\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) = \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \\
    & = p_s(u)\frac{d(u)+1}{d(u)} + \alpha r_s'(u) ,\\
    & = p_s(u) + \frac{p_s(u)}{d(u)} + \alpha r_s'(u) ,  \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{p_s(u)}{d(u)},\\
    \alpha r_s'(u)  &= \alpha r_s(u) -\frac{p_s(u)}{d(u)},\\
    r_s'(u) &=  r_s(u) -\frac{p_s(u)}{\alpha d(u)},
\end{align}

\paragraph{Update $r_s(v)$}
\begin{align}
    p_s(v) + \alpha r_s(v) & = p_s(v) + \alpha (r_s(v)+\Delta) \\
    &= (1-\alpha) \left( \frac{p_s(u)}{d(u)} + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{p_s(x)}{d(x)} \right) \\
    \Longrightarrow \alpha \Delta &= (1-\alpha) \frac{p_s(u)}{d(u)}\\
    \Delta &= \frac{(1-\alpha)}{\alpha} \frac{p_s(u)}{d(u)}\\
    \Longrightarrow r_s'(v) &=  r_s(v) + \Delta \\
    &= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{p_s(u)}{d(u)}
\end{align}

\subsection{Extend unweighted Dynamic PPR to weighted graph}
\label{appendix:unweighted-ppr-update} %\label{appendix:dyn-ppr-push}

We extend the dynamic adjust to weighted graph.  In Figure \ref{fig:new-edge-example}, we add new edge $(u,v,w_{(u,v)})$ to the weighted-graph \footnote{weighted-graph: $D(u) = \sum_{i \in N(u)} w_{(u,i)}$}. Similar to the analysis of invariant properties for unweighted graph, we found that the insertion of edges breaks the balance of node $j,k,v$, since the node degree of $u$ is has been changed. To compensate the new edges (weights),  first, we adjust $p_s(u), r_s{u}$ to keep invariant of out-neighbors (node j,k).

Update of $p_s(u):$
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \\
    p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\\
            &= (d(u)+w_{(u,v)}) \frac{p_s(u)}{d(u)},\\
            &= p_s(u) \frac{d(u)+w_{(u,v)}}{d(u)}, \label{eq:p-update-weighted}
\end{align}

Update of $r_s(u):$
\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) = \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \\
    & = p_s(u)\frac{d(u)+w_{(u,v)}}{d(u)} + \alpha r_s'(u) ,\\
    & = p_s(u) + \frac{w_{(u,v)} p_s(u)}{d(u)} + \alpha r_s'(u) , \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{w_{(u,v)} p_s(u)}{d(u)},\\
    \alpha r_s'(u)  &= \alpha r_s(u) -\frac{w_{(u,v)} p_s(u)}{d(u)},\\
    r_s'(u) &=  r_s(u) -\frac{w_{(u,v)} p_s(u)}{\alpha d(u)} \label{eq:r-update-weighted}
\end{align}

\paragraph{Update $r_s(v)$}
\begin{align}
    p_s(v) + \alpha r_s(v) & = p_s(v) + \alpha (r_s(v)+\Delta) \\
    &= (1-\alpha) \left( \frac{w_{(u,v)} p_s(u)}{d(u)} + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{w_{(u,x)} p_s(x)}{d(x)} \right) \\
    \Longrightarrow \alpha \Delta &= (1-\alpha) \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)}\\
    \Delta &= \frac{(1-\alpha)}{\alpha} \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)}\\
    \Longrightarrow r_s'(v) &=  r_s(v) + \Delta \\
    &= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{\Delta_{w_{(u,v)}}p_s(u)}{d(u)}
\end{align}

\section{Linearity in PPR}
\begin{align}
   \pi_{\alpha, s}^{(k)} &= (1-\alpha) \pi_{\alpha, s}^{(k-1)} \bm P + \alpha v_s\\
  &= (1-\alpha)^{k} \pi_{\alpha, s}^{(0)} \bm P^{k} + \alpha \sum_{i = 1}^{k}(1-\alpha)^{i-1} v_s \bm P^{i-1} \\
%   &= \alpha \sum_{i = 0}^{k-1}(1-\alpha)^{i} \overrightarrow{v_s} \bm P^{i},  \\
  &= \alpha v_s \sum_{i = 0}^{k-1}(1-\alpha)^{i} \bm P^{i}, \text{assuming that }  \pi_{\alpha, s}^{(0)} = \bm 0 \\
  \text{Note that:  } when k \rightarrow \infty \\
  \pi_{\alpha, s} &= \alpha v_s \sum_{i = 0}^{k-1}(1-\alpha)^{i} \bm P^{i}\\
  &= v_s R_{\alpha}
\end{align}

It proves that $\pi_{\alpha, s} $ is the linear combination of $v_s$
}


% \red{it's hard for global pagerank to detect in this case} %EU-CORE-W1
% \red{it's easier to detect as degree increases more}  %EU-CORE-W3
% \red{netwalk is not aligned.}
% \red{DynAnom use node representation, AnomRank is considered as using one float number to represent the node.}

% Table \ref{tab:time-node-anomaly} present the running time of each algorithm for node-level anomaly localization. 
% NetWalk, as the node-level deep learning method, is not suitable for dynamic graphs of many snapshot since its complexity involves $T$. \red{to add more discussion}
% While AnomRank \red{todo}
\vspace{-2mm}

==> chapter2-Z-GoPPE/figs/exp-1-v6/citeseer-debug-6/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (citeseer)}
\label{tab:clf-res-citeseer-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
goppe-ista & 0.6366 \\
ppe-ista & 0.6341 \\
mixrank-all & 0.5195 \\
pprgo-ista & 0.5049 \\
mlp & 0.3951 \\
gaussian & 0.1805 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (citeseer)}
\label{tab:clf-res-citeseer-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
ppe-ista & 0.5941 \\
goppe-ista & 0.5923 \\
mixrank-all & 0.4033 \\
pprgo-ista & 0.3775 \\
mlp & 0.3356 \\
gaussian & 0.1608 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/exp-1-v6/cora-debug-6/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (cora)}
\label{tab:clf-res-cora-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
ppe-ista & 0.7861 \\
goppe-ista & 0.7790 \\
pprgo-ista & 0.6742 \\
mixrank-all & 0.6524 \\
mlp & 0.4138 \\
gaussian & 0.2266 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (cora)}
\label{tab:clf-res-cora-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
ppe-ista & 0.7673 \\
goppe-ista & 0.7568 \\
pprgo-ista & 0.5506 \\
mixrank-all & 0.5055 \\
mlp & 0.2887 \\
gaussian & 0.1379 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/exp-1-v6/flickr-debug-6/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (flickr)}
\label{tab:clf-res-flickr-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
ppe-ista & 0.4513 \\
goppe-ista & 0.4435 \\
mlp & 0.4282 \\
mixrank-all & 0.4183 \\
pprgo-ista & 0.4142 \\
gaussian & 0.3490 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (flickr)}
\label{tab:clf-res-flickr-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
ppe-ista & 0.1428 \\
goppe-ista & 0.1416 \\
mlp & 0.1269 \\
gaussian & 0.1119 \\
pprgo-ista & 0.0847 \\
mixrank-all & 0.0843 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/exp-1-v6/ogbn-arxiv-debug-6/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-all & 0.4809 \\
goppe-ista & 0.4742 \\
ppe-ista & 0.4573 \\
pprgo-ista & 0.4530 \\
mlp & 0.3565 \\
gaussian & 0.1516 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
pprgo-ista & 0.1411 \\
mixrank-all & 0.1359 \\
goppe-ista & 0.1150 \\
ppe-ista & 0.1010 \\
mlp & 0.0916 \\
gaussian & 0.0077 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/exp-1-v6/pubmed-debug-6/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (pubmed)}
\label{tab:clf-res-pubmed-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-all & 0.8045 \\
pprgo-ista & 0.7880 \\
goppe-ista & 0.7880 \\
ppe-ista & 0.7855 \\
mlp & 0.6832 \\
gaussian & 0.3960 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (pubmed)}
\label{tab:clf-res-pubmed-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mixrank-all & 0.8087 \\
pprgo-ista & 0.7933 \\
goppe-ista & 0.7782 \\
ppe-ista & 0.7717 \\
mlp & 0.6820 \\
gaussian & 0.2810 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/chameleon-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (chameleon)}
\label{tab:clf-res-chameleon-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-high_low_ppr & 0.3358 \\
mlp & 0.3202 \\
mixrank-low_ppr & 0.3177 \\
mixrank-all & 0.3153 \\
polyrank-all & 0.3153 \\
polyrank-linear & 0.3153 \\
pprgo-ista & 0.3079 \\
mixrank-high_ppr & 0.3079 \\
mixrank-random_sample & 0.2931 \\
polyrank-softmax & 0.2800 \\
goppe-ista & 0.2315 \\
polyrank-poly & 0.2315 \\
ppe-ista & 0.2315 \\
gaussian & 0.1921 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (chameleon)}
\label{tab:clf-res-chameleon-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mlp & 0.2328 \\
mixrank-high_low_ppr & 0.2215 \\
mixrank-random_sample & 0.1803 \\
mixrank-low_ppr & 0.1790 \\
mixrank-all & 0.1737 \\
polyrank-all & 0.1737 \\
polyrank-linear & 0.1737 \\
pprgo-ista & 0.1707 \\
mixrank-high_ppr & 0.1707 \\
polyrank-softmax & 0.1570 \\
gaussian & 0.1399 \\
goppe-ista & 0.0752 \\
polyrank-poly & 0.0752 \\
ppe-ista & 0.0752 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/chameleon-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (chameleon)}
\label{tab:clf-res-chameleon-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
polyrank-softmax & 0.3169 \\
polyrank-linear & 0.3136 \\
mixrank-all & 0.3136 \\
polyrank-all & 0.3136 \\
mixrank-low_ppr & 0.3112 \\
mixrank-high_low_ppr & 0.3030 \\
pprgo-ista & 0.3021 \\
mixrank-high_ppr & 0.3021 \\
mixrank-random_sample & 0.2718 \\
mlp & 0.2463 \\
ppe-ista & 0.2315 \\
goppe-ista & 0.2315 \\
polyrank-poly & 0.2291 \\
gaussian & 0.2266 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (chameleon)}
\label{tab:clf-res-chameleon-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mixrank-high_low_ppr & 0.1989 \\
mixrank-low_ppr & 0.1945 \\
gaussian & 0.1861 \\
mlp & 0.1810 \\
mixrank-random_sample & 0.1789 \\
polyrank-softmax & 0.1788 \\
polyrank-linear & 0.1735 \\
mixrank-all & 0.1735 \\
polyrank-all & 0.1735 \\
pprgo-ista & 0.1682 \\
mixrank-high_ppr & 0.1682 \\
polyrank-poly & 0.0760 \\
ppe-ista & 0.0752 \\
goppe-ista & 0.0752 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/citeseer-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (citeseer)}
\label{tab:clf-res-citeseer-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
pprgo-ista & 0.6268 \\
mixrank-high_ppr & 0.6268 \\
mixrank-all & 0.6146 \\
polyrank-linear & 0.6146 \\
polyrank-all & 0.6146 \\
polyrank-softmax & 0.6106 \\
mixrank-high_low_ppr & 0.6041 \\
mlp & 0.5268 \\
mixrank-random_sample & 0.4789 \\
goppe-ista & 0.4610 \\
mixrank-low_ppr & 0.4171 \\
polyrank-poly & 0.3520 \\
ppe-ista & 0.2537 \\
gaussian & 0.2195 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (citeseer)}
\label{tab:clf-res-citeseer-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
pprgo-ista & 0.5356 \\
mixrank-high_ppr & 0.5356 \\
polyrank-softmax & 0.5267 \\
mixrank-all & 0.5153 \\
polyrank-linear & 0.5153 \\
polyrank-all & 0.5153 \\
mixrank-high_low_ppr & 0.5130 \\
mlp & 0.4162 \\
goppe-ista & 0.4138 \\
mixrank-random_sample & 0.3630 \\
mixrank-low_ppr & 0.3144 \\
polyrank-poly & 0.2632 \\
ppe-ista & 0.2299 \\
gaussian & 0.1910 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/citeseer-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (citeseer)}
\label{tab:clf-res-citeseer-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
polyrank-linear & 0.5024 \\
mixrank-all & 0.5024 \\
polyrank-all & 0.5024 \\
mixrank-high_low_ppr & 0.4951 \\
pprgo-ista & 0.4902 \\
mixrank-high_ppr & 0.4902 \\
polyrank-softmax & 0.4829 \\
mlp & 0.4439 \\
mixrank-low_ppr & 0.4439 \\
mixrank-random_sample & 0.4203 \\
polyrank-poly & 0.3569 \\
goppe-ista & 0.2813 \\
ppe-ista & 0.2528 \\
gaussian & 0.2000 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (citeseer)}
\label{tab:clf-res-citeseer-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
polyrank-linear & 0.3999 \\
mixrank-all & 0.3999 \\
polyrank-all & 0.3999 \\
mixrank-high_low_ppr & 0.3971 \\
pprgo-ista & 0.3910 \\
mixrank-high_ppr & 0.3910 \\
polyrank-softmax & 0.3629 \\
mlp & 0.3337 \\
mixrank-low_ppr & 0.3314 \\
mixrank-random_sample & 0.3153 \\
polyrank-poly & 0.2813 \\
goppe-ista & 0.2745 \\
ppe-ista & 0.2294 \\
gaussian & 0.1702 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/cora-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (cora)}
\label{tab:clf-res-cora-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-high_low_ppr & 0.6144 \\
polyrank-softmax & 0.6031 \\
mixrank-high_ppr & 0.6003 \\
pprgo-ista & 0.6003 \\
polyrank-all & 0.5644 \\
mixrank-all & 0.5644 \\
polyrank-linear & 0.5644 \\
ppe-ista & 0.4771 \\
mixrank-random_sample & 0.4616 \\
mlp & 0.4483 \\
mixrank-low_ppr & 0.4208 \\
polyrank-poly & 0.2857 \\
goppe-ista & 0.1921 \\
gaussian & 0.1527 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (cora)}
\label{tab:clf-res-cora-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mixrank-high_low_ppr & 0.4156 \\
mixrank-high_ppr & 0.4098 \\
pprgo-ista & 0.4098 \\
polyrank-softmax & 0.4004 \\
ppe-ista & 0.3987 \\
polyrank-all & 0.3634 \\
mixrank-all & 0.3634 \\
polyrank-linear & 0.3634 \\
mixrank-random_sample & 0.2930 \\
mlp & 0.2479 \\
mixrank-low_ppr & 0.2319 \\
goppe-ista & 0.1064 \\
gaussian & 0.0972 \\
polyrank-poly & 0.0635 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/cora-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (cora)}
\label{tab:clf-res-cora-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
polyrank-softmax & 0.6151 \\
mixrank-all & 0.6045 \\
polyrank-linear & 0.6045 \\
polyrank-all & 0.6045 \\
pprgo-ista & 0.5932 \\
mixrank-high_ppr & 0.5932 \\
mixrank-high_low_ppr & 0.5925 \\
ppe-ista & 0.4567 \\
mixrank-low_ppr & 0.4469 \\
mlp & 0.4384 \\
mixrank-random_sample & 0.4307 \\
polyrank-poly & 0.2857 \\
goppe-ista & 0.2533 \\
gaussian & 0.1773 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (cora)}
\label{tab:clf-res-cora-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
polyrank-softmax & 0.4102 \\
mixrank-all & 0.4098 \\
polyrank-linear & 0.4098 \\
polyrank-all & 0.4098 \\
pprgo-ista & 0.4004 \\
mixrank-high_ppr & 0.4004 \\
mixrank-high_low_ppr & 0.3954 \\
ppe-ista & 0.3803 \\
mixrank-low_ppr & 0.2668 \\
mixrank-random_sample & 0.2471 \\
mlp & 0.2347 \\
goppe-ista & 0.1545 \\
gaussian & 0.1085 \\
polyrank-poly & 0.0635 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/film-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (film)}
\label{tab:clf-res-film-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
pprgo-ista & 0.2797 \\
mixrank-high_ppr & 0.2797 \\
mixrank-all & 0.2698 \\
polyrank-linear & 0.2698 \\
polyrank-all & 0.2698 \\
mixrank-high_low_ppr & 0.2525 \\
mixrank-low_ppr & 0.2442 \\
polyrank-softmax & 0.2384 \\
mixrank-random_sample & 0.2277 \\
mlp & 0.2228 \\
polyrank-poly & 0.2038 \\
gaussian & 0.1931 \\
goppe-ista & 0.1188 \\
ppe-ista & 0.1188 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (film)}
\label{tab:clf-res-film-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
pprgo-ista & 0.1706 \\
mixrank-high_ppr & 0.1706 \\
gaussian & 0.1697 \\
mlp & 0.1627 \\
mixrank-all & 0.1504 \\
polyrank-linear & 0.1504 \\
polyrank-all & 0.1504 \\
mixrank-high_low_ppr & 0.1489 \\
mixrank-random_sample & 0.1312 \\
mixrank-low_ppr & 0.0956 \\
polyrank-softmax & 0.0948 \\
polyrank-poly & 0.0668 \\
goppe-ista & 0.0425 \\
ppe-ista & 0.0425 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/film-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (film)}
\label{tab:clf-res-film-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-high_ppr & 0.2781 \\
pprgo-ista & 0.2781 \\
polyrank-all & 0.2698 \\
mixrank-all & 0.2698 \\
polyrank-linear & 0.2698 \\
mixrank-high_low_ppr & 0.2607 \\
polyrank-softmax & 0.2368 \\
mixrank-low_ppr & 0.2343 \\
mixrank-random_sample & 0.2277 \\
mlp & 0.2228 \\
polyrank-poly & 0.2038 \\
gaussian & 0.1931 \\
ppe-ista & 0.1188 \\
goppe-ista & 0.1188 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (film)}
\label{tab:clf-res-film-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mixrank-high_ppr & 0.1697 \\
pprgo-ista & 0.1697 \\
gaussian & 0.1697 \\
mlp & 0.1627 \\
mixrank-high_low_ppr & 0.1510 \\
polyrank-all & 0.1504 \\
mixrank-all & 0.1504 \\
polyrank-linear & 0.1504 \\
mixrank-random_sample & 0.1312 \\
polyrank-softmax & 0.0944 \\
mixrank-low_ppr & 0.0832 \\
polyrank-poly & 0.0668 \\
ppe-ista & 0.0425 \\
goppe-ista & 0.0425 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/ogbn-arxiv-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
pprgo-ista & 0.3690 \\
mixrank-high_ppr & 0.3690 \\
polyrank-all & 0.3205 \\
polyrank-linear & 0.3205 \\
mixrank-all & 0.3189 \\
mlp & 0.3102 \\
mixrank-random_sample & 0.2566 \\
mixrank-high_low_ppr & 0.2331 \\
mixrank-low_ppr & 0.2322 \\
ppe-ista & 0.1448 \\
gaussian & 0.1368 \\
goppe-ista & 0.1175 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
pprgo-ista & 0.0553 \\
mixrank-high_ppr & 0.0553 \\
mlp & 0.0460 \\
polyrank-all & 0.0402 \\
polyrank-linear & 0.0402 \\
mixrank-all & 0.0397 \\
mixrank-random_sample & 0.0249 \\
mixrank-high_low_ppr & 0.0216 \\
mixrank-low_ppr & 0.0211 \\
gaussian & 0.0150 \\
ppe-ista & 0.0063 \\
goppe-ista & 0.0053 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/ogbn-arxiv-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
polyrank-all & 0.3519 \\
polyrank-linear & 0.3516 \\
pprgo-ista & 0.2879 \\
mixrank-high_ppr & 0.2879 \\
mixrank-all & 0.2602 \\
mlp & 0.2516 \\
mixrank-random_sample & 0.1984 \\
mixrank-low_ppr & 0.1726 \\
mixrank-high_low_ppr & 0.1640 \\
goppe-ista & 0.1441 \\
gaussian & 0.1258 \\
ppe-ista & 0.0586 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (ogbn-arxiv)}
\label{tab:clf-res-ogbn-arxiv-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
polyrank-all & 0.0528 \\
polyrank-linear & 0.0527 \\
pprgo-ista & 0.0382 \\
mixrank-high_ppr & 0.0382 \\
mixrank-all & 0.0272 \\
mlp & 0.0262 \\
mixrank-random_sample & 0.0160 \\
mixrank-low_ppr & 0.0105 \\
gaussian & 0.0097 \\
mixrank-high_low_ppr & 0.0087 \\
goppe-ista & 0.0063 \\
ppe-ista & 0.0047 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/squirrel-debug-4/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (squirrel)}
\label{tab:clf-res-squirrel-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mlp & 0.2438 \\
mixrank-high_ppr & 0.2430 \\
pprgo-ista & 0.2430 \\
mixrank-high_low_ppr & 0.2239 \\
mixrank-low_ppr & 0.2143 \\
gaussian & 0.2139 \\
polyrank-softmax & 0.2114 \\
polyrank-poly & 0.2114 \\
polyrank-all & 0.2114 \\
polyrank-linear & 0.2114 \\
mixrank-all & 0.2114 \\
ppe-ista & 0.2114 \\
goppe-ista & 0.2114 \\
mixrank-random_sample & 0.2032 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (squirrel)}
\label{tab:clf-res-squirrel-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
mlp & 0.2152 \\
gaussian & 0.1889 \\
mixrank-high_ppr & 0.1372 \\
pprgo-ista & 0.1372 \\
mixrank-high_low_ppr & 0.1242 \\
mixrank-random_sample & 0.1041 \\
mixrank-low_ppr & 0.0816 \\
polyrank-softmax & 0.0698 \\
polyrank-poly & 0.0698 \\
polyrank-all & 0.0698 \\
polyrank-linear & 0.0698 \\
mixrank-all & 0.0698 \\
ppe-ista & 0.0698 \\
goppe-ista & 0.0698 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/figs/legacy/squirrel-debug-5/tab-clf-res.tex <==
\begin{table}[ht]
\centering
\caption{Avg. Accuracy (squirrel)}
\label{tab:clf-res-squirrel-avg-acc}
\begin{tabular}{lr}
\toprule
 & accuracy-mean \\
model &  \\
\midrule
mixrank-high_low_ppr & 0.2347 \\
mlp & 0.2338 \\
pprgo-ista & 0.2293 \\
mixrank-high_ppr & 0.2293 \\
mixrank-random_sample & 0.2131 \\
mixrank-low_ppr & 0.2114 \\
polyrank-softmax & 0.2114 \\
polyrank-all & 0.2114 \\
polyrank-linear & 0.2114 \\
goppe-ista & 0.2114 \\
ppe-ista & 0.2114 \\
polyrank-poly & 0.2114 \\
mixrank-all & 0.2114 \\
gaussian & 0.1642 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Avg. Macro-F1 (squirrel)}
\label{tab:clf-res-squirrel-avg-macro-f1}
\begin{tabular}{lr}
\toprule
 & macro-f1-mean \\
model &  \\
\midrule
gaussian & 0.1416 \\
mixrank-high_low_ppr & 0.1340 \\
mlp & 0.1319 \\
pprgo-ista & 0.1255 \\
mixrank-high_ppr & 0.1255 \\
mixrank-random_sample & 0.1172 \\
mixrank-low_ppr & 0.0698 \\
polyrank-softmax & 0.0698 \\
polyrank-all & 0.0698 \\
polyrank-linear & 0.0698 \\
goppe-ista & 0.0698 \\
ppe-ista & 0.0698 \\
polyrank-poly & 0.0698 \\
mixrank-all & 0.0698 \\
\bottomrule
\end{tabular}
\end{table}



==> chapter2-Z-GoPPE/goppe-algo.tex <==

\begin{algorithm}[ht]
\caption{$\textsc{GoPPE}(\mathcal{G}_0, \Delta E_{1, \ldots, T}, \bm X_{1, \ldots, T}, \mathcal{S}, \epsilon, \alpha)$ }
\begin{algorithmic}[1]
\footnotesize
\State \textbf{Input: }  
Initial graph $\mathcal{G}_0 = (\mathcal{V}, \mathcal{E}_0, \bm X_0)$, 
Edge events $ \Delta E_{1, \ldots, T}$, 
Node attributes $ \bm X_{1, \ldots, T}$ , 
The train/test node sets, denoted as $\mathcal{\bar{S}} \text{ and }\mathcal{\hat{S}}$, respectively. And $\mathcal{S} = \mathcal{\bar{S}} \cup \mathcal{\hat{S}}$. 
PPR teleport factor $\alpha $,
PPR Vector $\ell_1$-error control parameter $\epsilon$.

\State $\bm \pi_{u, init} = \bm 0, \forall u \in \mathcal{S}$
\State \textcolor{blue}{// Calculate Initial PPR for each node $u$ in $\mathcal{S}$ using Algorithm \ref{algo:ppr-ista}.}
\State $\bm x_{u, t=0}, \nabla_{u, t=0} = \textsc{PPRIsta}(\mathcal{G}_0, \bm \pi_{u, init}),  \forall u \in \mathcal{S} $ 
\State $\bm \pi_{u, t=0} =  \sqrt{\bm d(u)} \times \bm x_{u, t=0}  ,  \forall u \in \mathcal{S} $
\State \textcolor{blue}{// Get Contextualized Node Features and Positional Encodings}
\State $\bm h_{u,t=0} = \textsc{FeatureFormer}(\bm \pi_{u, t=0},\bm X_0),  \forall u \in \mathcal{S} $ 
\State \textcolor{blue}{// Train classifier with the training samples $\bar{u} \in \mathcal{\bar{S}} \subset \mathcal{S} $}
\State $f_{\bm \Theta,t=0}(\cdot) = \textsc{Train}(\bm h_{\bar{u}, t=0}, \bm y(\bar{u})),  \forall \bar{u} \in \mathcal{\bar{S}}$ 
\State \textcolor{blue}{// Infer for the testing samples $\bm h_{\hat{u},t=0}, \forall \hat{u} \in \mathcal{\hat{S}}$}
\State $ \bar{y}_{\hat{u}, t=0} = f_{\bm \Theta,t=0}(\bm h_{\hat{u}}), \forall \hat{u} \in \mathcal{\hat{S}} $ 
\State \textcolor{blue}{// Update graphs, maintain PPR, then train/evaluate repeatedly.}
\For{$t \in [1,T] $}
    \State $ \bar{\bm x}_{u, t-1} =\textsc{PPRAdjust}(\bm x_{u, t-1}, \Delta E_{t})$
    \State $\mathcal{G}_{t} = \textsc{GraphUpdate}(\mathcal{G}_{t-1}, \Delta E_t, \bm X_t)$
    \State $\bm x_{u, t}, \nabla_{u, t} = \textsc{PPRIsta}(\mathcal{G}_1, \bar{\bm x}_{u, t-1}),  \forall u \in \mathcal{S} $ 
    \State $\bm \pi_{u, t} =  \sqrt{\bm d(u)} \times \bm x_{u, t}  ,  \forall u \in \mathcal{S} $
    \State $\bm h_{u,t} = \textsc{FeatureFormer}(\bm \pi_{u, t},\bm X_t),  \forall u \in \mathcal{S} $
    \State $f_{\bm \Theta,t}(\cdot) = \textsc{Train}(\bm h_{\bar{u}, t}, \bm y(\bar{u})),  \forall \bar{u} \in \mathcal{\bar{S}}$ 
    \State $ \bar{y}_{\hat{u},t} = f_{\bm \Theta,t}(\bm h_{\hat{u}}), \forall \hat{u} \in \mathcal{\hat{S}} $ 
\EndFor

\State \textbf{return} $\bar{y}_{\hat{u},t \in \{ 0, 1, \ldots, T \}}, \forall \hat{u} \in \mathcal{\hat{S}}$

\noindent\hrulefill
\Procedure{FeatureFormer}
{$\bm \pi_u,\bm X$}
\State \textcolor{blue}{// PPR-guided Node Contextualization}
\State $\bm h^c_u =  \bm X \bm \pi_u $
% \State \textcolor{red}{// There are many other aggregation designs }
\State \textcolor{blue}{// PPR-based Node Positional Encodings}
\State $\bm p_i = \textsc{HashReduceDim}(\bm \pi_u, \bar{d}=512)$
\State $\bm h^p_u = \bm W_{pe} \bm p_i $
\State \textbf{return}  Apply \textit{Concatenative PE }in Equ.\ref{equ:goppe} 
\EndProcedure

\noindent\hrulefill
\Procedure{PPRAdjust}{$ \bm x, \Delta E$}
% \State $t=0$
\For{$(u ,v)\in \Delta E$}
    \State $\bar{\bm x}_u:=$ update $\bm x_u$ Using Theorem \ref{theorem:update}.
    % \State \textcolor{blue}{Note that only $\bm x$}
\EndFor

\State \textbf{return} $ \bar{\bm x}$ 
\EndProcedure

\noindent\hrulefill
\Procedure{HashReduceDim}{$x,d$ } \label{proc:HashReduce}
\State // Hash function $h_{d}(i): \mathbb{N}\to [d]$
\State // Hash function $h_{\operatorname{sgn}}(i): \mathbb{N}\to \{ \pm 1\}$
\State $\bar x = \bm 0 \in \mathbb{R}^{d}$
\For{$i \in \textsc{Supp}|x|$}
    \State $j = h_{dim}(i)$
    \State $\bar x(j) \pluseq h_{\operatorname{sgn}}(i) \log \left(x(i) \right)$
\EndFor
\State \textbf{return} $ \frac{\bar x}{\| \bar x \|_1}$
\EndProcedure

\end{algorithmic}
\label{algo:goppe}
\end{algorithm}


==> chapter3-TitleModification/Figures/tex_samples_in_BERTScore_range_0.tex <==
\begin{tabular}{p{0.38\textwidth}|p{0.38\textwidth}|p{0.04\textwidth}|p{0.1\textwidth}}
\toprule
                                                                                                              Before &                                                                                     After &  Edit Dis. & BERTScore \\ \hline
\midrule
                                                                                                 the color of fandom &                                                        even when white men can jump . . . &          9 &   -0.0404 \\ \hline
                                                                     wall street slips on jitters before fed meeting &                                              s\&p 500 and dow end session at record highs &          9 &   -0.1540 \\ \hline
                                                                 amazon announces new york and virginia as hq2 picks &                before a deal , amazon had to know : could cuomo and de blasio get along ? &         15 &   -0.0930 \\ \hline
                                                                                                        \#bretttoo ? &                                      why america needs to hear brett kavanaugh ’s accuser &          9 &   -0.0626 \\ \hline
                                                 gold prices see muted trade after adp ’s private sector jobs report &                   gold heads higher , but looks to post biggest quarterly loss since 2016 &         12 &   -0.0138 \\ \hline
                                               \#oscarssowhite held up a mirror . hollywood still ca n’t look away . &                                     the hashtag that changed the oscars : an oral history &         13 &   -0.0787 \\ \hline
                                                                                   what trump and corruption cost us &                                  marie yovanovitch fought corruption , then lost her post &          8 &   -0.0045 \\ \hline
                                            jared kushner , trump ’s son- in - law , explores joining administration &                    trump offers national security post to michael flynn , retired general &         12 &   -0.0011 \\ \hline
                                                               if they ’re ‘essential , ’ they ca n’t be ‘ illegal ’ &                                                 a former farmworker on american hypocrisy &         13 &   -0.0183 \\ \hline
                                                                                   four more years of what exactly ? &                                                                      grievances on parade &          7 &   -0.1620 \\ \hline
                                                                                           surveillance as a service &                                             amazon wants to get even closer . skintight . &          9 &   -0.1191 \\ \hline
                                                                      out of office : a survey of our new work lives &                                                                work may never be the same &         11 &   -0.0099 \\ \hline
                                                                                are billionaires bad for democracy ? &                                           bill gates , i implore you to connect some dots &         10 &   -0.0364 \\ \hline
                                                                       democrats must make judgeships a top priority &                                                            what mitch mcconnell got right &          7 &   -0.0603 \\ \hline
                                                                                        democrats of the living dead &                                 have zombies eaten bloomberg ’s and buttigieg ’s brains ? &         10 &   -0.0053 \\ \hline
                                            polk awards honor articles on russia investigation and \# metoo movement &                                        new york times leads polk winners with four awards &         11 &   -0.0354 \\ \hline
                                             ta-nehisi coates rebukes mitch mcconnell at raucous reparations hearing &    digging into america ’s dark past , house panel makes history by exploring reparations &         14 &   -0.0411 \\ \hline
                                                party of personal responsibility declines to hold person responsible &                marjorie taylor greene apologized and got a standing ovation . seriously . &         12 &   -0.1253 \\ \hline
                                                            water main break plunges kennedy airport back into chaos &                                      jfk travelers ask : when can i catch a flight home ? &         12 &   -0.0025 \\ \hline
                                                                       unemployment claims rose slightly last week . &                                                        looking for signs of economic hope &          7 &   -0.0142 \\ \hline
                                                                                      if all this was just a movie … &                                                                 lights , camera , trump ! &          8 &   -0.1748 \\ \hline
                                               among the victims of the london attack : keith palmer and aysha frade &                               london attack leaves citizens of 10 nations dead or injured &         13 &   -0.0256 \\ \hline
                                                    moment knife - wielding thug charges at crowds during mass brawl &             covid uk : violence in liverpool , cardiff and primrose hill amid hot weather &         14 &   -0.0384 \\ \hline
                                                                 doctors should stand against trump reviving torture &                                                                when doctors first do harm &          7 &   -0.0768 \\ \hline
                                                        florida recount nears an end as counties finish manual tally &                                    bill nelson concedes florida senate race to rick scott &         10 &   -0.0500 \\ \hline
                                                                                  realism and repentance in virginia &                                                       why ralph northam should not resign &          6 &   -0.0889 \\ \hline
                                                                 photo by simone cecchetti / corbis via getty images &                                                                           gender euphoria &          9 &   -0.3761 \\ \hline
                                                                       to excuse trump , republicans embrace fantasy &                                                             devin nunes is danielle steel &          7 &   -0.1099 \\ \hline
                                                   turkey says it has identified gunman in istanbul nightclub attack &                                      in turkey , u.s. hand is seen in nearly every crisis &          9 &   -0.0167 \\ \hline
                                         gen z , i am genuinely curious if you have any clue who these 27 celebs are &                                       early ' 00s celebrity quiz : do you remember them ? &         16 &   -0.0016 \\ \hline
                                           2019 u.s. open : no. 2 barty and no . 3 pliskova lose in the fourth round &                                    serena williams wins as her half of the draw thins out &         17 &   -0.0224 \\ \hline
                                                                      what to watch : day 2 of cabinet confirmations &                 robert gates calls rex tillerson ‘ deeply knowledgeable ’ about the world &         12 &   -0.1056 \\ \hline
                                                                                           brexit , act iv , scene i &                                                              the brexit disaster has legs &          7 &   -0.0415 \\ \hline
                                             wall street opens higher ahead of march business surveys ; intel shines &                                  financials lift s\&p 500 , dow ; powell , yellen on deck &         12 &   -0.1197 \\ \hline
                                       de blasio to trump : ‘ are you telling n.y.c. to drop dead ? ’ : live updates &                                       watch now : governor cuomo gives coronavirus update &         17 &   -0.0515 \\ \hline
                                                                                                    at summer ’s end &                                                     our days have always been running out &          7 &   -0.0018 \\ \hline
                                                    a ‘ country grappling ’ with just about everything seeks answers &                                          the choice between biden ’s america and trump ’s &         11 &   -0.0090 \\ \hline
                                    elie honig explains what sedition charges may mean in capitol riot investigation &                 acting washington us attorney : ' unequivocal that trump was the magnet ' &         13 &   -0.1119 \\ \hline
                                                                     pete buttigieg and the parable of the wine cave &                                                                    give joe biden his due &          9 &   -0.1273 \\ \hline
                                                                               critiques of the pence- harris debate &                                 ‘ that intrepid fly respected the two-minute time limit ’ &          9 &   -0.0637 \\ \hline
                                          mulvaney withdraws effort to join impeachment lawsuit after bolton objects &                   feud between trump advisers underscores a white house torn by rivalries &         11 &   -0.0994 \\ \hline
                                             redline communications reports 2020 fourth quarter and year end results &                  / c o r r e c t i o n from source -- redline communications group inc. / &         18 &   -0.4584 \\ \hline
                                                                     where were you when oddvar bra broke his pole ? &                                                the ski pole that norway will never forget &         10 &   -0.0682 \\ \hline
                                                     hallucinogen eases depression in cancer patients , studies find &               a dose of a hallucinogen from a ‘ magic mushroom , ’ and then lasting peace &         14 &   -0.0077 \\ \hline
                                                                  u.k. prime minister to visit republicans ’ retreat &                           trump finds a target more tempting than obama : chelsea manning &         11 &   -0.0192 \\ \hline
                                         myanmar built camps to hold them . 730,000 people who fled wo n’t move in . &                  squalor , monsoons and rampaging elephants : home still scares them more &         16 &   -0.0429 \\ \hline
                                                         world cup 2018 : nigeria vs. croatia live score and updates &                                           croatia tops nigeria to take control of group d &         10 &   -0.0293 \\ \hline
                                                              service with a human touch — no smartphone can do that &                                                         the secret lives of hotel doormen &         11 &   -0.1163 \\ \hline
                                                                           jobs report for march : what to watch for &                                 u.s. added 103,000 jobs in march ; unemployment at 4.1 \% &         10 &   -0.1203 \\ \hline
                                                       public impeachment hearings will begin next week , house says &           top ukraine diplomat testified giuliani spearheaded pressure for investigations &         10 &   -0.1306 \\ \hline
                                                                    mnuchin meets with mohammed bin salman in riyadh &                            trump administration sends conflicting signals on saudi arabia &          8 &   -0.0192 \\ \hline
                                                maduro defends his no . 2 after u.s. allegations of drug trafficking &               venezuela closes ranks around sanctioned vice president , tareck el aissami &         12 &   -0.0315 \\ \hline
                                               a charity auction for coffee with ivanka trump appears to be canceled &                                               obama to russia : ‘we can do stuff to you ’ &         11 &   -0.0789 \\ \hline
                                                        global stocks follow wall st up on strong japan , korea data &                              wall street moves higher , pushing s\&p 500 over 4,000 level &         12 &   -0.1563 \\ \hline
                                                                              stocks and forex ride out turkey shock &                       global equities inch higher , bonds gain as europe covid cases rise &         12 &   -0.0540 \\ \hline
                                                                                         6,000 miles north of hawaii &                                                         surfing under the northern lights &          5 &   -0.0850 \\ \hline
                                                          harborside secures \\$ 12 million revolving credit facility &                                   / c o r r e c t i o n from source -- harborside inc . / &         17 &   -0.4588 \\ \hline
                                                           marco rubio will vote for tillerson as secretary of state &                    taxpayers will defend trump in suit charging constitutional violations &          9 &   -0.0063 \\ \hline
                                                      sessions ’s senate testimony : how to watch and what to expect &                          rosenstein vows mueller will have independence in russia inquiry &         12 &   -0.0515 \\ \hline
                                                 glugs of olive oil , flurries of cheese and two new menus every day &                               it takes a lot of skill to make a restaurant seem so casual &         14 &   -0.0275 \\ \hline
                                                                              when government works for the governed &                                       america deserves a leader as good as jacinda ardern &          9 &   -0.0541 \\ \hline
                                                          trump ’s washington hotel lost money in its opening months &                                 marco rubio will vote for tillerson as secretary of state &         10 &   -0.0488 \\ \hline
                                                      questioned over coronavirus deaths , china tries to curb grief &            china ​p​ushes for ​q​uiet ​b​urials ​amid ​q​uestioning ​o​ver ​d​eath ​to​ll &         10 &   -0.3982 \\ \hline
                                                                 is the enemy of the enemy of the people my friend ? &                                               the midterms are getting weirder and weider &         11 &   -0.1576 \\ \hline
                                                                          watch now : cuomo gives coronavirus update &                     n.y. virus deaths double in three days to almost 3,000 : live updates &         13 &   -0.0348 \\ \hline
                                                                                            new york ’s arts for all &                                       the newfound power of people wielding library cards &          8 &   -0.0324 \\ \hline
                                                          echoes of aids epidemic as south africa fights coronavirus &                  how can you social distance when you share a toilet with your neighbor ? &         14 &   -0.0516 \\ \hline
                                                                                            vote and renew democracy &                    you ’re not just voting for president . you ’re voting to start over . &         15 &   -0.0004 \\ \hline
         nearly half million covid - 19 related in - bound and out - bound calls handled by cortex registered nurses &                                                     / disregard release : cortex health / &         19 &   -0.2536 \\ \hline
                             golden globes 2018 live updates : ‘ three billboards ’ and ‘ lady bird ’ win top awards &                                 a golden globes draped in black warily addresses \# metoo &         17 &   -0.1398 \\ \hline
                                                                                 n’golo kanté and the art of winning &                                                        at chelsea , hard work as high art &          8 &   -0.0453 \\ \hline
                                                        what will today ’s g.d.p. reading show ? here ’s a preview . &                                        u.s. economy grew at 2.1 \% rate in fourth quarter &         13 &   -0.0201 \\ \hline
                                                          who is dimitrios pagourtzis , the texas shooting suspect ? &                                                                                        tk &         10 &   -0.3898 \\ \hline
                                                                                                      lives derailed &                  we spoke to 430 former immigrants in mexico . this is what they shared . &         15 &   -0.0488 \\ \hline
                                                       trump returns to u.s. , and to berating news media on twitter & reported talks by jared kushner with russia would be ‘ good thing , ’ trump official says &         17 &   -0.0063 \\ \hline
                                       de blasio announces task forces and councils to guide recovery : live updates &                                       watch now : governor cuomo gives coronavirus update &         13 &   -0.0007 \\ \hline
                                                                                                 injustice on repeat &                                      the injustice of this moment is not an ‘aberration ’ &          9 &   -0.1225 \\ \hline
                             movie theaters in n.y.c. can reopen with limited capacity late next week , cuomo says . &                 covid - 19 : u.s. surpasses 500,000 covid - 19 deaths , a monumental loss &         15 &   -0.0043 \\ \hline
                                                                                                      occupy hungary &                                                can students save george soros 's school ? &          8 &   -0.0941 \\ \hline
                                                     texas shooting victims ranged in age from 18 months to 77 years &    one minute they were a family praying in church . the next , eight of them were dead . &         18 &   -0.0279 \\ \hline
                                                               amid covid - 19 , china ups its game in latin america &                                                                     ‘ gracias china !!! ’ &         11 &   -0.0781 \\ \hline
                                                              u.s. added 209,000 jobs in july , beating expectations &                               jobs , factories and stocks provide economic lift for trump &         10 &   -0.0627 \\ \hline
                                                                                heat wave keeps its grip on new york &                more than 19,500 con edison customers lose power in third day of heat wave &         14 &   -0.0351 \\ \hline
                                                           new york politicians offer tax returns and pokes at trump &                                     what de blasio made as landlord , and cuomo as author &         10 &   -0.0558 \\ \hline
                                                     for interior , montanan with deep roots and inconsistent record &                                he will soon run a fifth of the nation . meet ryan zinke . &         14 &   -0.0104 \\ \hline
                                                        why amadou diallo ’s mother still fights ‘ this good fight ’ &                                     years before black lives matter , 41 shots killed him &         12 &   -0.0495 \\ \hline
                                                                                   where kites fly , kites also fall &                                                         meet the bird medics of new delhi &          7 &   -0.1401 \\ \hline
                                          xerox , an innovator hit by digital revolution , cedes control to fujifilm &                         after era that made it a verb , xerox , in a sale , is past tense &         16 &   -0.0305 \\ \hline
                                                                    oil prices ease after suez canal traffic resumes &                        banking shares retreat as markets weigh mixed trends on covid - 19 &         12 &   -0.0163 \\ \hline
                                                                                          dirty politics in new york &                                                andrew cuomo owes cynthia nixon an apology &          7 &   -0.0859 \\ \hline
engine debris rained over a mile across a denver suburb . now boeing recommends suspending its 777s with that engine &           engine on united airlines flight was showing signs of metal fatigue , ntsb says &         19 &   -0.0170 \\ \hline
                                                                                        turn on , tune in , start up &                                                      how and why silicon valley gets high &          8 &   -0.0685 \\ \hline
                                                     turkey rejects 2nd appeal to release u.s. pastor andrew brunson &                            qatar comes to aid of turkey , offering \\$ 15 billion lifeline &         12 &   -0.0149 \\ \hline
                                                                          s\&p 500 , nasdaq slip as bond yields rise &                         u.s. stocks close mixed as dow notches fifth straight record high &         11 &   -0.0315 \\ \hline
                                   champignon brands restates financial statements and md\&a files listing statement &                            / c o r r e c t i o n from source -- champignon brands inc . / &         18 &   -0.4218 \\ \hline
                         protest updates : ahmaud arbery suspect used racist slur after shooting , investigator says &               george floyd protest updates : murkowski endorses mattis ’s rebuke of trump &         13 &   -0.0530 \\ \hline
         biden will begin undoing trump ’s changes to title ix , including how colleges investigate sexual assault . &                    number of migrant children detained at border has tripled in two weeks &         18 &   -0.0778 \\ \hline
                                                                        mastering the monologue and the mammoth part &                                                      the part seems impossible ? hire her &          7 &   -0.0006 \\ \hline
                                                                                    mr. trump , do n’t back down now &                                                          jamal khashoggi deserves justice &          8 &   -0.1831 \\ \hline
                                                       trump : ‘i said roy moore will not be able to win’ in alabama &                                for trump , a moment of defeat but maybe not recalibration &         14 &   -0.0472 \\ \hline
\bottomrule
\end{tabular}



==> chapter3-TitleModification/Tables/BERTScore_range_0.tex <==
\begin{tabular}{p{0.4\textwidth}|p{0.4\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}}
\toprule
Original Text & Edited Text &  Edit Dis. & BERT Score\\
\toprule
                             house to approve stopgap bill as shutdown deadline nears &         ‘ shut it down ’ : trump threatens government shutdown over border security & 12 & -0.039919 \\ \hline
                                            america exports its corruption to ukraine &                  ‘ the beacon has gone out ’ : what trump and giuliani have wrought & 14 & -0.108891 \\ \hline
social media pollution , a huge problem in the last election , could be worse in 2020 & kissing babies , loving scrapple , fighting viral hoaxes : ’ 20 race ’s new routine & 16 & -0.042662 \\ \hline
                         senate committee advances jeff sessions for attorney general &                 trump to senate majority leader : ‘ go nuclear ’ to confirm gorsuch & 12 & -0.081574 \\ \hline
                     your power bill is likely to rise under lockdown . here ’s why . &                                       the city that never sleeps is waking up later & 14 & -0.007226 \\ \hline
\bottomrule
\end{tabular}



==> chapter3-TitleModification/Tables/BERTScore_range_1.tex <==
\begin{tabular}{p{0.4\textwidth}|p{0.4\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}}
\toprule
      ‘ no compromise , ’ democratic hopefuls say about gun control &                2020 democrats demand gun control , but differ on tactics & 11 & 0.345635 \\ \hline
                                 guess who ’s coming to trump tower & trump ’s son-in - law consults with lawyers about joining administration & 11 & 0.135659 \\ \hline
         on a greek island , migrants and locals are wary neighbors &             the scenic isle where the world ’s chaos comes home to roost & 12 & 0.145486 \\ \hline
2017 super bowl : patriots still fighting , but time is running out &                  2017 super bowl : patriots cut falcons ’ lead to 28- 20 &  8 & 0.255338 \\ \hline
  u.k. parliament faces a key brexit question : what does it want ? &   theresa may promises to step down if u.k. parliament backs brexit plan & 13 & 0.349018 \\ \hline
\bottomrule
\end{tabular}



==> chapter3-TitleModification/Tables/BERTScore_range_2.tex <==
\begin{tabular}{p{0.4\textwidth}|p{0.4\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}}
\toprule
                        mass shooting , trade war , r. kelly : your tuesday briefing &             toni morrison , mass shooting , r. kelly : your tuesday briefing &  4 & 0.686924 \\ \hline
            just days into a new congress , liberal freshmen are shaking the capitol &     liberal freshmen are shaking the capitol just days into the new congress & 13 & 0.666004 \\ \hline
michael phelps is o.k. with losing world records , and confident he is still no . 1. &    michael phelps is losing world records , but he ’s gained other treasures &  9 & 0.502817 \\ \hline
                       plane skids off runway in turkey , teetering on water ’s edge &            plane skids off runway in turkey : ‘ it ’s a miracle we escaped ’ &  9 & 0.466205 \\ \hline
                           british police arrest second man in london subway bombing & britain lowers threat level after arrest of 2nd man in london subway bombing &  7 & 0.670106 \\ \hline
\bottomrule
\end{tabular}



==> chapter3-TitleModification/Tables/BERTScore_range_3.tex <==
\begin{tabular}{p{0.4\textwidth}|p{0.4\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}}
\toprule
Original Text & Edited Text &  Edit Dis. & BERT Score\\
\toprule
                                        julia louis-dreyfus tweets news of breast cancer &                                                     julia louis-dreyfus says she has breast cancer & 3 & 0.807326 \\ \hline
    kimberly guilfoyle , top fund - raising official for trump campaign , tests positive & kimberly guilfoyle , top fund - raising official for trump campaign , tests positive for the virus & 3 & 0.930987 \\ \hline
north korea postpones talks with south korea and hints kim -trump summit may be in peril &                     north korea postpones talks with south , hinting kim -trump summit is in peril & 5 & 0.829025 \\ \hline
                                 shooting near raptors ’ victory parade leaves 2 injured &                                            shooting near raptors ’ victory parade leaves 4 wounded & 2 & 0.973514 \\ \hline
                u.k. general election 2019 : conservatives secure majority in parliament &                     u.k. general election 2019 : conservatives secure large majority in parliament & 1 & 0.973670 \\ \hline
\bottomrule
\end{tabular}



==> chapter3-TitleModification/Tables/tab_bertscore_by_agency.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &   Mean &   Std. &  Median &  Number \\
Domain          &        &        &         &         \\
\midrule
Huffington Post & 0.8292 & 0.1730 &  0.8966 &     174 \\
The Epoch Times & 0.8260 & 0.1740 &  0.8908 &     687 \\
The Hill        & 0.8087 & 0.1826 &  0.8644 &     336 \\
Fox News        & 0.7659 & 0.2310 &  0.8645 &     535 \\
New York Post   & 0.7305 & 0.2424 &  0.8174 &     923 \\
National Review & 0.7268 & 0.2660 &  0.8305 &      42 \\
The Blaze       & 0.7200 & 0.2758 &  0.8145 &     176 \\
CNN             & 0.6888 & 0.2531 &  0.7493 &    1288 \\
Washington Post & 0.6840 & 0.2778 &  0.7916 &     916 \\
Newsmax         & 0.6733 & 0.2714 &  0.7319 &      26 \\
Daily Beast     & 0.6584 & 0.2915 &  0.7693 &     570 \\
MarketWatch     & 0.6551 & 0.2608 &  0.7011 &    2591 \\
BBC             & 0.6031 & 0.2671 &  0.6260 &    1333 \\
Yahoo News      & 0.5985 & 0.2801 &  0.6160 &   19224 \\
Daily Mail      & 0.5936 & 0.2741 &  0.6348 &    5681 \\
OAN             & 0.5830 & 0.2590 &  0.5910 &    2177 \\
The Guardian    & 0.5579 & 0.2896 &  0.5826 &    1366 \\
New York Times  & 0.5234 & 0.3283 &  0.5595 &    1844 \\
BuzzFeed        & 0.5085 & 0.2529 &  0.4872 &    2017 \\
\bottomrule
\end{tabular}



==> chapter3-TitleModification/deprecate/background.tex <==
% \section{Motivation and Background}

% In this section, we first present background information on news
% agencies and online news platforms. Next, we define what an article
% title change is in the scope of this paper. We then explain how we
% chose which news publishers to monitor for article headline changes.


==> chapter3-TitleModification/deprecate/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion} 
In 2022, trust in the media is at an all-time low. In this paper, we explored one dimension that we argue has the potential to further reduce the public's trust in news outlets: post-publication headline changes. By monitoring over 411K articles for seven months across tens of news outlets, we discovered that 7.5\% of titles changed at least once after they were published. This rate of headline modifications is anything but uniform, with certain popular outlets changing almost half of their headlines \emph{after} publication. We used the BERTScore metric and devised a taxonomy to automatically characterize the type of post-publication change. 
We find that 49.7\% of changes go beyond benign corrections and updates, with 23.13\% corresponding to categories such as emotionalism, neutralization, and personalization.
%Even though the majority of changes (50.3\%) correspond to clarifications, dynamic updates of breaking news, and other benign categories, we find that 23.13\% of the modifications belong to categories that are significantly less benign, such as, emotionalism, neutralization, and personalization. 
We also characterized the effects of post-publication headline changes in relation to social media. Among others, we discovered that maximal spread of news on Twitter happens within ten hours after publication and therefore a delayed headline correction will come \emph{after} users have consumed and amplified inaccurate headlines. Finally, we discussed the issue of content caching in social networks and how it can further exacerbate the propagation of stale headlines.

\noindent\textbf{Acknowledgements:} This work was supported by the National Science Foundation (NSF) under grants CMMI-1842020, CNS-1941617, CNS-2126654, IIS-1926781, IIS-1927227, IIS-1546113 and OAC-1919752.

\noindent\textbf{Availability} To assist in the understanding of the spread of misinformation on the web, we are open-sourcing our news headline dataset: \url{https://scripta-volant.github.io/}

%Additionally, we will continue monitoring the news articles and report on future headline changes. This, along with our dataset, will be available post-publication.
%can be found on our website: %\url{https://verbavolant.github.io}\todo{Put real URL here}



==> chapter3-TitleModification/deprecate/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\noindent\textbf{Headline Changes.} The Internet has dramatically
decreased the time between newsworthy events, and the consumption of
information regarding those events by the public. This, along with the
propensity of people to simply skim headlines rather than read full articles~\cite{readheadlines}, 
has fostered an environment where post-publication changes to
article headlines can lead to diverging world-views among readers.
In this work, we studied the behavior of news publishers and
developed a taxonomy of article headline modifications. We find that
popular news publishers regularly make post-publication changes to their
headlines, with some modifying almost half of them. 

Additionally, we categorize these changes
into well-defined groups, allowing us to quantify the behaviors of each
publisher. We find that the majority of headline changes correspond to
updates of ongoing events. Alarmingly however, 20.13\% of headline changes are made to
either increase or decrease the provocativeness of the headline, presenting
a distorted view of the subject-matter to different groups of readers. Using
this taxonomy, we are able to quantify the different headline update strategies
of each news outlet studied, discovering a divergence in the perceived motives
between publishers.

While the news outlets presented in this study do not appear to have outright
malicious intentions, their actions contribute to the overall decrease in integrity
of information consumed by millions of people. 
In order to slow the spread of misinformation in society, news outlets should
limit the rate in which their article headlines are modified. With the speed in 
which news travels, headline changes can have devastating effects to reader 
understanding. We argue that, if a headline must be changed, the new headline should maintain
high lexical similarity to the original headline, only adding new information
to enhance reader understanding. 

%Moreover, news outlets should strive to alert
%readers that a headline has changed after original publication. We note that 
%some publishers provide readers with both a \emph{Published} and \emph{Updated}
%timestamp on each article webpage. However, we argue that this insufficient as many
%readers simply skim article headlines on the homepages of new outlets, rather than 
%click-through to each article's webpage. Rather, news outlets should include this information in all places an 
%article is referenced on their site, allowing a reader to revisit an article upon
%noticing its headline has been updated. 

\noindent\textbf{Information Travel on Social Media. }The rapid propagation
of information through shares and retweets on social media has only exasperated
the negative ramifications of news article headline modifications. By observing
the engagement of tweets associated with news articles with modified headlines,
we determined that the majority of favorites and retweets occur within ten hours 
of a tweet's publication. Due to the caching of article metadata and previews on
Twitter, most article shares will contain a different headline than what is active
on the publisher's website. While it is infeasible for social media platforms to 
constantly monitor each and every webpage linked to from all posts, decreasing the
caching of content can help reduce the spread of misinformation online. Moreover,
it would be worthwhile to explore ideas around the penalization of aggressive
headline changes. That is, if an article received 10K retweets \emph{before} a
significant headline change, is it appropriate for that article to keep all the 
clout that the previous title generated? Penalizing large changes has the potential
to act as a deterrent of unwanted publishing behavior and encourage publishers to
be more considerate about their content choices \emph{before} an article is published.

%\vspace{-1cm}

==> chapter3-TitleModification/deprecate/methodology.tex <==
\section{Dataset Preparation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{Figures/publishers.pdf}
    \caption{News publishers chosen based on their political bias and
    Alexa ranking.}
    \label{fig:newsPublishers}
    \vspace{-5mm}
\end{figure}


\label{sec:data_prepare} 
In this section, we discuss our process for selecting news publishers
to include in our study. We then describe the infrastructure we designed and implemented
to capture news articles, as well as detect post-publication headline changes and measure the spread of news on social media. 


\subsection{News Publisher Identification}

Prior to capturing and studying post-publication article headline changes,
we must first identify a set of news publishers to collect article data
from that are representative of a broad range of audiences, biases, and 
platform sizes.
To this end, we constructed a set of news publishers by first consulting
the Media Bias Chart created by Ad Fontes Media~\cite{mediaBiasChart}.
This chart maps news publishers onto a two-dimensional plane representing
political bias, and reputability. We focus only on the political bias of
each news publisher, selecting an equal number of publishers from each 
region of this axis. 

% Prior to capturing and analyzing the phenomenon of news article title
% changes, we first had to identify a set of news publishers to collect
% article information from, that represent a broad range of audiences,
% biases, and platforms. Doing so would allow us to determine which kinds
% of news agencies are more likely to modify the titles of the articles
% they publish.



\begin{figure*}[ht]
\centering
    \includegraphics[width=0.95\textwidth]{Figures/architectureDiagram.pdf}
    \caption{The overview of news crawling infrastructure}\label{fig:infraArchitecture}
\end{figure*}


Rather than utilize the reputability ranking of each
publisher on this chart, we opt instead to measure reputability with the 
Alexa ranking~\cite{alexarankings} of each publisher's website. We reason that the Alexa ranking
of each publisher is an effective and unbiased proxy for a publisher; with
more reputable publishers drawing a larger audience and higher rank. We group
publishers into buckets representing different Alexa rank ranges aiming for 
an equal number of publishers from each bucket. 
Figure~\ref{fig:newsPublishers} shows the news publishers we chose, and 
their positions in the two-dimensional plane we described.



\subsection{Data Collection Infrastructure}



% To this end, we choose news sources based on the Media Bias Chart created
% and maintained by Ad Fontes Media~\cite{mediaBiasChart}. This chart maps
% news publishers on a 2D-axis representing political bias (from left to right), 
% and reputability. For our purposes, we focus only on the political bias 
% of each publisher, selecting an equal number of publishers from both left
% and right political biases. Rather than use the reputability ranking of each
% publisher from this chart, we opt instead to measure reputability by the Alexa
% ranking of each publisher website. We reason that the reputability of each
% publisher will be represented by it's Alexa rank, with more reputable websites
% bubbling up the rankings over time. We group news publisher websites into 
% buckets depending on their Alexa ranking. Figure~\ref{fig:newsPublishers}
% shows the news publishers we chose, and their positions in the 2D grid we
% described.

% In addition to selecting news publisher to study, we also choose which article
% categories to collect in order to study the effect of topic on title change
% frequency. Thus, we decide upon three categories we hypothesize will
% contain the greatest number of title changes: Politics, Business, Entertainment,
% and Technology; and a control group that we do not expect to contain many title
% changes, but will be used to compare to the other topic groups: Family.


To measure the extent in which news publishers modify the titles of their articles
post-publication, we created a data collection infrastructure that visits the
web pages of news articles as they are posted and continually monitors them 
to detect changes to their titles and content. Additionally this infrastructure monitors the spread of news on Twitter.
%Additionally this infrastructure monitors the spread of misinformation on Twitter due to the title changes of linked articles.


\noindent\textbf{Post-publication Article Headline Changes} Figure~\ref{fig:infraArchitecture} provides an overview of our infrastructure.
(i) News article URLs are collected using a set of input modules corresponding to the
source in which the URLs are gathered from. For all news publishers we study, URLs
are collected using the RSS feeds provided by each publisher. However, our
infrastructure can be easily extended to support additional URL sources, such as
scraping the home page of a news publisher, by creating a new module for that source.
Our RSS module queries the RSS servers of each news publisher periodically to gather the
URLs of new articles shortly after they are posted.

The URLs for each new article are placed onto a queue in the article crawling module (ii)
where workers consume new URLs by visiting each URL and parsing metadata from the article
web page. We collect and save each HTML web page for future processing, but specifically
parse out the article title using the Python Newspaper library~\cite{python-newspaper}.

In order to detect title changes in news articles, (iii) we recrawl each article web page periodically for the two days following its original publication and parse out the same information as previously described. We arrived at this two-day threshold via a pilot crawling experiment where we established that any headline modifications were typically occurring in the first few hours after an article was published.

\noindent\textbf{Measuring the Spread of News on Twitter} In many cases, modifications to news articles occur \emph{after} these articles have already been consumed and shared. Social media platforms only exacerbate this problem due to the speed in which information propagates among users. 
We chose to study the propagation of news on Twitter because, unlike other social media platforms, Twitter prevents users from editing tweets after they are posted, leading to discrepancies in the information shared in the tweets of news agencies, and their related articles.
When crawling an article found to have a modified title, our infrastructure also searches the Twitter feed of the
relevant news publisher for a tweet containing a link to the article in question. If such a tweet is discovered, it is
recrawled at the same interval as the article itself. For each crawl of a tweet, our infrastructure records the tweet text, as well as the current number of favorites and retweets.
To measure the base level of interaction tweets from each news publisher receive, our data collection infrastructure also crawls a random sample of tweets from each publisher.
%Our infrastructure periodically crawls a random sample of tweets from each news publisher's twitter accounts, the crawler records the tweet text, along with the current number of favorites and retweets. 

%From that point on, each time the article is re-crawled, the tweet associated with that article is re-crawled as well.

% Thus, when the article crawling module detects that an article has produced a title change, 
% the article URL is added to a queue in the Twitter crawling module (iv). This module searches
% the timeline of the Twitter account associated with the article's news publisher and associates
% a tweet to the article if it contains a link to that article. The crawler records the tweet text,
% along with the current number of favorites and retweets. From that point on, each time the article
% is re-crawled, the tweet associated with that article is re-crawled as well.

% In addition to crawling the tweets associated with articles that had a title change, our
% infrastructure also periodically crawls a random sample of tweets from each news publisher's twitter
% accounts that are not associated with title changes. This group of tweets serves as a control group
% in which we can use to compare to the reach of tweets containing misinformation.




==> chapter3-TitleModification/deprecate/related_work.tex <==


\section{Related Work}
\label{sec:related_work}
A genuine news headline summarizes the content and enables readers to draw quick conclusions~\cite{rieis2015breaking, ifantidou2009newspaper, dor2003newspaper}. However, in the digital media era, false information or fake news~\cite{fazio2020pausing,shu2017fake, kumar2018false, zhou2019fake} threatens the public's information consumption by inducing readers with clickbait headlines and fabricated content. \citet{vargas2020detection} developed techniques to distinguish legitimate activity on Twitter from disinformation campaigns using coordination network analysis.
Additionally, a large research line \cite{zhou2019fake, reis2019supervised, karimi2018multi, golbeck2018fake} focus on fake news detection, satire detection\cite{rubin2016fake, de2018attending}, and clickbait detection~\cite{potthast2016clickbait}. \citet{hounsel2020identifying} proposed methods to discover disinformation websites using characteristics of their hosting infrastructure. 
In this work, we investigate news outlets that, in the process of publishing legitimate articles, modify their headlines.
%Some news articles may alter headlines after attracting a large enough audience. There is few study on the reasons behind new headline modifications.

The headline modifications may be harmless (e.g., updating competition score) or malicious (e.g., making the headline clickbaity~\cite{blom2015click}, or starting with an inaccurate headline that maximizes user views and eventually changing it to an accurate one). Hagar and Diakopoulos~\cite{hagar2019optimizing} discussed A/B  testing on news headlines and gather audiences' feedback on several headline writing practices (e.g., starting headlines with "why" or "how" and subjective ideals) and reported that headlines are optimized for specific metric (e.g., click-through rate) from A/B testing. \citet{kuiken2017effective} investigated the effectiveness of headlines by comparing click-through rate of the original title and its of the rewritten one, suggesting that clickbait features led to statistically significant increase in number of clicks.  However, the size of their dataset was limited, with 1,836 pairs of headlines that were rewritten from a single groups of editors.  

%\cite{molyneux2020aggregation} clickbait may lower perceptions of credibility and quality

Another related research line is text edit classification. Previous work \cite{daxenberger2013automatically} analyzed linguistic features for the task of edit category classification, organizing English Wikipedia's edits into 21 categories, from spelling corrections to vandalism. \citet{yang2017identifying} investigated the intentions behind text edits and created a 13-category taxonomy of edit intentions, then developed supervised learning models for automatic identification. Similarly, \citet{yin2018learning, marrese2020variational} employed encoder-decoder deep learning framework to learn the edit representation and predict its categories. Due to data availability, previous research mainly focus on Wikipedia post-edit instead of news headlines. Given our unique, large-scale dataset of 41K pairs of title changes, we aim to understand real-world headline modifications and derive a taxonomy for automated edit categorizations. In addition, we analyze the speed of news propagation over social networks, how they relate to post-publication headline changes, and offer guidance on the timings of responsible post-publication modification.

%Wikipedia - neutral point of view. not news headline. preventing vandalism editing. They collect data from Wikipedia edit history, and extract those edits containing explicit signal words (e.g, \textit{NPOV}) in the edit comments. 


%\noindent{\textbf{Journalism: Headline modification}}


%\noindent{\textbf{Clickbait and Click-through Rate}}


%\noindent{\textbf{Edit changes classification}}



==> chapter3-TitleModification/deprecate/title_change.tex <==


% tell total tracked number by each agency. (table of total  and sub-total )
% how long is a news title? (histogram)
% how many changed pairs detect? how many unique title changes? (combine with the table above)
% how about edit distance by news agency and overall. 
\section{Post-Publication Headline Changes}\label{sec:results}

Using our data collection infrastructure, we monitored 411,070 articles published by the news agencies listed in Figure~\ref{fig:newsPublishers}
from \dataCollectionStart{} to \dataCollectionEnd{}.
In total, we observed \numArticlesWithTitleChange{} (7.5\%) articles modify their headlines at least once, resulting in \datasetSize{} changed pairs\footnote{We consider one pair as two consecutive headline versions. Additionally, we list news categories of changed pairs per agency in Table \ref{tab:in_changed_news_cate_ratio_agency} in Appendix}. 
Figure~\ref{fig:news_edit_dist_change_timing} shows that over 90\% of changes occur within the first 10 hours after publication.
Readers who encounter an article shortly after publication will likely come away with a different opinion on the subject-matter than a reader
who encounters the same article after the headline has changed. Furthermore, if the headline change is to correct invalid information,
this can lead to rapid spread of misinformation through channels such as social media. In this section, we explore the magnitude of headline
changes in our dataset, assign labels to these changes corresponding to the nature of the modification, and compare the consistency of
headlines published by popular news outlets.
%Additonally, we present the percentage of the tracked news category and modification ratio in Table \ref{tab:in_changed_news_cate_ratio_agency} in appendix.

%In the following section, we discuss the general characteristics post-publication headline modifications, including the

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=0.5\textwidth]{Figures/fig_token_length_hist.pdf}
%    \caption{Length of the news titles (in token). Histogram (\textit{left}) shows that most titles are around 10-token long. CDF(\textit{right}) shows that approx. 95\% titles are shorter than %20 tokens.  }
%    \label{fig:news_title_length}
%\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/fig_edit_length_time_hist.pdf}
    \caption{Edit distance histogram (\textit{top}): a large fraction of edits are local edits with distance 1 to 3. Timing of title changes (\textit{bottom}): Most title changes occur within 10 hours after initial publishing. We present plots per publisher in Figure~\ref{fig:edit-time-per-agent} in the appendix.}
    \label{fig:news_edit_dist_change_timing}
\end{figure}

% assign credibility to the news agency by what kind of editing and how often they apply? 
% correlation with some public news agency credibility score? 
\subsection{Headline Change Magnitude}
\label{edit-dis-1}

The inclusion, exclusion, or modification of a single word or phrase in a headline can lead to large differences in reader perception. 
Figure~\ref{fig:news_edit_dist_change_timing} shows the edit distance of headline modifications we detected during our data collection period. 
In the context of headline modifications, we define a token as a single word. We observe a bi-modal distribution in our dataset, with a majority of headline changes resulting in an edit
distance of a single token, and a second local peak at approximately 10 tokens. Since we expect headline modifications in these two groups to be the result
of distinct contributing factors, we discuss them separately.%\todo{add other category}


%d1-only  (6036, 48)
%d1-replace-only: (3767, 48)

\noindent\textbf{Single-token Edit Distance.}
During our data-collection period, we observed 6,036 single-token edit changes. Among them, 3,767 are word substitution. Table~\ref{table:d1_pos_tag_change} shows the top five most common part-of-speech (POS) changes in headlines . 
We find that headlines with single-token substituted typically correspond to either updates of ongoing events, or error corrections. 

\begin{table}[ht]
\caption{The top-5 changes in part of speech}
    \label{table:d1_pos_tag_change}
    \centering
    \scalebox{1.0}
{
\begin{tabular}{l|r}
\toprule
POS Changes &  \# \\
\midrule
(NOUN, NOUN)   &         861 \\
(VERB, VERB)   &         573 \\
(NUM, NUM)     &         396 \\
(PUNCT, PUNCT) &         242 \\
(ADJ, ADJ)     &         216 \\
Others           &       1,479\\
% (PART, PART)   &         183 \\
% (PROPN, PROPN) &         172 \\
% (ADP, ADP)     &         118 \\
% (NOUN, VERB)   &          90 \\
% (ADJ, NOUN)    &          73 \\
% (VERB, NOUN)   &          69 \\
% (AUX, AUX)     &          69 \\
% (NOUN, PROPN)  &          59 \\
% (NOUN, ADJ)    &          51 \\
% (PROPN, PRON)  &          44 \\
\bottomrule
\end{tabular}}
\end{table}

Specifically for word substitution, 44.1\% of noun changes and 54.6\% of verb changes are synonyms, hyponymns, hypernymns, or otherwise share the same lemma.
Tables~\ref{tab:noun_changes} and~\ref{tab:verb_changes} in the appendix list these breakdowns for nouns and verbs, respectively. These modifications typically occur at the end of a newsworthy event; with modified verbs transitioning from present to past tense, indicating the end of the event.
Similarly, changes in headlines correspond to updates in ongoing events (e.g. score changes in sporting events). We observe that
68.39\% of numerical headline changes result in the number increasing by some value (e.g. reflecting more discovered injuries/casualties from an ongoing 
natural disaster). Table~\ref{tab:numerical_changes} in the appendix shows the full breakdown of all numerical changes we observed.

% 396 numbers -> 231 recognizable -> 158 increased


\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/fig_edit_bert_score_stats.pdf}
    \caption{Figure \textit{(left)}: BERTScore decreases as more edits being applied until the  pre/post-edit titles become irrelevant (BERTScore reaches to 0).  Figure \textit{(right)} shows that there is only few complete rewrite in news titles. }
    \label{fig:bertscore_stats}
\end{figure}

\noindent\textbf{Arbitrary Edit Distance.}\label{edit-dis-arbitrary}
To model headline modifications of arbitrary edit distance, we compute the difference of lexicon in changed pairs to distinguish whether it is a minor update or a complete rewrite. 
BERT-based word alignment score --\textit{BERTScore}~\citep{zhang2019bertscore} as defined in Eq.\ref{eq:bertf1} -- is a lexical alignment statistic using contextual word embeddings with attention mechanism. BERTScore can capture the semantic similarity in two sentences of dissimilar structures and lexicons, whereas an edit distance only measures superficial lexical differences.
We extend our analysis to all changed pairs with $BERTScore_{F1}\in [-1,1]$ as the semantic similarity measure. 
The relationship between edit distance and $BERTScore_{F1}$ is shown in Figure~\ref{fig:bertscore_stats}~\textit{(left)}.
%The overall statistics of $BERTScore_{F1}$ is shown in Figure \ref{fig:bertscore_stats} \textit{(left)}.

\begin{equation}
\begin{aligned}
    R = \frac{1}{|x|} \sum_{x_i \in x} {max_{\hat{x_j} \in \hat{x} } x_i \hat{x}_j  } &;\ \ 
    P = \frac{1}{|\hat{x}|} \sum_{\hat{x_j} \in \hat{x}} {max_{x_i \in x } x_i \hat{x}_j  } \\
    BERTScore_{F1} &=  2\frac{P*R}{R+P} \in [-1, 1],  
\end{aligned}
\label{eq:bertf1}
\end{equation}  where $x_i,\hat{x_i}$ denote $i^{th}$ token in two sentences $x,\hat{x}$. 





% \begin{figure}[htbp]
%     \centering
%     \subfloat[BERTScore vs. Edit Distance.\label{fig:bertscore_lev_dist}] {\includegraphics[width=0.126\textwidth]{Figures/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_edit_bertscore_errorbar.pdf}}\hfill
%     \subfloat[PDF \label{fig:bertscore_hist}] {\includegraphics[width=0.13\textwidth]{Figures/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_BERTScore_hist.pdf}}\hfill
%     \subfloat[CDF\label{fig:bertscore_cdf}] {\includegraphics[width=0.13\textwidth]{Figures/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_BERTScore_cdf.pdf}}\hfill
%     \caption{Semantic similarity between changed title pairs. The peak in Figure \ref{fig:bertscore_hist} shows that the most common changes are minor updates. Figure \ref{fig:bertscore_cdf} shows that there is only few complete rewrite in news titles. }
%     \label{fig:bertscore_stats}
% \end{figure}

%Figure \ref{fig:bertscore_lev_dist} shows the semantic similarity (BERTScore) against word-level edit distance. As we expected, semantic similarity keeps decreasing as more edits are applied. 
Figure~\ref{fig:bertscore_stats}~\textit{(right)} shows the distribution of BERTScore where the peak around 0.9 indicates that most edits do not change the semantic meaning of the headline, 
%(like the examples in Table \ref{tab:numerical_changes}), 
while the samples centered around 0 represent the post-publication edit completely changing the headline's semantic meaning. We present examples associated with BERTScore in Table~\ref{tab:category-example} of the appendix.
Using a BERTScore threshold of 0.25, we find approximately 10\% of the changed pairs in our dataset are significantly rewritten. 
%More examples of various BERTScore is in Table \ref{tab:category-example} in Appendix.
%\footnote{We present examples of various BERTScore in Table \ref{tab:category-example} in Appendix.}
We consider these headline changes to be the most damaging to readers as it is very likely that the message conveyed by the headline will change drastically after modification. 


\begin{table}[ht]
    \centering
    \caption{The statistics of semantic similarity (BERTScore) by agency (Ranked by the mean value). To clarify the similarity rankings from news reputation rankings, the ordered list does not reflect credibility. \textit{Tracked} is the total number of tracked articles, \textit{Mod. Ratio} is the percentage of the articles with at least one altered headline.}
    \label{tab:bertscore_agency}
    \vspace{-1ex}
%\hspace*{-25pt}
% copy from: tab_bertscore_by_agency.tex
    \begin{tabular}{lrrrr}
    \toprule
    Agency &   Mean &     Median &    Tracked &  Mod.Ratio \\
    \midrule
    Huffington Post & 0.8292 &  0.8966 &    4,875 &         0.0357 \\
    The Epoch Times & 0.8260 &   0.8908 &    4,765 &         0.1442 \\
    The Hill        & 0.8087 &   0.8644 &    5,676 &         0.0592 \\
    Fox News        & 0.7659 &   0.8645 &   11,003 &         0.0486 \\
    New York Post   & 0.7305 &   0.8174 &   13,881 &         0.0665 \\
    National Review & 0.7268 &   0.8305 &    3,324 &         0.0126 \\
    The Blaze       & 0.7200 &   0.8145 &    4,401 &         0.0400 \\
    CNN             & 0.6888 &   0.7493 &    6,344 &         0.2030 \\
    Washington Post & 0.6840 &   0.7916 &    6,076 &         0.1508 \\
    Newsmax         & 0.6733 &   0.7319 &    1,115 &         0.0233 \\
    Daily Beast     & 0.6584 &   0.7693 &    4,359 &         0.1308 \\
    MarketWatch     & 0.6551 &   0.7011 &    7,503 &         0.3453 \\
    BBC             & 0.6031 &   0.6260 &    5,854 &         0.2277 \\
    Yahoo News      & 0.5985 &   0.6160 &  227,246 &         0.0846 \\
    Daily Mail      & 0.5936 &   0.6348 &   75,118 &         0.0756 \\
    OAN             & 0.5830 &   0.5910 &    8,323 &         0.2616 \\
    The Guardian    & 0.5579 &   0.5826 &    6,916 &         0.1975 \\
    New York Times  & 0.5234 &   0.5595 &    9,746 &         0.1892 \\
    BuzzFeed        & 0.5085 &   0.4872 &    4,545 &         0.4438 \\
    \bottomrule
\end{tabular}
\vspace{-2ex}
\end{table}

\xingzhiswallow{
\begin{table}[t]
\small
    \centering
    \caption{The statistics of semantic similarity (BERTScore) by agency (Ranked by the mean value). To clarify the similarity rankings from news reputation rankings, the ordered list does not reflect credibility.}
    \label{tab:bertscore_agency}
\hspace*{-25pt}
% copy from: tab_bertscore_by_agency.tex
    \begin{tabular}{lrrrrr}
    \toprule
    Agency &   Mean &   Std. &  Median &    Tracked &  Mod.Ratio \\
    \midrule
    Huffington Post & 0.8292 & 0.1730 &  0.8966 &    4,875 &         0.0357 \\
    The Epoch Times & 0.8260 & 0.1740 &  0.8908 &    4,765 &         0.1442 \\
    The Hill        & 0.8087 & 0.1826 &  0.8644 &    5,676 &         0.0592 \\
    Fox News        & 0.7659 & 0.2310 &  0.8645 &   11,003 &         0.0486 \\
    New York Post   & 0.7305 & 0.2424 &  0.8174 &   13,881 &         0.0665 \\
    National Review & 0.7268 & 0.2660 &  0.8305 &    3,324 &         0.0126 \\
    The Blaze       & 0.7200 & 0.2758 &  0.8145 &    4,401 &         0.0400 \\
    CNN             & 0.6888 & 0.2531 &  0.7493 &    6,344 &         0.2030 \\
    Washington Post & 0.6840 & 0.2778 &  0.7916 &    6,076 &         0.1508 \\
    Newsmax         & 0.6733 & 0.2714 &  0.7319 &    1,115 &         0.0233 \\
    Daily Beast     & 0.6584 & 0.2915 &  0.7693 &    4,359 &         0.1308 \\
    MarketWatch     & 0.6551 & 0.2608 &  0.7011 &    7,503 &         0.3453 \\
    BBC             & 0.6031 & 0.2671 &  0.6260 &    5,854 &         0.2277 \\
    Yahoo News      & 0.5985 & 0.2801 &  0.6160 &  227,246 &         0.0846 \\
    Daily Mail      & 0.5936 & 0.2741 &  0.6348 &   75,118 &         0.0756 \\
    OAN             & 0.5830 & 0.2590 &  0.5910 &    8,323 &         0.2616 \\
    The Guardian    & 0.5579 & 0.2896 &  0.5826 &    6,916 &         0.1975 \\
    New York Times  & 0.5234 & 0.3283 &  0.5595 &    9,746 &         0.1892 \\
    BuzzFeed        & 0.5085 & 0.2529 &  0.4872 &    4,545 &         0.4438 \\
    \bottomrule
\end{tabular}
\vspace{-5ex}
\end{table}
}


%We breakdown the title changes by news agency, and measure which agency changes their news titles more significantly. 
Table~\ref{tab:bertscore_agency} shows the ordered list of news agencies by the average similarity score across all changed headlines. Generally, higher similarity indicates minor changes that do not alter the original semantic meaning. 
%In Table \ref{tab:bertscore_agency}, the "notorious" \textit{BuzzFeed} \footnote{\textit{BuzzFeed} is well-known for eliciting users' 
%attention in a clickbaity way.} is ranked last, which is consistent to our consensus. 
We find many well-regarded publishers (e.g., BBC, The Guardian, NYT) frequently modify headline semantics. This unexpected finding suggests that the popularity of a news outlet does not necessarily indicate greater restraint with post-publication headline changes. Contrastingly, we observe publishers such as The Epoch Times with an Alexa rank of close to ten thousand modify headlines at a much lower rate than publishers with a much larger online presence. 

Additionally, by noting the ratio of modified headlines with the average BERTScore for all modified headlines, we can deduce the
expected consistency of a particular news outlet. For instance, we find that BuzzFeed modified the headlines of 44\% of their articles during our data-collection period. Of those articles, we observe the headline changes produce the lowest average BERTScore (i.e. the modified headlines depart significantly from the original ones). Contrastingly, during our data collection period, The Huffington Post only modified the headlines of 3\% of observed articles; achieving the highest
average BERTScore with those changes. We can therefore conclude that, in terms of headline modifications, The Huffington Post is a more consistent news outlet compared to BuzzFeed. We note however, that this consistency of headlines does not necessarily imply accuracy of headlines.

%Table~\ref{tab:lowbert_example} shows the title examples of low similarity from different agencies. We observe that news agencies change 
%writing style or emphasize different content when rewriting the titles, which may give readers different first impressions. 
% \begin{quote}
% Before: "\textit{Hancock defends India travel ban delay as Covid variant cases mount} "\\
% After: "\textit{Hancock: most Bolton Covid patients eligible for jab but haven’t had it}" \\
% Similarity: 0.067
% \end{quote}
%For example, Although the news topic of the pair from \textit{The Guardian} in Table~\ref{tab:lowbert_example} does not change, the original title emphasizes on the action \textit{defend}, while the edited version emphasizes on vaccination rate. The shift of title
%s focus may greatly change based on editor's judgement. % \todo{add some reference here}.
%Table~\ref{tab:change_category_by_agency} shows the percentage of edit types that each agency applied. We found that BBC has significantly higher ratio of dynamic update, reflecting their strong %ability to report and update.


\subsection{Categorization of News Title Changes}




\begin{table*}[ht]
    \centering
    \small
    \caption{Examples of the altered titles sampled from our dataset by the modification category. The example of the label "Other" involves out-of-vocabulary words (J.\&J) and changes in tone. The example of "Concision" removes the specific person, while the "Elaboration" example expands the original title with an attributive clause. "Forward-Reference" adds a question mark and "Personalization" substitute reader into the title, which both trigger curiosity from the readers. The "Neutralize" example remove \textit{"long"} from the original title, making it less subjectivity. While "Emotional" example adds \textit{"tease, big"}, which makes the title more inflammatory.  }
    \label{tab:category-example-mainbody}
    \scalebox{1.0}{
% \begin{tabular}{>{\raggedright\arraybackslash}p{0.35\textwidth} >{\raggedright\arraybackslash}p{0.35\textwidth} >{\raggedleft\arraybackslash}p{0.1\textwidth}>{\raggedleft\arraybackslash}p{0.1\textwidth}}
\begin{tabular}{p{0.4\textwidth}p{0.4\textwidth}p{0.05\textwidth}p{0.09\textwidth}}
\toprule
                                                                                        Before &                                                                                                             After &  BERT-F1 &       Label \\
\midrule
One Dose of J.\&J. Vaccine Is Ineffective Against Delta... &	J.\&J. Vaccine May Be Less Effective Against Delta ... & 0.6830 & Other \\
% Nike chief executive says firm is 'of China and for China'	&Nike boss defends firm's business in China & 0.4559 & Other \\
                                           Senator Capito says Republicans plan new US infrastructure offer &                                                                          U.S. Senate Republicans prepare new infrastructure offer &         0.5434 &   Concision \\
                                           Raul Castro confirms he's resigning, ending long era in Cuba &                                                                        Raul Castro resigns as Communist chief, ending era in Cuba &         0.7310 &  Neutralize \\
                                        Fourth stimulus check update: Your next payment could be these &                                                                 Fourth stimulus check? These payments are already in the pipeline &         0.4479 & Forward Ref. \\
                                                        The Latest: UN: 38,000 Palestinians displaced in Gaza &                                                                         The Latest: Biden expresses 'support' for Gaza cease-fire &         0.4043 &  Dyn. Update \\

MAGA 2.0&	“A new bargain”: Biden’s 2024 tease bets big on nostalgia & 0.0257 & Emotional \\
                                                                               23 Amazing Jokes From Hot Fuzz &                                                      23 Jokes From "Hot Fuzz" That Humans Will Laugh At For The Next 10,000 Years &         0.4715 & Elaboration \\
                                            %   Suspect arrested following series of Arizona traffic shootings &                                                     Arizona gunman goes on traffic shooting rampage, leaving one dead, 12 injured &         0.2247 &   Emotional \\
                                                 Watch Jeff Bezos’ ‘Blue Origin’ launch into space live today &                                                Everything you need to know as Jeff Bezos’ ‘Blue Origin’ launches into space today &         0.6179 & Personalize \\
                  Afghan guard killed: Firefight leaves at least one dead and others injured at Kabul airport &                  'It would be better to die under Taliban rule than face airport crush', say US embassy's 'betrayed' Afghan staff &         0.0656 &    Citation \\
\bottomrule
\end{tabular}
}
\end{table*}



% \subsection{Taxonomy of Editing Categories}
To discover trends in article headline changes, and the behaviors of the publishers responsible, we create a nine-class taxonomy of editing types based on journalism knowledge (e.g. Emotionalism, etc.), existing taxonomies for Wikipedia edits\cite{daxenberger2013automatically, yang2017identifying}, and the most common edits from our observations (e.g., Paraphrase, Dynamic update, etc.) . 
We design our taxonomy as follows:
%\textbf{Taxonomy Creation Pipeline}: 
\begin{itemize}
    \item \textbf{Paraphrase:} We assign the label \textit{Paraphrase} if the changed pairs have a similarity score (BERTScore-F1) greater than 0.8.
    \item \textbf{Dynamic Update:} If both old and new title contain keywords such as \textit{Monday brief, update, live, stream, etc}. The keywords were manually selected. 
    \item \textbf{Emotionalism\cite{kilgo2016six}:} if only the news title contains any of words in the subjective dictionary. 
    \item \textbf{Neutralization:} if only the old title contains subjective words mentioned above.
    \item \textbf{Forward Reference:} Forward Reference\cite{blom2015click, kilgo2016six} is a common feature in news titles, piquing reader curiosity. We assign this label only if the changed title contains the keywords such as \textit{why, when, which, how, etc.}
    \item \textbf{Personalization\cite{kilgo2016six}:} Personalization is used to retain audiences and make the readers feel involved in the news. We assign this label only if the new title contains keywords such as \textit{you, we, s/he, your, etc.}
    \item \textbf{Citation:} Citation is a common technique in news headlines that make them look more reliable. We assign this label only if the new title contains keywords like \textit{said, says, told, etc.}
    \item \textbf{Concision:} If the new title removes some text, and the remaining text aligns with the old title (P $< 0.6$, R $>0.5$). BERT-Score Precision/Recall is defined in Eq.\ref{eq:bertf1}
    \item \textbf{Elaboration:} If the new title adds text, and is semantically aligned with the old title: P $> 0.6$, R $< 0.5$). 
\end{itemize}


\begin{figure}[t]
    \centering
    % \subfloat[Histogram of Editing Categories.  \label{fig:category_stats_1}] {\includegraphics[width=0.2\textwidth]{Figures/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_edit_category.pdf}}\hfill
    % \subfloat[Coverage Assigned Category  \label{fig:category_stats_2}] {\includegraphics[width=0.2\textwidth]{Figures/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_edit_category_coverage.pdf}}
    \includegraphics[width=1.00\columnwidth]{Figures/fig_modif_label_stats.pdf}
    \caption{Assigned category statistics. Figure (\textit{left}) shows the majority change types are paraphrase and dynamic update. Figure (\textit{right})  shows that approx. 70\% of samples have at least one category assigned.  50.3\% modifications associate with benign edit categories (paraphrase, updates, elaboration, concision), while 23.13\% modifications are linked with the other less benign edits. }
    \label{fig:category_stats}
\end{figure}

\begin{table*}[t]
\caption{The breakdown of edit types per news agency. Each headline modification may belong to multiple labels. We highlight the top one in each column.}
\label{tab:change_category_by_agency}
\centering
%\hspace*{-30pt}
\begin{tabular}{lp{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.06\textwidth}}
\toprule
Agency &  Paraphrase &  Dynamic Update &  Elaboration &  Concision &  Emotional &  Neutralize &  Forward Reference &  Personalize &  Citation  \\
\midrule
BBC             &      0.3196 &      0.3848 &       0.0278 &     0.0113 &     0.1043 &      0.0818 &       0.0180 &       0.0188 &    0.0540  \\
BuzzFeed        &      0.1587 &      0.0203 &       0.0312 &     \textbf{0.1101} &     0.1026 &      \textbf{0.1894} &       \textbf{0.0709} &       \textbf{0.0699} &    0.0238  \\
CNN             &      0.4262 &      0.0916 &       0.0404 &     0.0148 &     0.0699 &      0.0738 &       0.0171 &       0.0342 &    0.0435 \\
Daily Beast     &      0.4754 &      0.1035 &       0.0246 &     0.0175 &     0.1123 &      0.0912 &       0.0386 &       0.0351 &    0.0298  \\
Daily Mail      &      0.2801 &      0.1158 &       0.0357 &     0.0144 &     0.0993 &      0.1218 &       0.0241 &       0.0521 &    0.0422  \\
Fox News        &      0.6056 &      0.1925 &       0.0187 &     0.0093 &     0.0710 &      0.0617 &       0.0168 &       0.0224 &    0.0262  \\
Huffington Post &      \textbf{0.7356} &      0.0690 &       0.0000 &     0.0000 &     0.0345 &      0.0632 &       0.0000 &       0.0345 &    0.0230  \\
MarketWatch     &      0.3867 &      0.0872 &       0.0413 &     0.0178 &     0.0965 &      0.0799 &       0.0363 &       0.0154 &    0.0247  \\
National Review &      0.5476 &      0.3810 &       0.0476 &     0.0000 &     0.0714 &      0.0476 &       0.0000 &       0.0238 &    0.0000  \\
New York Post   &      0.5211 &      0.0997 &       0.0336 &     0.0076 &     0.0715 &      0.0618 &       0.0336 &       0.0293 &    0.0141  \\
New York Times  &      0.2923 &      0.1171 &       0.0108 &     0.0108 &     0.1123 &      0.1432 &       0.0380 &       0.0184 &    0.0331  \\
Newsmax         &      0.3846 &      0.3077 &       0.0385 &     0.0000 &     0.0000 &      0.0769 &       0.0000 &       0.0000 &    0.0385  \\
OAN             &      0.2692 &      0.0156 &       0.0280 &     0.0184 &     0.1029 &      0.0988 &       0.0032 &       0.0023 &    0.0271  \\
The Blaze       &      0.5341 &      0.3239 &       \textbf{0.0625} &     0.0227 &     0.0682 &      0.0398 &       0.0227 &       0.0398 &    0.0455  \\
The Epoch Times &      0.6856 &      0.1659 &       0.0146 &     0.0204 &     0.0277 &      0.0422 &       0.0044 &       0.0087 &    0.0364  \\
The Guardian    &      0.2950 &      \textbf{0.4100} &       0.0271 &     0.0124 &     \textbf{0.1215} &      0.1164 &       0.0190 &       0.0190 &    \textbf{0.0688} \\
The Hill        &      0.6637 &      0.2024 &       0.0268 &     0.0327 &     0.0208 &      0.0446 &       0.0089 &       0.0060 &    0.0179 \\
Washington Post &      0.4891 &      0.2205 &       0.0186 &     0.0109 &     0.0884 &      0.0797 &       0.0207 &       0.0437 &    0.0371  \\
Yahoo News      &      0.3256 &      0.1846 &       0.0150 &     0.0126 &     0.1047 &      0.0977 &       0.0156 &       0.0161 &    0.0340  \\

\bottomrule


\end{tabular}
\end{table*}

\xingzhiswallow{
\begin{table*}[t]
\caption{The breakdown of edit types per news agency. We highlight the top one in each column.}
\label{tab:change_category_by_agency}
\small
\centering
\hspace*{-30pt}
\begin{tabular}{lp{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.06\textwidth}p{0.08\textwidth}}
\toprule
Agency &  Paraphrase &  Dynamic Update &  Elaboration &  Concision &  Emotional &  Neutralize &  Forward Reference &  Personalize &  Citation &  \#Changed \\
\midrule
BBC             &      0.3196 &      0.3848 &       0.0278 &     0.0113 &     0.1043 &      0.0818 &       0.0180 &       0.0188 &    0.0540 &    1333 \\
BuzzFeed        &      0.1587 &      0.0203 &       0.0312 &     \textbf{0.1101} &     0.1026 &      \textbf{0.1894} &       \textbf{0.0709} &       \textbf{0.0699} &    0.0238 &    2017 \\
CNN             &      0.4262 &      0.0916 &       0.0404 &     0.0148 &     0.0699 &      0.0738 &       0.0171 &       0.0342 &    0.0435 &    1288 \\
Daily Beast     &      0.4754 &      0.1035 &       0.0246 &     0.0175 &     0.1123 &      0.0912 &       0.0386 &       0.0351 &    0.0298 &     570 \\
Daily Mail      &      0.2801 &      0.1158 &       0.0357 &     0.0144 &     0.0993 &      0.1218 &       0.0241 &       0.0521 &    0.0422 &    5681 \\
Fox News        &      0.6056 &      0.1925 &       0.0187 &     0.0093 &     0.0710 &      0.0617 &       0.0168 &       0.0224 &    0.0262 &     535 \\
Huffington Post &      \textbf{0.7356} &      0.0690 &       0.0000 &     0.0000 &     0.0345 &      0.0632 &       0.0000 &       0.0345 &    0.0230 &     174 \\
MarketWatch     &      0.3867 &      0.0872 &       0.0413 &     0.0178 &     0.0965 &      0.0799 &       0.0363 &       0.0154 &    0.0247 &    2591 \\
National Review &      0.5476 &      0.3810 &       0.0476 &     0.0000 &     0.0714 &      0.0476 &       0.0000 &       0.0238 &    0.0000 &      42 \\
New York Post   &      0.5211 &      0.0997 &       0.0336 &     0.0076 &     0.0715 &      0.0618 &       0.0336 &       0.0293 &    0.0141 &     923 \\
New York Times  &      0.2923 &      0.1171 &       0.0108 &     0.0108 &     0.1123 &      0.1432 &       0.0380 &       0.0184 &    0.0331 &    1844 \\
Newsmax         &      0.3846 &      0.3077 &       0.0385 &     0.0000 &     0.0000 &      0.0769 &       0.0000 &       0.0000 &    0.0385 &      26 \\
OAN             &      0.2692 &      0.0156 &       0.0280 &     0.0184 &     0.1029 &      0.0988 &       0.0032 &       0.0023 &    0.0271 &    2177 \\
The Blaze       &      0.5341 &      0.3239 &       \textbf{0.0625} &     0.0227 &     0.0682 &      0.0398 &       0.0227 &       0.0398 &    0.0455 &     176 \\
The Epoch Times &      0.6856 &      0.1659 &       0.0146 &     0.0204 &     0.0277 &      0.0422 &       0.0044 &       0.0087 &    0.0364 &     687 \\
The Guardian    &      0.2950 &      \textbf{0.4100} &       0.0271 &     0.0124 &     \textbf{0.1215} &      0.1164 &       0.0190 &       0.0190 &    \textbf{0.0688} &    1366 \\
The Hill        &      0.6637 &      0.2024 &       0.0268 &     0.0327 &     0.0208 &      0.0446 &       0.0089 &       0.0060 &    0.0179 &     336 \\
Washington Post &      0.4891 &      0.2205 &       0.0186 &     0.0109 &     0.0884 &      0.0797 &       0.0207 &       0.0437 &    0.0371 &     916 \\
Yahoo News      &      0.3256 &      0.1846 &       0.0150 &     0.0126 &     0.1047 &      0.0977 &       0.0156 &       0.0161 &    0.0340 &   19224 \\

\bottomrule


\end{tabular}
\end{table*}

}

These nine categories allow us to better understand headline modifications by classifying them into groups corresponding to their perceived purpose. 
With the combination of BERTScore, Stanza Pipeline~\cite{qi2020stanza}, word sentiment dictionary~\cite{riloff2003learning}, 
and hand-crafted rules,  we are able to automatically assign labels using our proposed NLP pipeline. We empirically determined the thresholds to use 
by finding those that made the most sense with manual inspection.  
Table~\ref{tab:category-example} of the appendix present more examples of each of these categories.
%Figure~\ref{fig:category_stats} show the histogram and coverage of the taxonomy. Each sample may have multiple categories if the headline meets the criteria for more 
%than one category (e.g., Elaboration and Emotionalism).

Figure~\ref{fig:category_stats}~\textit{(right)} shows the resulting label coverage. Our proposed categorization rules cover approximately 70\% of news title changes (the changed pair has at least one assigned category). 
Among the 30\% of modifications not covered by our pipeline, we find that the missing cases usually have a BERTScore of less than 0.8, involve more complex sentence structure changes (double negation), or out-of-vocabulary words (most of them are COVID-related “COVID-19, J.\&J., AstraZenec”, which debuted after the release of the pre-trained model). 
We listed several examples in Table \ref{tab:category-example-mainbody} and more examples in Table \ref{tab:category-example} in the Appendix.

% In Table , we show two examples of the label 'Other'.
%\todo{Why can't we categorize the other headlines?}.



 We also find that the most common changes belong to the ``Paraphrase'' and ``Dynamic Update'' categories (44.24\%), which do not significantly change the semantic meaning of the headlines. Changes in these categories typically correspond to updates of ongoing events and grammatical/spelling corrections. However, we note that all other 
categories in our taxonomy may contain headline changes that can be perceived as harmful to at least some readers.
%['lb_paraphrase_indicator', 'lb_dyn_update_indicator']
%18540 (41906,) 0.44241874671884696

Over the course of our data collection period, we observed an equal distribution of ``Emotionalism'' and ``Neutralization'' headline changes, 
suggesting that publishers are just as likely to add emotional words to attract more readers after initial publication as they are to remove them.
However, since both of these categories transition the headline from a provocative to non-provocative state, or vice-versa, these two groups can have
the same effect on different groups of readers. In the case of ``Emotionalism'' changes, readers who view a headline after it has been modified, will 
likely have a more emotional response to the subject-matter, while ``Neutralization'' changes will have the same effect on readers who view a headline pre-modification.
Together, these two groups make up 20.13\% of all headline changes in our dataset.

%['lb_emotionalism_indicator', 'lb_neutralization_indicator']
%8437 (41906,) 0.2013315515677946
Table~\ref{tab:change_category_by_agency} shows the percentage of articles by each publisher belonging to each of the nine categories in our taxonomy. 
Since it reflects the explanation of headline changes, the percentage does not reflect the general media bias, which may be embedded in the static news headlines. 
%\todo{What does this sentence mean? I thought these percentages have nothing to do with semantic similarity}
We observe that over 70\% of the articles published by the Huffington Post, The Epoch Times and The Hill belong to either the ``Paraphrase'' or ``Dynamic Update'' categories, demonstrating that their headlines will typically not change 
in ways which will lead to drastically different opinions among readers. We also notice that 
\textit{BuzzFeed} leads in three change categories, including the categories most closely related to click-bait: ``Forward Reference'', and ``Personalization''. 

% ['lb_paraphrase_indicator', 'lb_dyn_update_indicator']
% BBC 753 1333 0.5648912228057015
% BuzzFeed 347 2017 0.17203767972235995
% CNN 597 1288 0.4635093167701863
% Daily Beast 294 570 0.5157894736842106
% Daily Mail 2013 5681 0.354339024819574
% Fox News 358 535 0.6691588785046729
% Huffington Post 133 174 0.764367816091954
% MarketWatch 1112 2591 0.4291779235816287
% National Review 28 42 0.6666666666666666
% New York Post 512 923 0.5547128927410617
% New York Times 720 1844 0.39045553145336226
% Newsmax 15 26 0.5769230769230769
% OAN 601 2177 0.2760679834634819
% The Blaze 115 176 0.6534090909090909
% The Epoch Times 503 687 0.7321688500727802
% The Guardian 856 1366 0.6266471449487555
% The Hill 243 336 0.7232142857142857
% Washington Post 567 916 0.618995633187773
% Yahoo News 8773 19224 0.4563566375364128


By observing the categorizations of each publisher, a model can be developed on their overall headline-modification strategies. For instance, the ``Citation'' category
of our taxonomy allows us to deduce that \textit{The Guardian} is the most likely to include witness or expert testimony in headlines post-publication, with 6.8\% of their articles falling into that category.
Conversely, we find that the publisher National Review is very unlikely to make such a headline change as we did not observe any instances of modification by either publisher during our data collection period. These observations quantify the regularity with which publishers modify their headlines, and can be used as a supplementary feature for future research on digital journalism and public trust in news.

\subsection{News Propagation over Twitter}

In recent years, social media services have emerged as a vital tool for news publishers to quickly share stories with the public. Due to the ability of
users to share and ``repost'' links to articles with others connected to them online, information can spread faster than ever before. Because of this 
user-assisted amplification, false or misleading information in article headlines can propagate to exponentially many readers before headline changes 
occur, magnifying the negative repercussions of unanticipated headline changes. 

We track the reachability of news on Twitter in terms of user engagement. As mentioned in Section~\ref{sec:data_prepare}, our data-collection infrastructure 
records the number of likes and retweets of tweets associated with news articles with modified headlines from the accounts of each publisher. In total,
we detect 5,384 tweets corresponding to articles with modified headlines during our data collection period. We note that these tweets correspond to the
original article headlines, with their immutability preventing publishers from simply editing their contents to reflect headline changes. Rather,
publishers must first delete the original, outdated tweet, and replace it with a new tweet. Alarmingly however, we find that only 0.15\% of all such tweets 
were deleted subsequent to a headline change in the corresponding article. Moreover, we find that these tweets on average garner 39 retweets and 137 favorites. 
This means that the vast majority of tweets associated with outdated and potentially misleading information remain online indefinitely, and receive considerable
attention from users who then spread this information to others.

%In 
%Figure~\ref{fig:news_twitter_prop_time}, red curves individually represent the normalized reached population~\footnote{Scaled by the maximally 
%reached population of each news article on Twitter} versus elapsed time (hour) after the initial release. We plot the fitted function in blue solid line.
%We use a sigmoid-like function to fit the curve as plotted in blue.

Figure~\ref{fig:news_twitter_prop_time} shows the distribution of time in which tweets associated with headline changes were ``retweeted'' and ``favorited''
by users.
We observe a clear trend that news stories gradually lose popularity on social networks as they become less novel.
People usually share (retweet) tweets associated with news stories within the first ten hours and react (favorite) within first five hours. 
Based on the observations in Figure~\ref{fig:news_edit_dist_change_timing}, we found that almost 80\% title changes happened within 
the first five hours after publishing. These findings are alarming as they show that many headline changes occur \emph{after} most
social media activity regarding the particular article ceases. This means that social media users are currently either spreading false or 
misleading information before the publisher can remedy it by modifying the headline, or sharing articles that will portray an entirely
different emotional response when their followers view it at a later point in time. Both of these scenarios can lead to situations 
where different readers of the same article or headline will come to different conclusions depending on when they encountered it.

\xingzhiswallow{

\begin{figure}[t]
    \centering
    % \subfloat[retweet vs time] {\includegraphics[width=0.2\textwidth]{Figures/retweet_vs_time.pdf}}
    % \subfloat[likes vs time] {\includegraphics[width=0.2\textwidth]{Figures/like_vs_time.pdf}}
    \includegraphics[width=0.95\columnwidth]{Figures/fig_tweet_vs_time.pdf}
    \caption{The normalized retweets and likes vs news published time (red curves). The blue curve is the fitted sigmoid-like curve (Eq.\ref{eq:sigfit}), approximating how quick the news achieves its max influence. }
    \label{fig:news_twitter_prop_time}
    %The learnt parameters of retweet-model is [0.9611 2.6353 0.7282].
\end{figure}


}


\begin{figure}[!t]
    \centering
    %\vspace{-5mm}
    % \subfloat[retweet vs time] {\includegraphics[width=0.2\textwidth]{Figures/retweet_vs_time.pdf}}
    % \subfloat[likes vs time] {\includegraphics[width=0.2\textwidth]{Figures/like_vs_time.pdf}}
    \includegraphics[width=1.0\columnwidth]{Figures/fig_tweet_vs_time_vs_edit_time_25.pdf}
    \vspace{-4mm}
    \caption{The normalized retweets (top) and favorites (bottom) V.S. news published time. The solid blue curve is the fitted curve 
    $y = a \cdot (1+e^{-b(x-c)})^{-1}$
 , approximating how quick the news achieves its max influence. }
 %We find the tweets generally reach its maximal audience before the most post-edits happen, demonstrating the potential risk of misleading information propagation.  }
    \label{fig:news_twitter_prop_time}
    \vspace{-3mm}
    %The learnt parameters of retweet-model is [0.9611 2.6353 0.7282].
\end{figure}

\noindent\textbf{URL Preview Cards} A popular feature of Twitter is the rendering of 
cards that preview the content located at the URL linked in a tweet. These cards work
by parsing and rendering the Open Graph~\cite{openGraph} metadata from the HTML source of the linked webpage 
directly below the tweet text. Typically, a webpage thumbnail, title, and description are rendered.
This metadata is cached for each particular URL for approximately one week; only updating when the URL
is modified~\cite{twitterPreviewCard}. This caching behavior can amplify the negative repercussions of
post-publication headline changes as any tweet containing the URL of an article that was published prior
to a headline change will display the outdated headline for at least one week. This is a behavior we
have observed on the Twitter accounts of popular news publishers. Figure~\ref{fig:tweetCardScreenshot}
demonstrates an example of this behavior with a headline change from the BBC, along with a tweet containing
a link to the article posted by the official BBC Twitter account. Twitter users who only read the headline and description
located on the rendered card will consume outdated information on the situation, as opposed to those who click through to the
article webpage.

%  \begin{figure}[t]
%     \vspace{-0mm}
%      \centering
%      \subfloat{{\includegraphics[width=7cm]{Figures/twitterScreenshot-crop-short-2.png} }}
%      \quad
%      \subfloat{{\includegraphics[width=7cm]{Figures/bbcScreenshot-crop-short.png} }}
%      \vspace{-0mm}
%      \caption{Twitter URL preview of article posted by BBC Politics. Article headline outdated on Twitter due to caching behavior of URL cards.}
%      \label{fig:tweetCardScreenshot}
%      \vspace{-5mm}
%  \end{figure}

 \begin{figure}[t]
    \vspace{-0mm}
     \centering
     \begin{subfigure}{}
     {\includegraphics[width=7cm]{Figures/twitterScreenshot-crop-short-2.png} }
     \end{subfigure}
     \quad
     \begin{subfigure}{}
     {\includegraphics[width=7cm]{Figures/bbcScreenshot-crop-short.png} }
     \end{subfigure}
     \vspace{-0mm}
     \caption{Twitter URL preview of article posted by BBC Politics. Article headline outdated on Twitter due to caching behavior of URL cards.}
     \label{fig:tweetCardScreenshot}
     \vspace{-5mm}
 \end{figure}

%\vspace{-2cm}
% \begin{figure}[t]
%     \centering
%     \subfloat{{\includegraphics[width=5cm]{Figures/twitterScreenshot.png} }}
%     \qquad
%     \subfloat{{\includegraphics[width=5cm]{Figures/bbcScreenshot.png} }}
%     \caption{Twitter URL preview of article posted by BBC Politics. Article headline outdated on Twitter due to caching behavior of URL cards.}
%     \label{fig:tweetCardScreenshot}
%     \vspace{-5mm}
% \end{figure}

%Observation I: The information spreads fastest via retweet within the first 10 hours. \\
%Observation II:  The number of likes usually saturates within the first 5 hours.

==> chapter4-BiosModification/Chapter_prediction_from_bio.tex <==


%To demonstrate the predictive power embedded in the biography, we set up experiments for predicting gender, ethnicity, personal interests. We report the performance of various models with biography and estimate how many tweets could achieve the similar performance. 

% Model description:
% 1. Naive Bayes: See the baseline, see the important key words. (50000 1-2 gram, tf-idf weighted.) remove stop words but keep he/she, gender related words.
% 2. Avg. Emb. + Logistic regression
% 3. LSTM bio sequence
% 4. Roberta (CLS)
% 5. Roberta (Token-last layer mean) - do parameter search
% 6. BERTweet -> 

To measure the predictive power of biographies, we set up binary/multi-class classification experiments for predicting gender, ethnicity and personal interest. 
We randomly sample the users with demographics information together with one bio in year 2020, and set the demographic labels as ground-truth if the inference confidence is greater than 95\% for gender (male/female) and 50\% for ethnicity (White/Black/Hispanic/Asian).  Hashtags in the tweets are strong evidence of users' interested topics. Similar to \citet{conover2011predicting}, we select 187 representative hashtags from the most frequent ones and categorize them into 7 groups as shown in Table.\ref{tab:hashtag_category}. More than 90\% of the users only have one label assigned, so we formulate it as a multi-class prediction task. 

To compare the predictive power between biographies and tweets, we also randomly sample up to 200 tweets associated to each user. 
We anonymize bios and tweets by removing contact information (phone, email, twitter handles), then convert Emojis and hashtags into a textual form in order to preserve as much information as possible
\footnote{Emoji: Convert Emoji to text: \url{https://github.com/carpedm20/emoji/} WordNinja: Split hashtag to meaningful word segments \url{https://github.com/keredson/wordninja}. We remove selected hashtags to avoid data leak.}.

Since the original label distribution is highly imbalanced, we under-sample the majority classes to keep label balanced, resulting in a total of 229,460/12,192/14,483 samples in the task of gender, ethnicity and personal interest  respectively.


For each task, we randomly sample 80\% data for training, 10\% for validation and 10\% for testing, then report the averaged accuracy after 5 trials with the following model settings. More detail is included in Table \ref{tab:model_cofig} in Appendix.
\begin{itemize}
    \item  \textbf{Naive Bayes} : Multinomial Naive Bayes classifier with tf-idf weighted 1 to 5-gram bag-of-words features of max vocabulary size 70,000.
    %\item \textbf{AvgEmb.}: Logistic regression classifier with averaged GLoVe pre-trained Twitter word embeddings \cite{pennington2014glove}
    %\item \textbf{BiLSTM}: Two layers of Bi-directional LSTM \cite{hochreiter1997long, schuster1997bidirectional} with two linear layers for classification.
    \item \textbf{RoBerta-CLS}: Pre-trained RoBerta (\textit{roberta-base}) from HuggingFace transformer\cite{wolf-etal-2020-transformers} library. Use [CLS] embeddings from the last layer for classification. We use averaged tweets embeddings as user-level features for training and predicting. 
    %We use 2-layer linear layers with ReLU as activation function without freezing any pre-trained layer.
    %\item \textbf{RoBerta-Mean}: Similar to RoBerta-CLS, but using average token embeddings from last layer as sentence representation for classification.
    \item \textbf{BERTweet}\cite{nguyen2020bertweet}: Similar to RoBerta-CLS, but we replace the pre-trained model with \textit{BERTweet}, which was pre-trained on 850M English Tweets. 
\end{itemize}

% To train a user-level classifier from varying number of personal tweets, we extract sentence embeddings for all the tweets of a user,  use average pooling to obtain the user-level embeddings, then train the classifier for the downstream tasks. In testing phase, we use the trained classifier and feed pooled embeddings of arbitrary number of tweets from a user. 



\begin{figure*}[htbp]
    \centering
    \subfloat {\includegraphics[width=0.32\textwidth]{Figures/gender_figures/biolen_vs_acc_caption_fix.pdf}}\hfill
    \subfloat {\includegraphics[width=0.32\textwidth]{Figures/ethnicity_figures/biolen_vs_acc_caption_fix.pdf}}\hfill
    \subfloat{\includegraphics[width=0.32\textwidth]{Figures/interests_figures/biolen_vs_acc_caption_fix.pdf}}\hfill
    %\hfill
    \caption{Bio Length vs. Prediction Performance: The classifier could predict more accurately, as people write more content in their bios. Short bios usually contain a list of informative words (e.g., \textit{mom, father, asian american, MAGA}), which explains the initial surprisingly good performance. }
    \label{fig:prediction_bio_len_res}
\end{figure*}
%The breakeven point between tweets and Bios is 16 ($2^4$).

\begin{figure*}[htbp]
    \centering
    \subfloat{\includegraphics[width=0.30\textwidth]{Figures/gender_figures/accuracy_transformer_berttweet_repeat_1.pdf}}\hfill
    %\subfloat[Ethnicity.\label{fig:ethnicity_nb}] {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/accuracy_nb_repeat_5.pdf}}\hfill
    \subfloat {\includegraphics[width=0.30\textwidth]{Figures/ethnicity_figures/accuracy_transformer_berttweet_repeat_1.pdf}}\hfill
    %\subfloat[Personal Interests.\label{fig:interest_nb}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/accuracy_nb_repeat_5.pdf}}\hfill
    \subfloat {\includegraphics[width=0.30\textwidth]{Figures/interests_figures/accuracy_transformer_berttweet_repeat_1.pdf}}\hfill
    %\hfill
    \caption{Prediction performance comparison between bio and tweets: it demonstrates the rich self-identity in bio.
    Gender Prediction (\textit{left}): Bios contain rich clues of gender. Approximately 1 bio equals to 16 ($2^4$) tweets. 
    Ethnicity Prediction (\textit{middle}): More tweets reveal more about ethnic background.  The break-even point is about 8 ($2^3$) tweets.
    Personal Interest Prediction (\textit{right}): a few tweets (approx. 2) suffice to reveal user's interest as one bio does.
    }
    \label{fig:prediction_res}
\end{figure*}


%Another option is to concatenate tweets as a long sentence, but it may be truncated due to 512-token limitation in BERT family models.
%As the number of tweets increases, there become a challenge of how to obtain sensitive enough document-level embeddings\cite{lynn2020hierarchical} (eg. weighted pooling or message-level attention). It is an interesting topic, but falls out of the scope of this paper. \todo{delete this?}


\begin{table}[htbp]
\centering
\caption{The prediction performance using Biography only. The BERTweet model performs best, showing the advantage of pre-training on social media text. }
\label{table:bio_pred_res}

\small
\begin{tabular}{p{0.2\textwidth} p{0.1\textwidth} p{0.1\textwidth} p{0.1\textwidth}}
\toprule 
Task: &Gender &Ethnicity & Interests \\
\midrule
\#Classes &2 & 4 &7 \\
\midrule
\#Samples & 229,460& 12,192 & 14,483 \\
\midrule 
 Random & 0.500  & 0.250  & 0.142  \\

 Naive Bayes & 0.738  & 0.414  & 0.578  \\

 %AvgEmb. & 0.707  & 0.403  & 0.573  \\

 %BiLSTM & 0.743  & 0.416  & 0.594  \\

 RoBerta - CLS &0.735  & 0.376  & 0.525  \\

 %RoBerta - Mean &0.735  &-- & 0.528  \\
 %\hline
 BERTweet  &\textbf{0.780}    &\textbf{0.493}   & \textbf{0.649} \\
\bottomrule
\end{tabular}
\end{table}

%\todo{Accuracy vs. bio length  --- using the best model}

% confusion matrix ??
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{Figures/gender_figures/accuracy_Naive_Bayes_repeat_5.pdf}
%     \caption{Naive Bayes classifier (repeat five times).}
%     \label{fig:gender_nb}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{Figures/ethnicity_figures/accuracy_nb_repeat_5.pdf}
%     \caption{Naive Bayes}
%     \label{fig:ethnicity_nb}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{Figures/interests_figures/accuracy_nb_repeat_5.pdf}
%     \caption{Naive Bayes}
%     \label{fig:interest_nb}
% \end{figure}




\begin{figure}[htbp]
    \centering
    \subfloat[Female.\label{fig:1a}] {\includegraphics[width=0.45\textwidth]{Figures/gender_figures/gender_pos_0_bio_keywords.pdf}}\hfill
    \subfloat[Male.\label{fig:1}] {\includegraphics[width=0.45\textwidth]{Figures/gender_figures/gender_pos_1_bio_keywords.pdf}}\hfill
    %\hfill
    \caption{Top predictive words of Male/Female in bios from Naive Bayes Classifier. Stop words are excluded. }
    \label{fig:gender_keywords}
\end{figure}

\begin{figure}[htbp]
    \centering
    \subfloat[Business.\label{fig:interest_key_bussiness}] {\includegraphics[width=0.45\textwidth]{Figures/interests_figures/interests_pos_business_lb_bio_keywords.pdf}}\hfill
    %\subfloat[Entertainment.\label{fig:interest_key_entertainment}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/interests_pos_entertainment_lb_bio_keywords.pdf}}\hfill
    %\subfloat[Literature.\label{fig:interest_key_literature}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/interests_pos_literature_lb_bio_keywords.pdf}}\hfill
    %\subfloat[Music.\label{fig:interest_key_music}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/interests_pos_music_lb_bio_keywords.pdf}}\hfill
    \subfloat[Politics.\label{fig:interest_key_politics}] {\includegraphics[width=0.45\textwidth]{Figures/interests_figures/interests_pos_politics_lb_bio_keywords.pdf}}\hfill
    %\subfloat[Sports.\label{fig:interest_key_sports}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/interests_pos_sports_lb_bio_keywords.pdf}}\hfill
    %\subfloat[Tech.\label{fig:interest_key_tech}] {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/interests_pos_tech_lb_bio_keywords.pdf}}\hfill
    %\hfill
    \caption{Top predictive words of Personal Interests in bios from Naive Bayes Classifier }
    \label{fig:interests_keywords}
\end{figure}


\subsection{Gender Prediction}
% first, we show the signal words (excluding stop words) from NB's top featured words. P(x|y). We can see clear gender distinctive words for male and female. It shows the bio contains many clues about users' gender in the self-identity.
The results in Table \ref{table:bio_pred_res} shows that gender can be predicted with a decent accuracy (78.0\%) from biography alone.  
%\todo{NOTE: There are still many words that appear on both sides (writer, love, music).  Why?  If they are positive predictors on one side and negative on the other, we should say so.  Or better, only include the strongest positive predictors in each. (Jason)}
We show the most predictive words in bios (extracted from Naive Bayes) in Figure \ref{fig:gender_keywords}, consists of words with very strong gender components (e.g., mom, father, husband).
%\todo{NOTE: Were these words predictive in the bios or the tweets or both?  We should say explicitly. (Jason)} 

In addition, Figure \ref{fig:prediction_bio_len_res} shows that prediction accuracy improves as the bio length (in token) increases, reflecting that longer self-description reveals more clues about the person.

% \begin{table}[!h]
%         \centering
% \begin{tabular}{|p{0.08\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|}
% \hline 
%   & Asian \ vs \ Hispanic & Asian vs Black & Asian vs White & Hispanic \ \ \ vs Black & Hispanic \ \ \ vs White & Black vs White \\
% \hline 
%  Bio  & 0.650 & 0.655 & 0.620 & 0.650 & 0.607 & 0.653 \\
% \hline 
%  \makecell[l]{\#Tweets} & \textasciitilde 2 & \textasciitilde 1 & \textasciitilde 2 & \textasciitilde 2 & \textasciitilde 2 & \textasciitilde 2 \\
%  \hline
% \end{tabular}
% \end{table}


We also investigate how much gender-related information is encoded in daily re/tweets.
In Figure \ref{fig:prediction_res}, we divided users into groups according to the number of utilized re/tweets (in x-axis)\footnote{We keep test samples which has tweets more than the designated number, so the bio performance curve may fluctuate.}, and predict the gender given the tweets. For example, when \textit{\#Tweet} equals to one, we use just single randomly selected tweet to predict gender for each user. As we saw in Figure \ref{fig:prediction_res}, a single bio contains richer gender information than a single tweet does: it needs approximately 16 tweets to achieve the similar performance of a bio. 



%Error analysis: 

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c|c|c}
%     \toprule
%     Bio & Ground truth & Prediction
%     \midrule
%     work, hard, pray, harder, romans, mechanical, engineering, student, nc, at & Female & Male  \\ 
%     \hline
%     nigeria, united, states, born, co, founder, ceo, co, host, podcast, tuesday, s, pm, wat, on, twitter, youtube, live & Female & Male  \\ 
%     \hline
%     \bottomrule
%     \end{tabular}
%     \caption{Error Cases}
%     \label{tab:gender_err_case}
% \end{table}

\begin{comment}
\begin{figure}[htbp]
    \centering
    \hspace{-0.034\textwidth} \subfloat {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/fig_pairwise_acc_bert.pdf}}\hfill
    \subfloat {\includegraphics[width=0.23\textwidth]{Figures/interests_figures/fig_pairwise_acc_bert.pdf}}\hfill
    \caption{Pairwise prediction accuracy. Blue color indicates low accuracy. Ethnicity (\textit{left}): It is difficult to distinguish Asian from White. Personal Interests (\textit{right}): It is hard to distinguish sports and entertainment.}
    \label{fig:prediction_res_breakdown}
\end{figure}

\end{comment}

\subsection{Ethnicity Prediction}
% Ethnicity is implicitly encoded in bio. We found few people explicitly indicate their ethnicity identity in bio. So most of key words in different ethnicity group looks very similar. But still we found some stereotypical key words  (engineer in Asian, Texas/Mexico in Hispanic)

As shown in Table \ref{table:bio_pred_res} and Figure \ref{fig:prediction_bio_len_res}, the best model can predict 4-class ethnicity with 49.3\% accuracy, and the accuracy increases as users write more in their bios.
In general, it is more challenging to predict ethnicity from bio, because we don't observe many highly ethnicity biased words. However, some anecdotes can be found, for example, we found predictive (but usually stereotypical) words: such as \textit{engineer} in Asian, \textit{Texas, Mexico} in Hispanic group and \textit{black} in African-American group. Similar feature analysis results were also observed in \cite{preoctiuc2018user}.
But, as Figure \ref{fig:prediction_res} shows, a single bio has more predictive power when compared to one random tweet. Approximately 8 tweets are required to achieve the same prediction accuracy as a single bio.
%, and it gains more accuracy as seeing more tweets.



%We present pair-wise (one-vs-one) ethnicity prediction accuracy in Figure \ref{fig:prediction_res_breakdown}.  
%We also include pair-wise Bios and Tweets comparison in Figure \ref{fig:prediction_res_ethnicity_breakdown} in Appendix. 

%\todo{add the figure in appendix -- add reference to ethnicity difference analysis?}

%https://www.aclweb.org/anthology/D11-1120.pdf
% 1. label is not clean 

% \begin{figure}[htbp]
%     \centering
%     \subfloat[Asian.\label{fig:eth_key_asian}] {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/ethnicity_pos_asian_bio_keywords.pdf}}\hfill
%     \subfloat[Black.\label{fig:eth_key_black}] {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/ethnicity_pos_nh_black_bio_keywords.pdf}}\hfill
%     \subfloat[Hispanic.\label{fig:eth_key_hispanic}] {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/ethnicity_pos_hispanic_bio_keywords.pdf}}\hfill
%     \subfloat[White\label{fig:eth_key_white}] {\includegraphics[width=0.23\textwidth]{Figures/ethnicity_figures/ethnicity_pos_nh_white_bio_keywords.pdf}}\hfill
%     %\hfill
%     \caption{Top predictive words of Ethnicity from Naive Bayes Classifier, excluding stop words. }
%     \label{fig:ethnicity_keywords}
% \end{figure}





\subsection{Personal Interests Prediction}
% We show the example of predictive words of personal interests from bio text. Many of them is directly related with the topics. (maga in politics, artist in music.  young people (university) in sports.)

Biographies may contain personal interests as shown in Figure \ref{fig:interests_keywords}.
The people of different interest groups use distinctive words in their bios. As Table \ref{table:bio_pred_res} and Figure \ref{fig:prediction_bio_len_res} shows, we can predict personal interest with 64.9\% accuracy, and the accuracy keeps improving as the bio length grows. 
% In Figure  \ref{fig:prediction_res_breakdown}, we observe that it's easier to distinguish a user interested in literature from one interested in business, while it is more difficult to discern sports interest from entertainment.

In addition, re/tweets also contains rich information as people often engage in the conversations (re/tweets) matching to their interests. 
From the experimental results in Figure \ref{fig:prediction_res}, roughly 16 random tweets could tell the personal interest with 80\% accuracy. A single bio still outperforms a single tweet.


% 8 pages,
% score of bio 
% routine classification  (2-3 pages)
% how bio evolves (3 pages) big novelty, promotion demotion ...
% (ex-..) how often that happened. things they were proud of.
%  former, ex-
% break down of different bio



\begin{comment}
\subsection{Data cleaning and Pre-processing:} The raw data is noisy, containing non-human accounts (e.g., official accounts of organizations) and inactive accounts without tweet or bio. We clean the data by the following procedure:

\noindent{\textbullet\  \textbf{Keep active English users:}} We filter out those accounts whose bio contains less than 25 characters (about 20\% as shown in Fig.\ref{fig:bio_len}), and use the FastText language identification tool \cite{joulin2016fasttext, joulin2016bag} to filter out all non-English bios.%\todo{NOTE: Can we give a count or percentage of users who were removed with this criterion? (Jason)} 

%38601 151671 1,353,325
\noindent{\textbullet\  \textbf{Filter non-human accounts:}}  We remove the accounts whose name is non-alphabetic and has more than three parts (assuming a normal name has first, middle and last name), and remove non human-like names by matching the first/last name to the public U.S. census data \footnote{ 2000 U.S. Census contains 38,601 unique first names and 151,671 last names. We consider it is a valid human name if either first or last name is in the list. \url{ https://github.com/rossgoodwin\/american-names} }. Then, we manually check the most frequent 100 names and remove common ambiguities\footnote{E.g: \textit{Center} is a relatively rare surname, but it is very common in the centers (buildings) named after human (e.g. Javits Center). To reduce noise, we remove all whose surname is Center. }.
We also filter out the users whose bio explicitly contains brand-like key words (e.g. \textit{official twitter/account}). After this cleaning process with our best efforts, we have 412,621 valid twitter human users with genuine names.


\noindent{\textbullet\  \textbf{Fetch and normalize tweets:}} To compare the predictive power between biographies and tweets, we randomly sample up to 200 tweets if available from each user. We anonymize bios and tweets by removing contact information (phone, email, twitter handles). Since Emojis and hashtags are very common and informative in bios and tweets, we convert them into a textual form in order to preserve as much information as possible
\footnote{Emoji: Convert Emoji to text: \url{https://github.com/carpedm20/emoji/} WordNinja: split hashtag to meaningful word segments \url{https://github.com/keredson/wordninja}}.

% 369850 for name
%373327 for 
% filtering out English, matching user name
\noindent{\textbullet\   \textbf{Demographics Acquisition from User Names:}}
% name filtering, removing brand and less likely name.
 Demographic information is important for social media analysis, however most platforms (e.g. Twitter, Facebook) do not provide access to these attributes due to privacy concerns. Human names reveal considerable information about gender and ethnicity, so we use name embeddings\footnote{Gender detector: \url{https://github.com/kensk8er/chicksexer}} \cite{sood2018predicting, ye2017nationality,ye2019secret} to infer gender and ethnicity of twitter users. 
To assure the inference quality, we only retain the results predicted with confidence threshold greater than 95\% for gender (male/female) and 50\% for ethnicity (White/Black/Hispanic/Asian) classification. 
Since the original label distribution is highly imbalanced, we under-sample the majority classes to keep label balanced, resulting in a total of 229,460 and 12,192 samples in the gender and ethnicity tasks, respectively.


\noindent{\textbullet\   \textbf{Personal Interests Acquisition from Tweet Hashtags:}}
Hashtags are important for social information diffusion \cite{small2011hashtag}. A hashtag often contain a word, phrase or short sentence, reflecting a specific topic or event that people care about. 
%For example: politics (\textit{\#Trump}), music (\textit{\#NowPlaying}), or sports (\textit{\#NBAFinal}), etc.
%Such hashtags in the tweets are strong evidence that the user is interested in such topics. 
Similar to \citet{conover2011predicting}, we select 187 representative hashtags from the most frequent ones and categorize them into 7 groups as shown in Table.\ref{tab:hashtag_category}.
More than 90\% of the users only have one label assigned, so we formulate it as a multi-class prediction task. Similarly, we under-sample the majority class to make it balanced with 14,483 samples in total.

\end{comment}


==> chapter4-BiosModification/Figures/twitter_bios_raw_chunk/0.tex <==
\begin{tabular}{p{0.38\textwidth}|p{0.38\textwidth}|p{0.04\textwidth}|p{0.1\textwidth}}
\toprule
                                                                                                                                                                                                                                           Before &                                                                                                                                                                    After &  Edit Dis. & BERTScore \\ \hline
\midrule
                                                                                                                                                                                          thinker of thoughts . doer of things . goer of places . &                                                                                                                                                     wash . your. hands . &         10 &   -0.0329 \\ \hline
                                                                                                                                                                             the official twitter account for singer \& designer matthew decker . & singer . songwriter . platinum blonde ( at heart ) . new single " star tonight " \& " shoes ( the remixes ) " available on @applemusic now . http://itsmatthewdecker.com &         29 &   -0.0148 \\ \hline
slaps : http://m.soundcloud.com/yo-rico \_\_\_\_\_\_\_\_\_\_\_\_\_\_ snapchat : @gurvinder54 \_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_ it is what it is \_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_ &                                                                                                                          | • 19 | •fresno state 🐾 | •sc / / gurvinder 54 &         14 &   -0.1805 \\ \hline
                                                                                                                                                                                                  i'll be the actress starring in your bad dreams &                                                                                                                                            💕🎶meet me in the afterglow🎶 💕 &          8 &   -0.1650 \\ \hline
                                                                                                                                                                                      lately been feeling lost so im slowly trying to find myself &                                                                                                                                                               01/31 | rd &         11 &   -0.2706 \\ \hline
                                                                                                                                                                                                                                          kee|key &                                                                                                                                                                dayung1 ✨ &          2 &   -0.2400 \\ \hline
                                                                                                                            a slowly moving mass or river of ice formed by the accumulation and compaction of snow on mountains or near the poles &                                                                   a quorum of lobster brains with a twitter account λ code ♪ music ◉ games δ dsp ☼ graphics ⁓ stats / ml &         22 &   -0.2947 \\ \hline
                                                                                                                                                                                                                     i ’m literally 99 \% hot gas &                                                                                                                                                 farts boobies buttcracks &          7 &   -0.0204 \\ \hline
                                                                                                                                  follower of jesus ✝️ | blogger 💻 | \#vstate20 | new post ✨ : https://upopinion.weebly.com/blog/august-02nd-2018 &                                                                  follower of jesus | creative | \#vstate20 | set free | new youtube video : https://youtu.be/jzc4sbg5cbo &          9 &   -0.0397 \\ \hline
                                                                                                                                              we need to be reflective and respectful of diverse ideas in an ever- more chaotic , violent world . &           visiting scholar @rutgers\_cghr | oud virtuoso | composer | music director \& founder @ \#aleppoensemble | \# thejasminetree \#album | \# soho \#album @itunes &         24 &   -0.2545 \\ \hline
                                                                                                                                                                                                                 the purpose of life is to sing ! &                                                                                              wall street veteran turned singer of life ... http://youtu.be/ucadlxwkase?a &          9 &   -0.2402 \\ \hline
                                                                                                                                                                                                                                       lol u wild &                                                                                                                                       valerie says i look like lilo ///: &          7 &   -0.1464 \\ \hline
                                                                                                                                                                                                                                       in the lab &                                                                                                                                                             .... loading &          3 &   -0.0231 \\ \hline
                                                                                                                           i started parting my hair on the side in 2002 because of kim possible and it 's the only hairstyle i've had since then &                                                                                                                                                          super fantastic &         24 &   -0.0641 \\ \hline
                                                                                                                                                                                                                           mercy college baseball &                                                                                                                                      stick to the plan , stay focused !! &          8 &   -0.1626 \\ \hline
                                                                                                                                                                                                                huge wrestling fan , football fan &                                                                                                                                                        the whole shebang &          6 &   -0.2405 \\ \hline
                                                                                                                                        am skater and freestyle dancer from campo grande - ms / brasil | nephew clothing | snapchat : mathrodrigz &                                                                                                                                     hi ! i'm support 👻snap : mathrodrigz &         17 &   -0.0404 \\ \hline
                                                                                                                                                                                                                                   ♡ tip or die ♡ &                                                                             young matriarch / / party enabler//gemstoner//incubating artist//ocean explorer//beachcomber &          8 &   -0.3934 \\ \hline
                                                                                                                                                                                                       🇲🇽🇺🇸 | snap : carooogarzaaa | @chanceperez &                                                                                                                                    life is short do what u want // utrgv &          9 &   -0.5171 \\ \hline
                                                                                   blessed young man basketball comeback 2016 : 21 years of age : future phd holder : creat higher education for somalia \# firm beliver in change allah is first &                                     all praise to the almighty , being humbled is key , success comes from prayer and i pray we all succeed future politician in somalia &         28 &   -0.1376 \\ \hline
                                                                                                                             enjoying time with my daughter and wife ! go spurs and go texans ! someone bring me an michelob ultra and some bbq ! &                                                                                  life is not a matter of holding good cards , but sometimes , playing a poor hand well . &         24 &   -0.1151 \\ \hline
                                                                                                                                                                                                                                        anthony ❤ &                                                                                                                                                            sc : mandyk34 &          3 &   -0.1124 \\ \hline
                                                                                                                                                             statement of who i am . statement of what i do . statement of this is all my fault . &                                writer at @thermofisher . grad student at @wsupullman . bibliophile wherever i happen to be . trying to make the world a little clearer . &         22 &   -0.0351 \\ \hline
                                                                                                                                                                                     aspiring film producer . former nickelodeon casting intern . &                                                                                                                                                                   👑☘️🏜 ✨ &          9 &   -0.4425 \\ \hline
                                                                                       i 'm a man of god . i am focused on becoming all that i can be and make a difference in this world ! \#striveforgreatness \# besomebody \# leadforgodssake &                                                                                                                                \#akronmanufacturesdreams \# thewiseunite &         29 &   -0.0837 \\ \hline
                                                                                                                                                          offensive coordinator \& quarterbacks coach at the college of william \& mary . \# gogo &                                                                                                                                            hawai ’i wide receivers coach &         14 &   -0.0702 \\ \hline
                                                                                                                                                                   john wayne movies and i do n't line dance . south dakotan in oklahoma \# swosu &                                                                                                                                                     trainin wild animals &         16 &   -0.2140 \\ \hline
                                                                                                                                                                                                                            brazil honduras spain &                                                                                                                                                                       ot &          3 &   -0.2887 \\ \hline
                                                                                                                                                                                                                             antisocial extrovert &                                                                                                                                                                nurse joy &          2 &   -0.0606 \\ \hline
                                                                                                                                                                                                                 we get it , you vape i am second &                                                                                                     i believe in two things , the first amendment and boobs . kanye 2020 &         13 &   -0.8166 \\ \hline
                                                                                                                                                                                                                     get your game on \# dontplay &                                                                                                                                                              more life 🍔 &          6 &   -0.0507 \\ \hline
                                                                                                                                                                                                                           stay humble . \# msu19 &                                                                                                                                                        morgan state / ct &          5 &   -0.1588 \\ \hline
                                                                                                                                                                             it 's a dog eat dog world do n't get bit bruh .. \# blacklivesmatter &                                                                                                                                            ravioli stuffed with diamonds &         15 &   -0.4398 \\ \hline
                                                                                                                                                  i swear i do n't care about your feelings , especially since i do n't have feelings of my own . &                                                                                                                                  5'1 but my attitude is 6'3 . rip dad ❤️ &         21 &   -0.0599 \\ \hline
                                                                                                                               professional skateboarder . ☮ ♥ ♫ live with love ! follow me on instagram @carlosmacias\_mo \#skaterboy \# chicago &                                                                skater . gym. live with love ! class clown turned pro* candy enthusiast * dougnuts are life ☮ ♥ ♫ 4/18/13 &         19 &   -0.0100 \\ \hline
                                                                                                                                                                                                                             dont shoot your shot &                                                                                                                                                              tyson ray 🕊 &          4 &   -0.2834 \\ \hline
                                                                                                                                                                                              texas tech womens basketball student assistant ' 17 &                                                                                                                                                        texas tech alum👆🏻 &          6 &   -0.1410 \\ \hline
                                                                                          24 . student affairs . cat person . internet enthusiast . nail polish obsessed . lover of the sun . extreme foodie . spicy and sweet . dolphin alumni . &                                                                                                                                                                weird . 🖤 &         29 &   -0.0266 \\ \hline
                                                                                                                                                                                                    thomas university baseball ' 19 \# nighthawks &                                                                                                                                       just out here witnessing greatness &          7 &   -0.2095 \\ \hline
                                                                                                                        dennis dudley | oviedo varsity student - athlete | sophomore ( 2019 ) | http://www.hudl.com/athlete/6266580/dennis-dudley &                                                                                                                                                           wb @ lhhs \# 3 &         15 &   -0.2330 \\ \hline
                                                                                                                                                                                                                                  @carolinajay 11 &                                                                                                                                         lchs football \# 80 / / ⚡️wru⚡ ️ &          8 &   -0.4611 \\ \hline
                                                                                                                                                                                          http://youtube.com/neobeartvhttp://youtube.com/neomerge &              https://t.co/ybwuqly2fb - thottieciti -i play video games with my wife at https://t.co/ernc0pl4o6 and my personal channel with is athttps://t.co/xql5hiovnz &         19 &   -0.2394 \\ \hline
                                                                                               im a lyricist . captain of the abstract movement known as middle finger militia or mfm download my newest tape at http://epthedreamer.bandcamp.com &                                                                                 please take a listen and enjoy the music i make to inspire you in my link provided below &         20 &   -0.0642 \\ \hline
                                                                                                                                                                                                               heres to feeling good all the time &                                                                                                                                                    looking and listening &          7 &   -0.1142 \\ \hline
                                                                                                                                                                                                                                ig : kyle\_bronco &                                                                                                                                                                  absecon &          3 &   -0.2592 \\ \hline
                                                                                                                                                                                                                          in dog years i'm dead . &                                                                                                                               🌙✨ " ugly on the skin , beautiful within " &         10 &   -0.0500 \\ \hline
                                                                                                                                                                                        university of cincinnati 's college panhellenic council . &                                                         university of cincinnati 's college panhellenic council — γφβ | δδδ | θφα | καθ | κδ | κκγ | πβφ | φμ | φσρ | χω &         20 &   -0.0785 \\ \hline
                                                                                                                                                                                                 fisher high and southeastern la alum . sports .. &                                                                                                                     who dat . snapchat : b\_robeaux fantasy football guy &          9 &   -0.1294 \\ \hline
                                                                                                                                            pragmatic . non ideological and non populist . 5'11 " / 180 . great lakes and western us enthusiast . &                                                                       a lewbowski urban achiever . i share what i'm reading . i like and retweet interesting headlines . &         17 &   -0.1217 \\ \hline
                                                                                                                                     young , single , n a educated mixed kid huh but my blackness is always dominant✊ georgia is my home aries♈ ️ &                         one soul\textasciitilde{}one man african american / dutch caribbean / native american ... aries♈️6️⃣ \# dawgnation \# falcons \# bronbron \# blm &         22 &   -0.1235 \\ \hline
                                                                                                                                 web designer by day , manager of @primeexample716 by night . tellin it like it is since ' 89 . \# primetime \#pe &                                                                                         its never too late to change your life . always keep improving . \# thinkforward &         20 &   -0.0274 \\ \hline
                                                                                                                                                                                                                                 thick and lonely &                                                                                                                                                                  lsu σαε &          3 &   -0.2620 \\ \hline
                                                                                                                                                                                             ls4laj 👼 longliveeazy ☝🏾millyano3739@gmail.com 37-39 &                                                                                                                                                           resteazy • l4l &          5 &   -0.1441 \\ \hline
                                                                                                                                                                                                              i ’ve ran out of shit to put here . &                                                                                                                                                            stay golden 🥀 &         10 &   -0.1378 \\ \hline
                                                                                                                                                                                                  \#goga \#eat \# job \#charers \# sipboy \# nols &                                                                                                                                      ole miss football signee .... octid &          9 &   -0.2778 \\ \hline
                                                                                                                                                                                                                         sf • mac artist • jja ❤️ &                                                                                                          certified mac artist / bay area mua • jja • |rip zahid arshad | &         11 &   -0.0756 \\ \hline
                                                                                                                                          god 1st \& foremost .... artist / picture painter \# fewbucksandadream free dl : http://piff.me/9195d55 &                                           god 1st | picture painter | \#justdoit | \# perfectstorm | \# superfreak |thamackmusic@gmail.com | no co-signers ... just me 💯 &         18 &   -0.1448 \\ \hline
                                                                                                                                                                        pink palace pimp 1 - 800 - ayy-lmao fuck kingdude23 \# gorillalivesmatter &                                                                                                                                                    where 's my naivety ? &         12 &   -0.4105 \\ \hline
                                                                                                                                                                                                                class of 2016 snap - corrina.foss &                                                                                                                                 music helps me fall asleep \& it 's nice &          9 &   -0.0937 \\ \hline
                                                                                                                                                                                                                                     get schwifty &                                                                                                                                                                 ooo-weee &          2 &   -0.1235 \\ \hline
                                                                                                                                                                                                                                            22:24 &                                                                                                                                             \#444 neighborhood superstar &          3 &   -0.4808 \\ \hline
                                                                                                                                                                                                                                           blm✊ 🏾 &                                                                                                                                                                       🇧🇧 &          2 &   -0.3603 \\ \hline
                                                                                                                                                                                                     its always your favorite sins that do you in &                                                                                                                                      18 years old •fsu theatre major• ♏️ &          9 &   -0.2792 \\ \hline
                                                                                                                                                                                                           authentic . ( larrybyrdstl@gmail.com ) &                                                                               my new single run that checc up available on itunes , google play , etc ... \#hustlerzonly &         17 &   -0.7507 \\ \hline
                                                                                                                                                                           history \& sociology major at the university at albany \# the7linearmy &                                                                                                                                              a long suffering sports fan &         11 &   -0.1368 \\ \hline
                                                                                                                                                                                                 roll a bleezy take it easy \#onenationundersquad &                                                                                                                                                      on to better things &          7 &   -0.1677 \\ \hline
                                                                                                                                                thirty -something . pale . vaguely potato-shaped . gay twitter archivist . hydrated \& unamused . &                                                                                                      “ why are you like this ? ” — my friends , relatives , \& coworkers &         16 &   -0.0238 \\ \hline
                                                                                                                                                                                                                             living in the moment &                                                                                                                                                                  5/14/16 &          4 &   -0.3787 \\ \hline
                                                                                                                                                                                                                   i like yoga and alkaline water &                                                                                                                                                     creator of fr▲nc\_tv &          6 &   -0.1727 \\ \hline
                                                                                                                                                                      home of the 2016 fantasy football championship team the certified bangerz . &                                                                                       do you know how many basic bitches would kill to have the same personality as me ? &         16 &   -0.1245 \\ \hline
                                                                                                                                                                                                                                       mv / cc 18 &                                                                                                                             seattle u•leftist political slut•indie trash &          5 &   -0.2365 \\ \hline
                                                                                                          artist • new debut single \# feeling out now on itunes , apple music , spotify and more ! ep coming soon!http://patreon.com/sofiazorian &                                                              pop blues⚡️music artist | songwriter 💌 contact@sofiazorian.com 📸 @sofiaslens http://patreon.com/sofiazorian &         22 &   -0.2459 \\ \hline
                                                                                              cali born , texas raised . managing editor of @sawmillsports and junior at sfa . vice prez at @sfasu\_ifc , frater in @sfatke . opinions are mine . &                                  offspring of california hippies || editor @sfasawmill || co-host @ purple lights podcast || hubs @the\_jacy || tke || snap : iniedrauer &         27 &   -0.0691 \\ \hline
                                                                                                                                                                        trying to make my way in this crazy world . 🇺🇸 and 🇸🇻 equal parts of me . &                                                                                                                               immigrant ✊🏼 mother ❤️ we shall overcome . &         17 &   -0.0959 \\ \hline
                                                                                                                                                                                                                           question everything 🕴🏼 &                                                                                                                                             i ’m just happy to be here🕴🏼 &          7 &   -0.4903 \\ \hline
                                                                                                                                                                                                                       i know the boys who did it &                                                                             senior content manager , http://shondaland.com pitch me , y'all : seth at shondaland dot com &         15 &   -0.2495 \\ \hline
                                                                                                                                                                                                                                 bills mafia baby &                                                                                              i'm not a bad kid i just did n't have no guidance \# billsmafia \#dubnation &         15 &   -0.0027 \\ \hline
                                                                                                                                                                                                                   i catch flights , not feelings &                                                                                                                                      in a collab w/ æjoey | ig : simpney &          9 &   -0.1056 \\ \hline
                                                                                                                                                                                           melodramatic artist . graphic design . ig : agnikaii\_ &                                                                                                                                                      artist or something &          8 &   -0.2845 \\ \hline
                                                                                                                                                                                                             smoke big green call me bruce banner &        the key to improvement is simply asking yourself the right questions combined with a certain level of creativity . also i play rob in super smash bros . ultimate &         29 &   -0.1170 \\ \hline
                                                                                                                                                                                                                      mhs c/ o ' 17 / / mvp sj⚡ ️ &                                                                                                                  she see money all around me , i look like i'm the man ! &         14 &   -0.2620 \\ \hline
                                                                                                                                  i do political things but mainly tweet about cute animals and the blues • just happy to be here • mo state alum &                                \# moleg staffer and oxford comma enthusiast \{@missouristate and @trisigma alum\} | views are my own because no one else will claim them &         23 &   -0.1260 \\ \hline
                                                                                                                                                                                                               r.i.p britt , flee , lil man \&chi &                                                                                                                                                         sc : deeva2811 📸 &          8 &   -0.3126 \\ \hline
                                                                                                                                                                                                                            i am trying very hard &                                                                                                                       girl laughing alone http://instagram.com/mintshake &          5 &   -0.0324 \\ \hline
                                                                              love god \& family , wife , passionate warning people dangers of opiate abuse . drug abuse is an equal opportunist . \#herionkills \# destroysfamily \# letgoletgod &  love god guns are safer than drugs .. too many youth oding daily basis . war on drugs never worked . help instead of criminalize addict for being on drugs / nonviolent &         29 &   -0.0648 \\ \hline
                                                                                                                                                                                                                •coffee , cats , and technology • &                                                                                                                                 jasmine 🌹🖤 • " gucci owes me a check . " &         11 &   -0.1391 \\ \hline
                                                                                                                                                                                            to weird to live • to rare to die • @juanvelazquezx\_ &                                                                                                                                             @skatehighx ♡ @wyldstyl\_htx &         11 &   -0.1621 \\ \hline
                                                                                                                                                                                                                  hairdresser✂ ️ \#lyssowen\_hair &                                                                                                                                                     it ’s shalyssa bitch &          4 &   -0.2281 \\ \hline
                                                                                                                                                                                                         hey everyone , karma got its kiss for me &                                                                                                                                                            he / him /his &          9 &   -0.1691 \\ \hline
                                                                                                                                                the only constant thing in this world is change ... and the bacterial growth in your intestines . &           stu alum / university of miami research assistant , department of psychiatry \& behavioral science / ucf graduate student of biomedical sciences ( fall 2019 ) &         26 &   -0.2698 \\ \hline
                                                                                                                       a warrior not a worry ( er ) comedian , cool ass human being trying to make the world laugh , smile \& fulfill the promise &                         multi-talented humorist catch me on http://beatnetwork.com podcast : pillow talkfb : tavon greatness pattersonig : tavongreatnesssc:tavongr8ness &         26 &   -0.2050 \\ \hline
                                                                            year of the rabbit , capricorn ; adaptive technology instructor @lbph ; cheers for the mountaineers , ravens , celtics \& orioles ; reader of mysteries love movies . &                                                                                 accessible technology specialist @lbph . connosseur of cheeseburgers \& vanilla shakes . &         25 &   -0.0949 \\ \hline
                                                                                                                                                                                                                             february 's very own &                                                                                                                                  sorry ladies , i'm not the golfing type &          8 &   -0.1384 \\ \hline
                                                                                                                                                             we ’ve cried enough in our lives . vocals in vvitchking ⚰️selena got me all like 😍🥴🥺 &                                                                                            idk man i just like black metal and tweeting dumb shit . 24 . ⚰️ \\$ painxpiss &         17 &   -0.0485 \\ \hline
                                                                                                                                                                                                      i love angell d'lucas ❤️ christian athlete™ &                                                                                  work hard in silence , let success make the noise .................. |how you doing ? | &         16 &   -0.2512 \\ \hline
                                                                                ⚾️ stuff ... joe blanton has more world series home runs than ted williams and more world series wins than nolan ryan . not affiliated with major league baseball &                         baseball stats \& commentary . author ( see pinned tweet ) . purdue data science ‘ 23 . founder of @diamond\_digest . not affiliated with @mlb . &         25 &   -0.1134 \\ \hline
                                                                                                                                                           but a mermaid has no tears , and therefore she suffers so much more | rowan university &                                                                                                                                                     aries ☼ / aquarius ☾ &         17 &   -0.3478 \\ \hline
                                                                                                                                                                                                                                    2016 , all in &                                                                                                                                                                  16 ' ♨️ &          4 &   -0.1424 \\ \hline
                                                                                                                                                                                                everyone say u the best better not be nothin less &                                                                                                                           pick of the litter nigga mellohypeee@gmail.com &          9 &   -0.2881 \\ \hline
                                                                                                               morning becomes eclectic is hosted by @kcrw 's music director @jason\_bentley . m-f 9 - noon on 89.9. on demand at http://kcrw.com &                                                                                kcrw 's signature music program featuring new releases , live performances and interviews &         21 &   -0.0387 \\ \hline
\bottomrule
\end{tabular}



==> chapter4-BiosModification/Figures/twitter_bios_raw_chunk/1.tex <==
\begin{tabular}{p{0.38\textwidth}|p{0.38\textwidth}|p{0.04\textwidth}|p{0.1\textwidth}}
\toprule
                                                                                                                                                                      Before &                                                                                                                                                                     After &  Edit Dis. & BERTScore \\ \hline
\midrule
                                                                                                                                                               be about it . &                                                                                                                                                just following my dreams . &          4 &    0.1764 \\ \hline
                                                                                                                             certified athletic trainer . isu alum . tacos . &                                                                                               pe / health teacher . athletic trainer . lover of tacos \& hocus pocus 💀🌮 🔮 &         13 &    0.0143 \\ \hline
                                                                                                 live the life you 've imagined . snapchat : @ishieeee • insta : @iishaaaa\_ &                                                                  make you banana pancakes , pretend like its the weekend .. snappiesnap @ishieeee\_ • insta : @iishaaaa\_ &         13 &    0.2110 \\ \hline
                                     dj / producer / artist i produce and mix electronic music along with photography . if you want to make something together let me know ! &                                                                                     producer / photographer / enlightened / want me to edit a photo for you let me know ! &         19 &    0.0939 \\ \hline
                                                                                                                                                                  be happy . &                                                                                                                                                             loving home 🏡 &          3 &    0.0709 \\ \hline
                                           i like business ... transactions . music. sports . sabres , steelers , nats , byu , jazz , rsl . winner dahl american - best zoob &                                                                                      music ! sports ! byu , jazz , steelers , nats , sabres , rsl , west ham \# coyi ⚒⚔ ️ &         20 &    0.1988 \\ \hline
          do what ever makes you fucking happy . childhood pornstar turned rapper . @indycut family member . creature of habit out now . booking : forrestgumpshun@gmail.com &                                                                            forrest gumpshun is a childhood pornstar turned rapper . do whatever makes you fucking happy . &         20 &    0.2848 \\ \hline
       conversion optimization : http://deveshdesign.com. content marketing : @growandconvert . basketball : warriors ( lots of gsw tweets , be warned ) . nepali american . &                                   co-founder of @growandconvert , a content marketing agency ( http://growandconvert.com). founder of http://growthrock.co a cro agency . &         22 &    0.2056 \\ \hline
                                                                                                                                    love yourself enough and live in peace . &                                                                                                                                                        a typical cancer . &          7 &    0.1807 \\ \hline
  already toast . writer ( essays , food , recipes ) , editor , recovering victorianist , \# takebacktuesday , \#binders . tweeting dinner ideas by request @kitchenmacgyver &              writer ( essays , food , recipes ) , editor , recovering victorianist . dining critic @sacbee\_news . all opinions my own . also @kitchenmacgyver \# binders &         16 &    0.3829 \\ \hline
                                                                                                                                       writer / photographer . \# teamtulane &                                                                                                                                      nola boywriter / photographer . \#tu &          4 &    0.1265 \\ \hline
                                                                                                                                        | etsu ' 19 • referee at just jump | &                                                                                                                                                     etsu • alpha xi delta &          8 &    0.0475 \\ \hline
                                                                  burrage like courage . 😸📰 bacon enthusiast | clear talent group | new york city instagram : @joshuaburrage &                                                    currently doo-wopping with @bxtalemusical 🇮🇹 @newsies \& @catsbroadway | clear talent group instagram : @joshuaburrage &         12 &    0.0586 \\ \hline
                                                                                                  lawyer guy • poli-sci nerd • film fan • phd candidate • very stable genius &                                                                                                                                  legal nerd • politics nerd • film nerd • &         10 &    0.2034 \\ \hline
                                                                                                                                                                  just stuff &                                                                                                                                       overanalyzing everything since 1991 &          4 &    0.1047 \\ \hline
                                                                             i do my daily service just to see the gates of afterlife |csu northridge c/ o ' 19|👻@shmoneytay &                                                                                                                            |csun🎓 | 🎨👟🔥|👻@shmoneytay | ig : @devo.customs &         18 &    0.0625 \\ \hline
              when i ’m not writing novels and short stories ( mostly in my journal ) , i ’m climbing rocks , pursuing truth , and trying to make the most of my mortality . &                                                                  portland , or writer of speculative fiction , the research for which results in the rest of my writing . &         29 &    0.1109 \\ \hline
                                       writer of stung on @netflix and the communication room from @vbp\_publishers in print and ebook ... typing till my fingers fall off . &                                                                                                                                         typing till my fingers fall off . &         16 &    0.1680 \\ \hline
                                                                                                                                                        i do sea bass things &                                                                                                                        lions do n't lose sleep over the opinions of sheep &          9 &    0.1861 \\ \hline
                                                                                                                                             father . feeder driver at ups . &                                                                                                                                      husband . father . ups feeder , cach &          7 &    0.1952 \\ \hline
energy independence - legal immigration - fairtrade -stand with israel - brexit-states rights - wounded warriors are my heroes , not football players \# maga \# truethevote &                                                                                                                                           like kanye , i'm a free thinker &         26 &    0.0042 \\ \hline
                                                                                                                                    newfield hs ' 18 fly high dylan 4/6/2016 &                                                                                                         i ’m as sick as spongebob with the suds | fly high dylan 4/6/2016 &         10 &    0.0719 \\ \hline
                                                                                                                                     snapchat - jake\_mcleod | \# patsnation &                                                                                                                                                     \#patsnation • tke πθ &          6 &    0.0205 \\ \hline
                                                                                          rise in christ ! glow ya light , show ya love :) watch videos here @arksparkoflove &                                                                                 \#championsofchange🌟\#keepgodfirst \& \#letlovebeyourlegacyvideovisualart @arksparkoflove &         15 &    0.1568 \\ \hline
                                                                                                                                                           no dogs , no me . &                                                                                                                      an artist that deals in sound ( and sometimes dogs ) &         11 &    0.2014 \\ \hline
            daddy , storyteller , faa-certified drone pilot \# publicsafetyuas , photo / video maker , podcast host , former political / business journalist . tweets=mine . &                                                                                      proud dad | drone pilot | podcaster | photographer | journalist | dreamer | optimist &         24 &    0.1269 \\ \hline
                                                                           honolulu 's premiere concert and events venue since 2012 . https://soundcloud.com/jointherepublik &                                  honolulu 's premiere concert and events venue , locally owned \& operated since 2012 . check our website for upcoming shows and events . &         14 &    0.3567 \\ \hline
        national lecturer , touring the country , offering seminars on the size matters handwriting program and practical strategies on improving school - based ot practice &                                          our mission is to bring materials to therapists , teachers , and parents that are effective , efficient , affordable , and fun . &         25 &    0.1854 \\ \hline
                                                                                                                                                        ncat📚• personal blog &                                                                                                                                      god bless • ncatalum • ig📸mxttdxwson &          6 &    0.0155 \\ \hline
         recording artist | music addict | battle rap fan | basketball fiend | faith junkie | \#neversettle \#goingformine \# shelltown \# bullcity \#heatnation \# buzzcity &                                                                                                        recording artist | nerd | weirdo |rebel |http://www.dontecredo.com &         21 &    0.0496 \\ \hline
                                                        huge fan of hard rock \& metal music \& wwe wrestling , bassist for upcoming brand new metal band unlimited damage . &                                                                                                                                       singer for my upcoming metal band . &         18 &    0.2638 \\ \hline
                                                                                 i start riots and finesse these hoes without them even knowing . snapchat : @wyatttheriot08 &                                                                          saucing up your whole life from home to japan soundcloud : https://soundcloud.com/user-525053112 &         14 &    0.0133 \\ \hline
                                                                                        host | actor | writer | latina who hates flan . snap \& instagram : @graceparra360 . &           host | actor | writer | latina who hates flan . proud daughter of immigrants \& \#istandwithimmigrants . catch my healthcare doc grace anatomy on @fusion now ! &         16 &    0.1243 \\ \hline
                                                                                                                                                                    shs ' 17 &                                                                                                                                                                  yea baby &          3 &    0.0580 \\ \hline
                                                                                                                        the coolest , the truest , one of the fewest . nsu . &                                                                                                                                           here for the jokes . nsugrad🔰 . &         10 &    0.0752 \\ \hline
                                                    charlotte native , tarheels , hornets , and panthers fan . business owner and family man . love god more than yourself . &                                                                                    hi my name is tim and i get called a liberal and a fag because i disagree with trump . &         20 &    0.0355 \\ \hline
                                                                                                       github : https://github.com/bryanjos blog : http://bryaninspired.com/ &                                            the big elixir conference november 8th - 9th in new orleans : https://www.thebigelixir.com/github: https://github.com/bryanjos &         13 &    0.3080 \\ \hline
                                                                     one of a kind .... check http://chiiirp.com for my talents . art blogger at http://www.jackthriller.com &                                                                                                                                                        one of a kind .... &         10 &    0.3142 \\ \hline
                                                                                                                                                          coochie pls ma ’am &                                                                                                                                                          coochie defender &          3 &    0.3568 \\ \hline
                                                                                                                                                             i write for fun &                                                                                                                        keep your expectations low and your tolerance high &          8 &    0.0506 \\ \hline
                                                                                                                                                                    comedian &                                                                                                                                                   comedian . \\$ tonedmack &          3 &    0.0027 \\ \hline
                 nyc via nc . 1st gen somali-american muslim woman . speaker . audience development \& digital advocacy strategist . your digital hypewoman . \# actupsis 🏁💙 &                                i ’m only interested in solutions and black radical unity . | your digital hypewoman . | westside of charlotte . | brooklyn . | \#actupsis &         25 &    0.1773 \\ \hline
                                                             nwhl color analyst . beauts beat reporter , @716sportpodcast . nhl writer for fanragsports . also , dad jokes . &                                  creative services manager , @getincept . nhl writer for @diebytheblade . beer , food , \& spirits for @gustobuffalo . also , dad jokes . &         16 &    0.1680 \\ \hline
                                                                                                                                               ' ] [ ' emple university ' 18 &                                                                                                                             ' ' ] [ ' ' emple university 18 ( hopefully ) &          6 &    0.3580 \\ \hline
                                                                                                       works for topeka sod farm and greatlife golf \& fitness . father of 3 &                                                       works for mammoth sports construction , afp golf course construction . . \& kansas turf . father of 3. rock chalk . &         15 &    0.2782 \\ \hline
                                                                                                                                              just having fun in alaska .... &                                                    homesteaded for 10 years in the alaskan bush , lived in the arctic for 6 years . now i drive to walmart . no whining ! &         25 &    0.1240 \\ \hline
                  singer / rapper/drummer/skateboarder/dreamer/photographer / filmmaker / gamer \#fuckyourteam \#hexxxlife \#adversary \# tokaiartstation \# bsest93 \#lum15 &                                             vocalist / producer | for inquiries : brandonnewby1017@yahoo.com \#hexxxlife \#adversary \# tokaiartstation \# thecloudsvfers &          9 &    0.1721 \\ \hline
                                                          entrepreneur | mind body soul wellness passionista | neuro coach | hemp / cbd oil marketer | join my tribe today ! &                           mom , wife and mimi |entrepreneur | mind body soul wellness passionista | neuro , life and business coach | cbd hemp solutions for all 🌱✨🙌🏻🌎🐾 🐴 &         19 &    0.1272 \\ \hline
                                                                                                                                                                    robert ♡ &                                                                                                                                                                r ✧*:･ﾟ✧ ♡ &          2 &    0.0238 \\ \hline
                                                                                                                                            suffering - reduction enthusiast &                                       suffering - reduction enthusiast . tweets about social democracy , globalism , effective altruism , among other things . he / him . &         19 &    0.3864 \\ \hline
                                                                                                                                          nu 'est writer ' loveliest\_re n ' &                                                                                                                                                     nu 'est writer , love &          4 &    0.2042 \\ \hline
             - taken - woo tae woon ! [ yoongi is my ult ! ] - bts ( newark day 2)3/24/2017🔥-b.a.p 4/9/2017-block b 6/24/2014-g-dragon 7/27/2017-taeyang 9/6/2017-bewhy-soon &                                  i 'm a squid - bts 3/24/17 \_10/2/18\_10/3/18💣-b.a.p 4/9/17🎉-g-dragon 7/27/17🎙-taeyang 9/6/17🌼-bewhy 11/9/17🇰🇷-san e\& madclown 4/7/18 💵 &         24 &    0.2869 \\ \hline
                        \#sahm who peels oranges and distributes goldfish all day long . i also love coffee , books , wine , and cooking but not necessarily in that order . &                                                                                       interests : books , podcasts , politics , cooking , coffee , wine , and kid stuff . &         23 &    0.1957 \\ \hline
                                                 filmmaker . writer. artist . droppings of critical thought from the trail of my life . sometime contributor for @popmatters &                                                                                               i 'm a fan of things that people make and the people that make the things . &         19 &    0.0806 \\ \hline
                    the most well - intentioned mess you 'll ever meet . intern for @clevelandscene , advocate for @ppaohio / @genactionou , and avid consumer of potatoes . &                                              the most well - intentioned mess you 'll ever meet . passionate about : women 's rights , friendship , dogs , and potatoes . &         13 &    0.3545 \\ \hline
                                                                                                                              believe in yourself and aliens / sc : mintleaf &                                                                                                                                 believe in yourself and aliens / / d.y. 🌹 &          3 &    0.3807 \\ \hline
                                                                                                                                            under promise and over deliver . &                                                                                     under promise and over deliver . \#rangers\#braves\#cowboys\#sooners\#thunder\#browns &          1 &    0.3053 \\ \hline
                                                                                •it 's fun to be a follower , but you make more money as a leader• •ellet- ohio university • &                                                      •so me think , why waste time say lot word , when few word do trick - kevin• •ellet ’ 16 - ohio university ‘ 20ish • &         23 &    0.0688 \\ \hline
                                                                                    this is the place to come if you play baseball and want to get better ! ( 479 ) 595-0551 &                                           198 college signees \& 3 mlb draft picks in 6 years . this is the place players come that want to get better . ( 479 ) 595-0551 &         19 &    0.3780 \\ \hline
                                                                                                                                               virgo♍️ l snap-chelceycooper5 &                                                                                                                                            19 l snap-chelceycooper5 | jcc &          3 &    0.3258 \\ \hline
                                                                                                                                       tweets are mainly about sports \& got &                                                                                                                                      tweets are mainly about sports 🤘🏽✭ 🤠 &          2 &    0.1061 \\ \hline
                                                                                                                      professional drummer / / / make america groove again 🥁 &                                                                                                               professional drummer / / /owner of http://groovebooking.com &          6 &    0.2058 \\ \hline
                                                                                         author of eating my way to heaven , ezekiel 's mom , the happy harpist , activist . &    ezekiel 's mom , author of eating my way to heaven , harpist , comedian , activist . 🤣🎼🌊🌊🌊🌊🎼🤣let 's unite the immigrant families and house them safely on our planet ! &         22 &    0.1422 \\ \hline
                                                                                                                                                 @imp\_hq | twitch affiliate &                                                                               gm for @andromgg | former competitive call of duty player | \# theempire | twitch affiliate &         13 &    0.1371 \\ \hline
                                                                                                                            tennessee tech ' 18 | intern reed on @midday 180 &                                                                                                                                                       tennessee tech ‘ 18 &          7 &    0.3272 \\ \hline
                                                                                                                                                                happy friday &                                                                                                                                                        thanks , i hate it &          5 &    0.0070 \\ \hline
                                                                                                                                 my condolences to anyone who ever lost me . &                                                                                                               why listen to the “ streets ” ? when i ’m the main source . &         13 &    0.0383 \\ \hline
                                                                                                        \#rme \#treatedcrew \# cge booking contact merk merkmurphy@gmail.com &                                                                                           t r a p f e v e r \#rmg \#gmg \#treatedcrew booking \\$ bookbodideeder@gmail.com &         15 &    0.0396 \\ \hline
                     dm 's currently closed please email purerubydragon@gmail.com or telegram purerubydragon thanks ! fursuit account - @twerkingshep current icon - @jenkia &          currently on twitter hiatus but you can check out my instagram for some current stuff ! http://instagram.com/purerubydragon purerubydragon@gmail.com or telegram &         20 &    0.0956 \\ \hline
                                   \#honeybeez \# thehive i do n't want hope , hope is killing me . my dream is to become hopeless . when you 're hopeless you do n't care . &                                                                                                                     today is better than yesterday \#honeybeez \# thehive &         29 &    0.1273 \\ \hline
                                         lovin life as a fangirl of everything , especially taylor swift and 1d . [ be nice to everyone and do it five minutes early . - h ] &                                                                                                                                                            all the love . &         28 &    0.0210 \\ \hline
                                                                                                                         by any means necessary ! \# 2up2down \#virginiatech &                                                                                                    its a beauty in the struggle when you ’re growing inside . \# 2up2down &         13 &    0.2131 \\ \hline
       roots reggae lover - soccer fan ( real football ) - ( manchester city mcfc and barcelona fc and argentina national team ) irie ! social justice anything else ask i . &                                                                                             roots reggae music , manchester city and tulsi 2020 🤘 love is all we need !!! &         27 &    0.0154 \\ \hline
                                          photojournalist for @memphisnews , cover @memgrizz for european wire services , lover of memphis music , beer nerd \& doting dad . &                                                                                            memphis based photojournalist , lover of memphis music \& avid home - brewer . &         16 &    0.2887 \\ \hline
       i generally have a love / hate relationship with existing but at the moment i just want a nap . i also enjoy fictional worlds . \# spoonie \#overcastkid \#hufflepuff & 25 . i do n’t think i will ever “ grow out ” of my emo phase . perpetually rolling my eyes . \# localmusicmatters \#spoonie \#overcastkid \#hufflepuff \# cannabispatient &         28 &    0.2464 \\ \hline
                                                                                                                   29 . enjoy politics , weather , aviation . \# tcot \#tlot &                                                                                                          aviation , weather , politics \#scwx \#tcot \# tlot @ap4 liberty &         10 &    0.2548 \\ \hline
                               author of ya \& contemporary romance . ravenclaw + cats + snacks . rep @sarahlapolla member of @windy\_city\_rwa @sweetheartsofya \#pitchwars &      author of ya \& contemporary fiction.rep : @evascalzo member of @windy\_city\_rwa \# pitchwars blog crew ( she / her ) tis the season for love out now ! \# destiny2 &         25 &    0.3223 \\ \hline
                                         @cronkitenews reporter on @arizonapbs • @cheddaru correspondent • @cronkite\_cc president • @nlgjaasu president • 📸 : brycenewberry &                                                                                                           @kvue reporter • proud @cronkite\_asu alum • bnewberry@kvue.com &         14 &    0.0685 \\ \hline
                                                                                                                                                      grand chungus railroad &                                                                                                                                                      full stack enveloper &          3 &    0.0323 \\ \hline
                                                                                               music and hockey are my life / london is where i belong / monmouth university &                                                                                                     i love three things : music , hockey , and london monmouth university &         13 &    0.1852 \\ \hline
               @uw junior | freelance journalist | news editor @thedaily | intern @seattleweekly , formerly @ricksteves | @uwcomm | @uwjsis | coffee enthusiast | feminist . &         teaching aspiring journos as the development editor @thedaily | former intern now working at the news desk @king5 seattle | reach me at katelynmayclark@gmail.com &         21 &    0.0233 \\ \hline
                                                                                                                        insane sports fanatic ! why do i do this to myself ? &                                                                                            nhlcanes sth , tar heel alum -- huge sports fan . why do i do this to myself ? &         10 &    0.3615 \\ \hline
                     sg studios designs themed attractions featured in theme parks , retail , restaurants , children 's spaces , and entertainment venues across the globe . &                   sr. creative director-visual development for the attraction industry . working in sculpture , props , \& prototypes . oh , and i ca n't stop painting ! &         23 &    0.1152 \\ \hline
                                                                                                                                                                georgia tech &                                                                                                                                      atlanta native , georgia tech alum 🐝 &          5 &    0.0895 \\ \hline
                                                                                   wellness maven \& rockstar parallel parker married to @mindbodygreen founder @jasonwachob &                                                                                                                    founding partner \& chief brand officer @mindbodygreen &          9 &    0.1411 \\ \hline
                                                                                                                                                               super chill . &                                                              one half of your girlfriend 's favorite tag team .. \# thekoolpeople for bookings : sammy.p.deleon@gmail.com &         16 &    0.1039 \\ \hline
                                                              founded by wes jackson . perennial polyculture \& natural systems agriculture for people , land \& community . &        founded 1976 . global partnerships . creating agriculture that mimics natural systems to produce ample food \& reduce negative impacts of industrial agriculture . &         19 &    0.1987 \\ \hline
                                                    archaeologist living in new orleans , attending tulane university , and working in the puuc region of yucatan , mexico . &                                            anthropological archaeologist | new orleans | tulane university | inequality in prehistory | anthropology of sports | luchador &         15 &    0.1132 \\ \hline
                                                                                                                                           girl next door with big dreams ❤️ &                                                                                                                ♍️girl next door with big dreams \& things ❤️ @arryoppy 💍🖤 &          5 &    0.3789 \\ \hline
         | 21 | cowboys nation sc : nathan0412 - everything i like is either expensive , illegal , or do n't text back / bp gator / ig : @its\_nathan\_green ford 7.3 on 40s &                                        | 21 | cowboys nation ! there is a special place in hell for people who waste good whiskey .ig : @its\_nathan\_green renee is my 🌎 &         26 &    0.2251 \\ \hline
                                                                                                                            news and updates from google for entrepreneurs . &                               google for startups brings the best of google 's products , connections , and best practices to enable startups to build something better . &         22 &    0.1776 \\ \hline
                                                                                                                                  find what you ’d die for and live for it . &                                                                                                                                                 libra sun . black power . &         10 &    0.0731 \\ \hline
                                                                                                                senior| 17 | not looking , so do n't bother .xvii-ix-mmxv .❣ &                                                                                    senior | do n't let your happiness depend on something you may lose . | 17 . | \# ht20 &         20 &    0.0549 \\ \hline
                               ⭐️ nicolette / yirico • costumer / seamstress • i love axel • she / her / your majesty • support me on ko - fi : http://ko-fi.com/a1632mwy ⭐️ &         ⭐️ nicolette • professional costumer • i love axel • she / her / your majesty • wishlist : https://www.amazon.com/hz/wishlist/ls/2jlwx0l8w8f3s?ref\_=wl\_share ⭐️ &         12 &    0.3040 \\ \hline
        geek girl blogger , @geekgirlsrising , injured production assistant , future film student , film tech , gamer , super hero \& comic book nerd . tv \& movie addict . &                                                 artist , documentary film maker . addicted to film , tv and comics. , locations , research , writer \& opinionated geek , &         26 &    0.1201 \\ \hline
                                   sales gal @sigstrapp | city girl w/ a small town soul | interior designer | proud @butleru and @linkedin alum | oh , and my dog is famous &           sales gal @salesforce | social media guru | safer beauty advocate @beautycounter | dog momager | living a life full of grace | proud @butleru \& @linkedin alum &         24 &    0.2811 \\ \hline
                                                                                          do n't let twitter become your life . @eagles @sixers @phillies ig : eagles\_chica &                                                                                                                                                           @sixers @eagles &         13 &    0.2420 \\ \hline
                                                                                                                                       mia , ny ✈️ drautomotive professional &                                                                                                                                                   automotive professional &          5 &    0.2076 \\ \hline
                                                                                                                                                                   now being &                                                                                                                                                                     being &          1 &    0.2113 \\ \hline
                                                                             \#teamzayn . i actually saw the boys on 10/05 / 14 for wwa , pinch me i still think im dreaming &                                                                                                                       \#teamzayn . i'm honestly just winging through life &         19 &    0.2151 \\ \hline
\bottomrule
\end{tabular}



==> chapter4-BiosModification/Figures/twitter_bios_raw_chunk/2.tex <==
\begin{tabular}{p{0.38\textwidth}|p{0.38\textwidth}|p{0.04\textwidth}|p{0.1\textwidth}}
\toprule
                                                                                                                                                                      Before &                                                                                                                                                                                                                                                 After &  Edit Dis. & BERTScore \\ \hline
\midrule
 band manager @xangelxanatomyx , social media strategist at https://t.co/iwhttjqwwa, notary public \& courier at advanced title past : anime banzai and omniture \# bearclan &                                                                                                                                                                            band manager @xangelxanatomyx past : anime banzai and omniture \# bearclan &         13 &    0.4762 \\ \hline
                                                                           happiness can be found even in the darkest of times if one only remembers to turn on the lights . &                                                                                                                           happiness can be found even in the darkest of times if one only remembers to turn on the lights . rip blackjack 5-29-2017 💙 &          4 &    0.7144 \\ \hline
                                                                                                          independent intelligence analyst seeking to get the truth to power &                                                                                                          independent intelligence analyst seeking to get truth to power . have evidence trump election was coup.need help telling senate 312-664-2631 &         12 &    0.4528 \\ \hline
\# [ ] \_ [ ] alum ( 2008 ) , bs.ed major in sports admin . - m.s. sports admin. from st.thomas u ( 2011 ) - current sports writer . hopefully a english teacher this fall ! &                                                                                           \# [ ] \_ [ ] alum ( 2008 ) , bs.ed major in sports admin . - m.s. sports admin. from st.thomas u ( 2011 ) current substitute teacher @ two private schools &         11 &    0.7728 \\ \hline
                                                                                                                               fishing guide and father ... neither is a job &                                                                                                                                   fishing guide and father ... neither is a job . love god , family , the usa , and that ride down the laguna madre ! &         17 &    0.5558 \\ \hline
                                                                        be the change you want to find in the dryer tumblr \& instagram : rachelshapshak snapchat : crabshak &                                                                                                                                                             be the change you want to find in the dryer insta : rachelshapshak // snapchat : crabshak &          4 &    0.7583 \\ \hline
               reppin ' \#eaglesnation since birthphilly 's home \& is in my blood \# 4 for4 philly sports fan\#dubnation fan ( since ' 90 ) \# athletics fan ( since ' 95 ) &                                                                                             reppin ' \#eaglesnation since birth \# 4 for4 philly sports fan\#dubnation fan ( since ' 90 ) \# athletics fan ( since ' 95 ) cash app : \\$ khrisphuego85 &         13 &    0.6082 \\ \hline
                                                                                                        coach - \# always100 2025 elite .... husband , and dad .... my views &                                                                                                                               coach - \# always100 elite 2025 .... husband , business owner , and dad .... my views http://www.always100elite2025.com &          6 &    0.4793 \\ \hline
                                                                                                                                             making sounds in @nocturnal\_mo &                                                                                                                                                                               making sounds in @nocturnal\_mo . a major disappointment to my family . &          8 &    0.6975 \\ \hline
             award - winning ny playwright @ 29thstplaywrights @articulatetc @oraclesnyc @dramatistsguild @sexyplaywright @icwp @lptwomen @newplayx @havescripts @youthplays &                                                                                                        playwright . @29thstplaywrights @oraclesnyc @dramatistsguild @sexyplaywright @icwp @lptwomen @newplayx @havescripts @youthplays @dramanotebook &          8 &    0.6458 \\ \hline
  pastor city church gainesville , director for bridge the city . \# waytoospiritualwednesday enthusiast , jesus \& justice . we 're all in this together ! \# kingdomminded &                                                                                       director for bridge the city . \# waytoospiritualwednesday enthusiast , jesus \& justice . pastor and preacher . we 're all in this together ! \# kingdomminded &          9 &    0.7388 \\ \hline
                                                 follower of god , husband , military vet , m.ed . instagram : 2tmorris3 \# dav \# cowboynation \# mavsnation \#rangernation &                                                                                                   follower of god , husband , military vet , m.ed . instagram : petty2 chains \# dav \#cowboynation \# mavsnation \#rangernation snapchat : tmorris23 &          7 &    0.6747 \\ \hline
                                                                                                         books.baseball . beer. social work student . you 'll need me soon . &                                                                                                                                                                                                 books.baseball.beer.bsw 2015 . you 'll need me soon . &          6 &    0.5065 \\ \hline
                                                                                                                                                         foot lover in pa !😋 &                                                                                                                                                                             foot lover in pa!😋nsfw 18 + the above photo is of the amazing @thetetra69 &         11 &    0.4261 \\ \hline
                                        wife of the world 's best husband mother of usc upstate soccer player , fmu soccer player , irmo basketball player and young scholar &                                                                                                            wife of the world 's best husband mother of uw gradstudent , univ . of sc soph . , limestone college basketball commit and young scholar . &         13 &    0.4039 \\ \hline
                                            associate at lowry johnson / goldstein casting . chicagoan living the la life . hella gay . views are my own , obvi ( he / him ) &                                                                               associate at lowry johnson / goldstein casting . chicagoan / angeleno . black lives matter . roseanne called me a “ bigoted toad ” once . views are my own ( he / him ) &         17 &    0.5133 \\ \hline
             architecture , planning , urban design . walkable communities and livable streets . \# fixthestreet . veritas . \#resist . \# slc // @realsaltlake // \# goutes &                                                                                                     architecture , planning , urban design . walkable communities . livable streets . \#register \#vote 🗳 . \# slc // @realsaltlake // \#2020iscoming &          9 &    0.6045 \\ \hline
                                                    ✌❤☺ player of alistriona the mage on aie / er \& ctr / ap [ icon art by @samaramon ] | @habantdark is my paladin irl ; d &                                                                                                                     ✌❤☺ player of cara the mage in @ctrguild \textasciitilde{} icon art by @samaramon \textasciitilde{} @habantdark is my paladin irl &         14 &    0.5719 \\ \hline
                                                                                                                                                  coder , gamer , musician . &                                                                                                                                                                                                                 coder , gamer , musician , he / him . &          4 &    0.7251 \\ \hline
                                                                    helping small business get teh most out of social media http://muchsocial.com. find me also @billgelwick &                                                                                                                      we are passionate about helping small business get the most out of social media http://muchsocial.com. find me also @billgelwick &          5 &    0.7676 \\ \hline
        ao is recognized as the premier international association for implant dentistry professionals . \# trendingtopic articles do not necessarily reflect ao 's opinion . &                                                                                   ao is recognized as the premier international association for implant \# dentistry professionals . \# aoconnect articles do not necessarily reflect ao 's opinion . &          2 &    0.7707 \\ \hline
                                                                                                                    too interested in too many things to be good at anything &                                                                                                                                  ex - challenger / ex-global / ex-everything just a casual - too interested in too many things to be good at anything &         11 &    0.4669 \\ \hline
                                                               i can do all things through christ which strengtheneth me philippians 4:13 ⓜ️obbrother® ( mbs ) class of 2015 &                                                                                                                                                       i can do all things through christ which strengtheneth me philippians 4:13 ⓜ️obbrother® ( mbs ) &          3 &    0.5102 \\ \hline
                                                                                                                                              i'm just a boy who loves mechs &                                                                                                                                                                                                  i'm just a boy who loves mechs and @lauraxreynolds 💙 &          3 &    0.5062 \\ \hline
                                                                     23. married ( 5/26/12 ) , then came lily ( 5/3/13 ) and isaac ( 11/19 /14 ) expecting again ( 5/22/16 ) &                                                                                                                                                   24. married ( 5/26/12 ) , then came lily ( 5/3/13 ) , isaac ( 11/19 /14 ) and elijah ( 5/16/16 ) ❤️ &          6 &    0.7781 \\ \hline
      country music fan , family is everything , \& i love my friends . god has really blessed me :) huge chris young fan ! been an aaron carter \& nick jonas fan for yrs . &                                                                                                                family is everything . i love my friends . god has really blessed me :) huge chris young fan ! \#rodeo \# countrymusic \#houstontexans &         17 &    0.4020 \\ \hline
                   media contributor | clinical psychologist | exec director - the center for emotional health , specialist in anxiety , ocd , \& bfrbs / trichotillomania . &                                                                            clinical psychologist | executive director - the center for emotional health of greater phila . ( ceh ) specialist in evidence - based tx of anxiety , ocd , ts , \& bfrbs &         21 &    0.4445 \\ \hline
   i 'm a humanist . i'm passionate about psychology and have written about / worked in it , k- 12 ed and tech . i love people and being outside . i 'm following my bliss . &                                                                                                                                            web developer . future psychologist . editor . i love people and being outside . i 'm following my bliss . &         22 &    0.5015 \\ \hline
                            small lady , firm handshake - @ny1 reporter - @columbiajourn alumna - formerly @krnv @kfyr @cnn - represented by @unitedtalent - gnome collector &                                                                                                                              small lady , firm handshake - @abc10 reporter @columbiajourn - formerly @ny 1 @cnn @krnv @kfyr - repped by @unitedtalent &         11 &    0.6449 \\ \hline
                                            believer / substitute teacher / baristaaspiring teacher , former sports reporter , semi-amateur softball player . i tweet sports &                                                                                                                                                 believer / 4th grade teacher / former sports reporter / semi-amateur softball player . i tweet sports &          6 &    0.5572 \\ \hline
                                                                                                                                                alpha chi omega • iupui ' 19 &                                                                                                                                                                                                                              panhellenic • iupui ' 19 &          3 &    0.4315 \\ \hline
                                  mom of 5 ... teacher educator ... believer in strong public schools , teacher professionalism , and developmentally appropriate learning . &                                                                                                                                                                                mom of 5 ... teacher educator ... public school advocate ... iowa girl &         13 &    0.4547 \\ \hline
              just a girl , loves to write \& inspire others with my passion for tarot storytelling . infp • ☀️ ♊ • 🌙 ♏ • asc ♎ • dom planet ♇ • sign ♏ • element 🌊 shawol 💎 &                                                                                                 i love to write \& inspire others with my passion for tarot storytelling . voice actor 🎤 in training . mom of 1 furbaby . infp • ☀️ ♊ • 🌙 ♏ • asc ♎ • &         25 &    0.4193 \\ \hline
                                                                                                                                  isaiah 54:10 | @grant\_\_brady says i'm ok &                                                                                                                                                                                      atx to abi to cstat | isaiah 54:10 | @grant\_\_brady says i'm ok &          6 &    0.4475 \\ \hline
                                                                                                        dbu patriot , guitarist , worshipper of jesus christ , texas forever &                                                                                                                                                                         dbu patriot alum , guitarist , worshipper of jesus christ , texas rangers fan &          3 &    0.6986 \\ \hline
                                                                                                     abc news producer . photographer . my favorite superhero is lois lane . &                                                                                                                                                                       producer . photographer . @abc news alum . my favorite superhero is lois lane . &          6 &    0.7060 \\ \hline
                                                                                              praying 🙏🏾 , growing 🌻 , glowing ✨. que sera , sera . \# vsu19 slot ! ah🔺 1913 &                                                                                                                                                                            vsu alumna |🔺 1913 | praying 🙏🏾 , growing 🌻 , glowing ✨. que sera , sera . &         11 &    0.6067 \\ \hline
                                                                                                                                          yeet or be yeeten | angsty barista &                                                                                                                                                                                                     yeet or be yeeten | angsty cat mom of your dreams &          5 &    0.6549 \\ \hline
                  the best ragna player you 've never heard of|exhausted protagonist|professional masher|see me in groove coaster|sam walton 's fav slave|psn : xentrinal 17 &                                                                                                          the best ragna player you 've never heard of|exhausted protagonist|morally gray|see me in groove coaster|ultimate underdog|psn : xentrinal17 &          9 &    0.7439 \\ \hline
                                                                                                                                                         i do n’t eat meat 🌹 &                                                                                                                                                                                                                            i do n’t eat meat 🌻 \# blm &          3 &    0.7360 \\ \hline
            daughter of the king 🇺🇸🇮🇳 artist @epic\_records @sonymusicindia || grammy nominated songwriter @pulserecording \# thecomeup \# cityslums bookings@rajakumari.com &                                                                                                                                                                                              daughter of the king 🇺🇸🇮🇳 bookings : info@rajakumari.com &         13 &    0.4716 \\ \hline
                                                                                                               director || playwright || the end of fear is where we begin . &                                                                                                                                                                   director || playwright || " i am an echo of the eternal cry of ' let there be ! ' " &         15 &    0.4716 \\ \hline
                                                                                i like 'em brown , yellow , puerto rican and jamaican my name es-ko from tha lucian nation . &                                                                                                                                     i like 'em brown , yellow , puerto rican and jamaican my name es- ko from tha lucian nation .🇱🇨💟 blacklivesmatter &          4 &    0.6405 \\ \hline
                                                                                                                                     87 pieces of wood - woodchuck l( iv ) e &                                                                                                                                                                                                                         87 pieces of wood - woodchuck &          4 &    0.4995 \\ \hline
 jenny : solve crimes . vastra : protect the empire . jenny : there 's quite a lot of running . vastra : \& some spectacular dresses . strax : so dresses then ! @rycbar1963 &                                                                          eng lit major . jenny : solve crimes . vastra : protect the empire . jenny : there 's quite a lot of running . vastra : some spectacular dresses . strax : so dresses then ! &          6 &    0.6666 \\ \hline
  española , mom , \# foodie , winelover , geek , traveler , girlscoutleader , \#ibmer \#ibmcloud \# marketing , capture life in snapshots , austinite , tweets are my own ! &                                                                                          española 🇪🇸 , mom , \# foodie , winelover , geek , traveler , \#marketing @ rackspace , girlscoutleader , ibm alumni , capture life in snapshots , austinite &         14 &    0.4297 \\ \hline
                                                                                                                   || westminster soccer \# 7 ⚽️ || @hancockhazen ||focus st &                                                                                                                                                                                                || westminster soccer \# 7 ⚽️|| focus st || ia 319 ✈ ️ &          7 &    0.4091 \\ \hline
                                           saluki alum , hr professional , and history enthusiast who lives in sw florida . proud baseball and volleyball mom . go cubs go ! &                                                                                                                     saluki alum , hr professional and history buff who lives in fl with my love ❤️ . proud baseball and volleyball mom . go cubs go ! &          7 &    0.6644 \\ \hline
                 4th grade teacher , technology leader , edulastic innovator team , donors choose teacher ambassador , mastiff lover , golfer , denver bronco fan ! \#edtech &                                                                                   4th grade teacher in oregon , technology leader , edulastic innovator team , donors choose ambassador , classroom champions ambassador denver bronco fan ! \#edtech &          8 &    0.6764 \\ \hline
                                                                                                                                   it is well✨ \# blancaarismendiphotography &                                                                                                                                                                                    it is well || free chapel college || \# blancaarismendiphotography &          6 &    0.6737 \\ \hline
                                                                                        proud husband | father | drag racing | pro wrestling | \# bbn| \# browns | \# cavs | &                                                                                                                                                                                           proud husband | father | drag racing | \# cavs| \# browns | &          7 &    0.5474 \\ \hline
                                                              college hockey player at university of arizona , from greensboro , nc. sports reporter for http://goazcats.com &                                                                                     retired college hockey player @universityofarizona , from greensboro , nc. jack of all trades covering @aplayersprogram and @arizonafball at http://goazcats.com. &         15 &    0.4307 \\ \hline
                                                                                                                            |unl ‘ 20 | business admin| @davisjasen | co➡️ne &                                                                                                                                                                                                                     |unl ‘ 20 | business admin co➡️ne &          3 &    0.6733 \\ \hline
             work hard !!! sprints / jumps coach for hammonton boys track / field 💙 music 🎶 live music 🎤🎶 basketball🏀 family / friends / pups / gecko 🐾 yoga / meditation 🕉💜 &                                                                                                                                   proud sprints / jumps coach for hammonton boys track / field 💙 music 🎶 family / pups / gecko 🐾 yoga / meditation 🕉💜 &          9 &    0.7248 \\ \hline
                                                                                                        ph.d. media scholar , web designer , psychic detective ( retired ) . &                                                                                      ph.d. media scholar , web designer , psychic detective ( retired ) . to be absolutely clear : i tweet on behalf of no one but myself . all opinions are my own . &         21 &    0.4713 \\ \hline
                                                          i 'm not superstitious , but i am a little stitious ... karsten creek golf shop guy , retired donut chef \#okstate &                                                                                                                                                           i 'm not superstitious , but i am a little stitious ... retired do nut chef ok state alum 🍊 &         10 &    0.5552 \\ \hline
                                                i 'm chris , single , straight , lover of all people and would love a ts girlfriend call , text or whatsapp + 44 7519 752058 &                                                                                                                                                                 i 'm chris , straight , sexually open-minded call , text or whatsapp + 44 7519 752058 &         12 &    0.6802 \\ \hline
                                                                    father of 4 , fantasy football geek , wolfpack fan , soccer coach , poker player and aspiring novelist . &                                                                                              father of 4 , fantasy football geek , wolfpack fan , soccer coach , poker player and aspiring novelist \& sometime contributor to http://cardiaccane.com &          5 &    0.7450 \\ \hline
                                                           uofl alum ( sae ) , miami rep - uf grad - environmental consultant , empire waste and logistics consultants , llc &                                                                            uofl alum ( sae ) , miami alumni rep - uf grad ( mba ) - empire waste and logistics consultants , llc . youth ⚾️ coach , msv marlins \& danny berry miami beach thunder⚡ ️ &         19 &    0.4316 \\ \hline
                                                                                                                                contorting verbosity into lyric and dialogue &                                                                                                                                                                                                                    contorting verbosity into libretto &          3 &    0.6761 \\ \hline
                                              father . geek . award - winning journalist , security researcher . taking some time to do other projects . tweets are my own . &                                                                                                             father . geek . former award - winning journalist , now a security researcher . board of directors at circlecitycon . tweets are my own . &         10 &    0.6402 \\ \hline
                                                                                                                                               senior • cathedral highschool &                                                                                                                                                                                                                     jn• senior • cathedral highschool &          1 &    0.5794 \\ \hline
                                                             labrador , anthony || mediocre photographer . || life is a bitch then you die || team @nike || @anthonylabphoto &                                                                                                                                             labrador , anthony || mediocre photographer . || team @nike || @anthonylabphoto || adventure is out there &         11 &    0.7043 \\ \hline
                                                                                                        life is like a box a chocolate , you never know what you gonna get . &                                                                                                                                                                              " life is like a box a chocolate , you never know what you gonna get . " &          2 &    0.7923 \\ \hline
                                                                                    grb class of ' 13 . lmc class of ' 17 . esf class of ' 18 . sustainable energy student . &                                                                                                                               grb class of ' 13 . lmc class of ' 17 . esf class of ' 18 . commercial consultant for nyserda ( opinions are my own . ) &         10 &    0.5811 \\ \hline
                                                             host , - http://nratv.com the mission is to expose idiocracy . ( views are my own , feel free to adopt them . ) &                                                                                                   radio and newsmax tv host . nra member and \# maga champion . the mission is to expose idiocracy . ( views are my own , feel free to adopt them . ) &         12 &    0.5532 \\ \hline
                                                                                             death to anybody that oppose my spirit ig - @toe . kneeee sc- walelovesme \#tsu &                                                                                                                                                           death to anybody that oppose my spirit . tennessee state . ig - toe. kneeee sc- walelovesme &          7 &    0.6536 \\ \hline
                                                                                                                  today 's agenda : medicare for all and class consciousness &                                                                                                                   today 's agenda : medicare for all and class consciousness . some rts about sri lanka . @simonsrock alumna , @cunyjschool currently &         12 &    0.4761 \\ \hline
                                                                                                               \#blacklivesmatter||\#lgbtlivesmatter||sc:maddieelkins||ryan❥ &                                                                                                                                                                             \#blacklivesmatter|||\#lgbtlivesmatter|||be kind to every kind|||ttu ‘ 24 &          7 &    0.4023 \\ \hline
                  average student at weber state . seattle to salt lake . it 's all about the experience . 16 front / 21 main megapixel sony xperia xa ultra . go wildcats . &                                                                                                                         weber state graduate . seattle to salt lake to detroit . it 's all about the experience . sony xperia 10 plus . go wildcats . &         14 &    0.5354 \\ \hline
                                                               official twitter account of the @nahl new jersey titans \# breakingtheice tix@njtitanshockey.com 888-997-goal &                                                                                                                  official twitter account of the @nahl new jersey titans \# breakingtheice • tickets call ( 732 ) 856-9700 • \#njtpuck \#titansnation &         10 &    0.4515 \\ \hline
                                                                                        plz follow me ask for a follow back my facebook cassia evans my instagram cassiae 21 &                                                                                                                                                                                                      my facebook cassia evans my instagram cassiae 21 &          8 &    0.5260 \\ \hline
 †loving jesus† i am happily married to @meredithartner . she is the love of my life †serving god where i can† \# maga \# 1 a \# 2a \#notpoliticalcorrect \# trump2020 \#nra &                                                                              †loving jesus† i am happily married to @meredithartner . she is the love of my life †serving god where i can† \# maga❌\#1a❌\#2a❌\#notpoliticalcorrect❌\#trump2020❌\#nra❌ &         10 &    0.7375 \\ \hline
                                           learn how to grow 4c hair here : https://blackhairomg.net/how-to-get-perfectly-soft-manageable-type-4-hair-the-mane-choice-clover &                                                                                                                                                                 learn how to grow 4c hair here : https://www.naturalhair-products.com/coily-hair.html &          1 &    0.4295 \\ \hline
                                                                                                                     \#livinghealthy youtuber : https://youtu.be/djiuhfepqi8 &                                                                                                                                                    \#livinghealthy youtuber link to my most recent video always in bio : https://youtu.be/ffso3ionfeq &         10 &    0.5183 \\ \hline
                                                                   preparing high -potential , underserved high school students for top-tier college admission \& graduation &                                                                                                    we prepare more than 1,200 high - potential students from underserved communities to apply , attend and graduate from the nation 's top colleges . &         23 &    0.4312 \\ \hline
                                                            there is no track 9 . there is no track 13 . i make french house music and play games . usually the latter tho . &                                                                                                        there is no track 9 . there is no track 13 . i make french house music and play games . usually the latter tho . 27 , she / her or they / them &          9 &    0.7343 \\ \hline
              voice artist | writer | gamer | streamer | pansexual gender - fluid femme . cast member on @questsandchaos . \# ttrpg has become my life ! won \#nanowrimo2019 &                                                                                 voice artist | writer | gamer | streamer | pansexual gender - fluid femme . cast member on @questsandchaos and misty on @rollforweird . \# ttrpg has become my life ! &          6 &    0.7354 \\ \hline
       disc makers ' official twitter . we stand alone as the undisputed leader in optical disc manufacturing for indie artists , filmmakers , and businesses . since 1946 ! &                                                                               disc makers ' official twitter . we stand alone as the undisputed leader in optical disc manufacturing for \#indieartists , filmmakers , and businesses . \# discmakers &          5 &    0.7607 \\ \hline
                                                                love playing video games , good food and motorcycle rides w/ husband mark @ivson1 cvi retired police officer &                                                                                  love playing video games , good food and motorcycle rides w/ husband mark @ivson1 cvi he is a retired police officer . have 3 beautifu daughters and 6 grandchildren &         11 &    0.6826 \\ \hline
                                                                                                                            psych student . i follow back . ig ; melissacgmz &                                                                                                                                                                                                                      i follow back . ig ; melissacgmz &          3 &    0.7235 \\ \hline
                     since 2004 , pvhs has won 98 league championships , 17 cif championships , 28 cif academic team championships and 4 state championships ! \# beaseaking &                                                                                                                                since reopening in 2002 , pvhs has won 102 league , 19 cif , 28 cif academic and 5 state championships ! \# beaseaking &         10 &    0.7195 \\ \hline
   social media manager @katunews . previously @huffpostlive . franco-american producer . emmy award winner . afi \& berkeley alumn . views\textbackslash{}tweets are my own & multimedia producer / social media manager - prev @katunews @huffpostlive\textasciitilde{}emmy award winner\textasciitilde{} afi\&berkeley alumn\textasciitilde{}og parisienne / true angeleno\textasciitilde{}views\textbackslash{}tweets are my own &         20 &    0.4853 \\ \hline
                                                                                              su ' 20 ig : aesthetic\_ . \_genetics sc : myaaa\_m tumblr : aesthet1cgenetics &                                                                                                                                                                                                   su ' 20 ig : aesthetic\_ . \_genetics sc : myaaa\_m &          3 &    0.6629 \\ \hline
                                                                                                                                                     i do makeup sometimes . &                                                                                                                                                                                                           i do makeup sometimes . / ig : jc. beautyyy &          5 &    0.5463 \\ \hline
                                                                                                                                                               dad 👼🏼 cml 👼🏼 &                                                                                                                                                                                                                          dad 👼🏼 cml 👼🏼 👻-tylergrammer &          1 &    0.6576 \\ \hline
                                                                            researcher , lover of people , conversationalist , creative . http://welcometomyrehab.tumblr.com &                                                                                                                                                         spoken word artist | blogger | media personality | friend 🤗http://welcometomyrehab.tumblr.com &         11 &    0.4869 \\ \hline
                                                                            arsenal fan in america . loves web design , scotch whisky , mesut özil , and low - brow comedy . &                                                                                                    web developer . father . arsenal fan in america . love scotch whisky , mesut özil , and low - brow comedy . just another asshole with an opinion . &         16 &    0.6254 \\ \hline
                                    managing editor at @mwcconnection | @thesfjournal | @twinfallstn columnist | royal jay | two - time march classic champion : 2017 , 2018 &                                                                                          managing editor at @mwcconnection | @thesfjournal | @twinfallstn columnist | two -time march classic champion : 2017 , 2018 | sem / seo manager at @kountinc &         12 &    0.7208 \\ \hline
                                     digital advertising @condenast | \#luxuryfashion sponge . croptop queen . @newhousemasters guided me to become the jill of all trades . &                                                                                                                             digital girl @condenast | \#luxuryfashion sponge . croptop aficionado . @newhousemasters grad flying with her own wings . &         11 &    0.4620 \\ \hline
                                                                                                                        do n't say i never gave you anything . \# teamlebron &                                                                                                                                                                                                        do n't say i never gave you anything . \# tolo &          1 &    0.7893 \\ \hline
                                                                                                 23 . i retweet a lot . \# bb19 \# britneyarmy \# lorde \# teamtinashe \#nyr &                                                                                                                                                                                               i retweet a lot . \# bb20 \#nyr britney / lorde/tinashe &         10 &    0.5250 \\ \hline
                                                                                               + twitch streamer + 24hr stream king + pvp is life .. but pve is alright .. + &                                                                                                                                                         + twitch streamer + 24hr stream king + on a streaming break + bassist in hostile masquerade . &         10 &    0.4001 \\ \hline
                                                                       adoring husband to the beautiful @jsksnnnb . proud stepfather . bleeds orange \& blue . \#lgm \# mets &                                                                                                                    adoring husband to the beautiful @jsksnnnb . proud stepfather to bryson and daddy to anakin . bleeds orange \& blue . \#lgm \#mets &          8 &    0.7531 \\ \hline
                                                        sales . student . husband . assistant coach @ bghs . head coach 8th @ bgjhs . \# bbn \#tops \# cowboysnation \# cubs &                                                                                                 husband . general manager @ anytime fitness . full time student . head bball coach @bgjhs . assistant @ bghs . \# bbn \#tops \# cowboysnation \# cubs &         15 &    0.5673 \\ \hline
                                                                                                                             missouri state university - world record holder &                                                                                                                                                                                                                             missouri state university &          4 &    0.5837 \\ \hline
                                                                                             finding solutions that will help resolve the problems facing our planet today . &                                                                                                                                                       husband , father and entrepreneur . finding solutions to the problems facing our planet today . &          9 &    0.4990 \\ \hline
                                                                                  common ground bar \& grill , a gastropub serving the allston community for over 16 years . &                                                                                                                                                                                common ground bar \& grill served the allston community for 16 years . &          5 &    0.7882 \\ \hline
                                                                                                                                                     ||•proverbs 31:25 • | | &                                                                                                                                                                                                                             🌻 ||•proverbs 31:25•| | 🌻 &          4 &    0.5727 \\ \hline
                                                                                                                     lupus advocate , public speaking , consulting , charity &                                                                                                                                                                                            lupus advocate , public speaking , consulting , aapac tvhs &          2 &    0.6060 \\ \hline
\bottomrule
\end{tabular}



==> chapter4-BiosModification/Figures/twitter_bios_raw_chunk/3.tex <==
\begin{tabular}{p{0.38\textwidth}|p{0.38\textwidth}|p{0.04\textwidth}|p{0.1\textwidth}}
\toprule
                                                                                                                                                                                                                         Before &                                                                                                                                                                                                                         After &  Edit Dis. & BERTScore \\ \hline
\midrule
                                                                                                                                                                 literary agent interested in finding what a book wants to be . &                                                                                                                                         literary agent interested in finding what a book wants to be . authors guild member . &          4 &    0.8813 \\ \hline
                                                                                                                                                                                                        so it goes|fl st8|20|♊️ &                                                                                                                                                                                                      so it goes|fl st8|21 |♊️ &          2 &    0.9715 \\ \hline
                                                                                                                  jcsu alumni ' 14 \# lead by faith , follow by trust \# jhs \#fnf \#gbulls \#riseup 2011 pioneer bowl champion &                                                                                                                 jcsu alumni ' 14 \# lead by faith , follow by trust \#aflete \#fnf \#gbulls \#riseup 2011 pioneer bowl champs &          3 &    0.8206 \\ \hline
                                                                                                                          live updates of jac and sheldon 's race schedule and results . http://facebook.com/haudenschildracing &                                                                                                                      live updates of jac \& sheldon 's races , schedule , \& results . http://facebook.com/haudenschildracing &          5 &    0.8300 \\ \hline
                                                             indian \& nepalese cuisine 899 s plymouth ct . chicago downtown , lunch buffet , dine in , carry out , delivery , cateringph - 312 362 9999 http://t.co/mnhu31uwkn &                                                                 taste of himalayan . 899 s plymouth ct . chicago downtown , lunch buffet , dine in , carry out , delivery , catering ph - 312 362 9999 http://t.co/mnhu31uwkn &          6 &    0.8105 \\ \hline
                                                          author , alternative hip hop / spoken word artist and producer . 1 / 2 of @darkalleyechoes . inquire : drowning.ophelia.ent@gmail.com . music : https://goo.gl/7pwv2r &                                                                    author , alt . hip hop / spoken word artist , producer . 1 / 2 of @darkalleyechoes . booking : drowning.ophelia.ent@gmail.com music : http://goo.gl/7pwv2r &          6 &    0.8562 \\ \hline
                                                                                                                                                         there 's beauty in the struggle , ugliness in the success . \# armyvet &                                                                                                                                       there 's beauty in the struggle , ugliness in the success . \# armyvet \# cowboysnation &          2 &    0.8912 \\ \hline
                                                                               artist . writer . traveler . @nutmeganimals founder . @patriots journalist . musician . authoring an african safari memoir . instagram : e\_scal &                                                                   artist . writer . traveler . @nutmeganimals founder . @patriots journalist . musician . aesthete . authoring an african safari memoir . instagram : e\_scal &          2 &    0.9017 \\ \hline
                                                                      veteran of the marines . huge football fan , supporter of denver broncos \& wvu . avid gamer , paranormal enthusiast , and supporter of the pride of wv . &                                                                   veteran of the marines . huge football fan , supporter of denver broncos \& wvu . avid gamer , paranormal enthusiast , and fan of everything walking dead . &          5 &    0.8126 \\ \hline
                                                                                                                                             dc via buffalo . \#immigrantheritagemonth . \# iamanimmigrant . \# jlwvol @jlwdc . &                                                                                                                    dc via buffalo . \#immigrantheritagemonth , \#istandwithimmigrants , \#iamanimmigrant . \# jlwvol @jlwdc . &          4 &    0.8460 \\ \hline
                                                          artist . photographer . fashion lover . constant reader . watcher of movies . traveler on this road called life . feet on the ground , eyes looking up at the stars . &                                                                         artist . photographer . constant reader . watcher of movies . traveler on this road called life . feet on the ground , eyes looking up at the stars . &          3 &    0.9161 \\ \hline
                                                                                                                      join over 58,000 awesome pokemon fans and subscribe to us on youtube at http://youtube.com/thepokecapital &                                                                                                                     join over 60,000 awesome pokemon fans and subscribe to us on youtube at http://youtube.com/thepokecapital &          1 &    0.9912 \\ \hline
                                                       the home of heidelberg university football . 1972 stagg bowl champions . seven time oac champion . over 40 all - americans and 5 academic all - americans . \# bergpride &                                                      the home of heidelberg university football . 1972 stagg bowl champions . seven time oac champion . over 50 all - americans and 6 academic all - americans . \# bergpride &          2 &    0.9881 \\ \hline
                                                                            former  , current  consultant running marketing / branding @bebitech | 🤴 of @sonyrumors | 💚er of 🇩🇪 / ⚽️ / 🐱 /☕️ | 🤓 for @bmw / @marvel / fashion &                                                             former  , current  consultant running marketing / branding @bebitech | 🤴 of @sonyrumors | 💚er of 🇩🇪 / ⚽️ / 🐱 /☕️ | 🤓 for @bmw / @marvel / fashion \# fuckcancer &          2 &    0.9222 \\ \hline
                                                                                                                                                 \#abolishice \#abolishprison \#abolishpolice ✨ chercher . espérant . croître . &                                                                                                                                       \#abolishice \#abolishprison \#abolishpolice✨ chercher . espérant . croître . she / her &          5 &    0.8772 \\ \hline
                                                                               the trials of life will make you either bitter or better . mi to fl. ✈️ follow me on instagram : pchammond kik : pchammond snapchat : det4life15 &                                                                                          the trials of life will make you either bitter or better . mi to fl. ✈️ follow me on instagram : pchammond and snapchat : det4life15 &          3 &    0.8531 \\ \hline
                                                                                                     writer , content creator , videomaker . former tv journalist . seattle native , syracuse \& university of florida alumni . &                                                                                                                           writer , content creator , videomaker . seattle native , syracuse \& university of florida alumni . &          4 &    0.8702 \\ \hline
                                                                                                                                                                                                   b a y a r e a ✈️ la ✈️ nyc | &                                                                                                                                                                                                | b a y a r e a ✈️ la ✈️ nyc | &          1 &    0.9250 \\ \hline
                                                                   corporate recruiting guy , rugby coach \& jam band music phan who loves making a difference . always be connecting , is my mantra . \#recruiting \# sourcing &                                                        corporate recruiting guy , rugby coach \& jam band music phan who loves making a difference . always be connecting , is my mantra . \#recruiting \# sourcing \# begood &          2 &    0.9598 \\ \hline
                                                        die-hard met fan since 1978 ; ya gotta believe ; \# the7linearmy . ... big time fan of snl , jimmy fallon , and seth meyers // follow me for politics @rebecca\_resists &                                                  die-hard met fan since 1978 ; ya gotta believe ; \# the7linearmy . ... big fan of snl , fallon , colbert , and seth meyers ... au mom follow me 4 politics @rebecca\_resists &          8 &    0.8295 \\ \hline
                                                                                                                             norse pagan / wiccan shaman , folk magic , unapologetic womanist , prochoice=prolife , foster dogs &                                                                                                                             norse pagan / wiccan shaman , folk magic , unapologetic womanist , prochoice=prolife , rescuedogs &          2 &    0.9215 \\ \hline
                                                                                                            live life to the fullest 🌈 cause you only get one 💯 \# e4lee 💉👼 \# e4 grandma 😇💜 05/28/2018 ♊️👶 \# mommylovesyou 👼💜 &                                                                                           live life to the fullest 🌈 cause you only get one 💯 \# e4lee 💉👼 \# e4 grandma 😇💜 \# e4 mommy 👼💪05/28/2018 ♊️👶 \#ripmommylovesyou 👼💜 &          6 &    0.8643 \\ \hline
                                                                                                                                                                                           \#praisegod \#onwisconsin \# bearfam &                                                                                                                                                                                          \# praisegod \#onwisconsin \# bearup &          3 &    0.8299 \\ \hline
                                                                                     disney theme parks fan . love the history \& ops as much as the magic . dad , it guy , music lover \& baseball fan . keep moving forward . &                                                               disney theme parks fan . love the history \& ops as much as the magic . dad , it guy , music lover , baseball fan , traveler , and frequent starbucks visitor . &          8 &    0.8156 \\ \hline
                                                                                                                      husband , proud father of two strong girls , foodie , beer lover , woke progressive and functional stoner &                                                                                                             husband , proud father of two strong girls , foodie , beer lover , woke progressive and functional stoner\#resist &          1 &    0.8860 \\ \hline
                                                                                                                                                                                     22 || matthew 's dad || 👻 : raymondcantu95 &                                                                                                                                                                                    23 || matthew 's dad || 👻 : raymondcantu95 &          1 &    0.9996 \\ \hline
                                                                      passionate visionaries dedicated to designing bespoke wardrobes that define \# thelookofyourlegacy . \#alightbeyondappearance email : contact@alba-la.com &                                                                        passionate visionaries dedicated to designing bespoke wardrobes that define \# thelookofyourlegacy . \#alightbeyondappearance email : info@alba-la.com &          1 &    0.9820 \\ \hline
                                                              credit union ceo . music is my life ! @raleigh\_keegan 's fan club leader for al . faves : @kelliepickler @saraevansmusic @meghanlinsey @lindsayell @thebandperry &                                                           credit union ceo . music is my life ! @raleighkeegan 's fan club leader for al . i ❤️@kelliepickler @saraevansmusic @meghanlinsey @lindsayell @thebandperry @halsey &          5 &    0.8283 \\ \hline
                                                                                the official twitter account for cleveland metropolitan school district news . rt ≠ endorsement . \# partoftheplan also follow @ericgordon\_ceo &                                                                                                   the official twitter account for the cleveland metropolitan school district . \# partoftheplan also follow @ericgordon\_ceo &          6 &    0.8105 \\ \hline
                                                                                                                                                              reporter at @wgrz . story ideas ? email stephanie.barnes@wgrz.com &                                                                                                                                                    daybreak reporter at @wgrz . story ideas ? email stephanie.barnes@wgrz.com &          1 &    0.8804 \\ \hline
                                                                                                                                                                                            i am the real life peter griffin :p &                                                                                                                                                                                              i am the real life peter griffin &          1 &    0.8131 \\ \hline
                                                                                             upstate ny native , now in seattle ; retired ( ex - \\$ amzn \& \\$ expe ) ; blackhawks / cowboys / indians / bullets ; conservative &                                                                                              upstate ny native , now in seattle ; retired ( ex \\$ amzn \& \\$ expe ) ; blackhawks / cowboys / indians / bullets ; conservative &          1 &    0.8903 \\ \hline
                                                            since 1983 , hundreds of accounting software implementations for small / mid market businesses . certified partners for @sageintacct \# msdynsl \# msdyngp \#unanet &                                                        since 1983 , hundreds of accounting software implementations for small / mid market businesses . certified partners for \# sageintacct \# msdynsl \# msdyngp \# unanet &          4 &    0.9691 \\ \hline
                                                      @miamihurricanes assistant director of ticket operations . new jersey born and raised . clemson ' 13 . k- state ' 15 . man imposes his own limitations , do n't set any . &                                                     @miamihurricanes associate director of ticket operations . new jersey born and raised . clemson ' 13 . k- state ' 15 . man imposes his own limitations , do n't set any . &          1 &    0.9921 \\ \hline
                                                                                                                         ιφθ spr 17 ' \# deuceclub \# tail🐎🐎 the politician k.eeping i.ndividuality d. eveloping d.reams = kidd &                                                                                                                      🏁🏁ιφθ spr 17 ' \# deuceclub \# tail🐎🐎 the politician k.eeping i.ndividuality d. eveloping d.reams = kidd &          1 &    0.8754 \\ \hline
                                                                                      professional weirdo . i watch and write movies . might even make one someday . i get very excited about things . co- host of @notnewmovie &                                                                                                professional weirdo . i like movies . might even make one someday . i get very excited about things . co- host of @notnewmovie &          3 &    0.9158 \\ \hline
                                                                                                                                                                                    ( ｡• ᵕ •｡ ) *: ･ﾟ✧ • ig : http://celeste.ly &                                                                                                                                                                 ( ｡• ᵕ •｡ ) *: ･ﾟ✧ • ig : http://celeste.ly • \\$ honeythiighs &          3 &    0.8350 \\ \hline
                                                                                                          public radio , podcasts , and media innovation . curating and sharing media since before the public internet . ♥️ = ⭐ &                                                                                                             podcasts , public radio , media innovation . curating and sharing media since before the public internet . ♥️ = ⭐ &          5 &    0.8287 \\ \hline
                                                                                                                      going to 1st sawyer concert 11 - 6 - 15 fav musician is @sawyerfrdrx scott burwell holloway http://jw.org &                                                                                                                      went to 1st sawyer concert 11 - 6 - 15 fav musician is @sawyerfrdrx scott burwell holloway http://jw.org &          1 &    0.9993 \\ \hline
                                                                                                                                                                                           the tougher it gets the cooler i get &                                                                                                                                                                                        the tougher it gets , the cooler i get &          1 &    0.9106 \\ \hline
                                                                                                                                            when you want to succeed as bad as you want to breathe , then you ’ll be successful &                                                                                                                               when you want to succeed as bad as you want to breathe , then you ’ll be successful - leo messi &          3 &    0.8340 \\ \hline
                                                                                                                                          britzi. 23. cali. christian . make up addict . singer . musician . dodgers 💙 brian💏 💍 &                                                                                                                                         britzi. 24. cali. christian . make up addict . singer . musician . dodgers 💙 brian💏 💍 &          1 &    0.9913 \\ \hline
                                                                                                                     i play games , usually at a quicker pace than casuals but slower than most speedrunners . icon by @xwemblr &                                                                                                          i play games , usually at a quicker pace than casuals but slower than most speedrunners . he / him. icon by @xwemblr &          3 &    0.9042 \\ \hline
                                                                                   daughter of glory | one of the janus girls | 3rd generation superstar | part of the \# janusdynasty - forever yours @janusathena ( rp acct ) &                                                                      daughter of glory | one of the janus girls | 3rd generation superstar | part of the \# janusdynasty - forever yours @janusathena ( rp / parody account ) &          3 &    0.8547 \\ \hline
                                                                                                                                                             eagles fan , target stl , frenchie owner and luckiest husband ever &                                                                                                                                                  eagles fan , target stl , frenchie owner and luckiest husband and daddy ever &          2 &    0.9095 \\ \hline
                                                      father , antitheist , tree hugger , humanist . guitars , martial arts , gsds and my baby girl inspire . movies , mountain biking and xbox ( lynx411 ) when time permits . &                                                         father , antitheist , tree hugger , humanist . guitars , martial arts , gsds and my baby girl inspire . movies , mountain biking / hiking \& xbox when time permits . &          5 &    0.8632 \\ \hline
                                                                                                                                                         official twitter page of the fredonia blue devils men 's soccer team . &                                                                                                                                                  official twitter page of the fredonia state blue devils men 's soccer team . &          1 &    0.9263 \\ \hline
                                                             officially shout ! from bill and ted \& army of darkness to mst3 k \& other new productions , we 're celebrating 15 + years of putting pop culture on a pedestal ! &                                                            officially shout ! from bill and ted \& army of darkness to mst3 k \& other new productions , we 're celebrating 17 + years of putting pop culture on a pedestal ! &          1 &    0.9919 \\ \hline
                                                                                                                                helping parents raise teenagers during those fast \& furious years . http://www.yourteenmag.com &                                                                                                                                  helping parents raise teenagers during those fast \& furious years . https://yourteenmag.com &          1 &    0.9560 \\ \hline
                                                                                                   backpacker turned rat packer , fashion blogger \& writer , financial analyst ... just my interpretations , of the situations &                                                            backpacker turned rat packer , fashion blogger \& writer , designer , financial analyst , ( podcast in the works ) ... just my interpretations , of the situations &          9 &    0.8540 \\ \hline
                                                                                                                                                 political news junkie . @hoyajournalism graduate student , c/o approx . 2020 . &                                                                                                                                                        political news junkie . @hoyajournalism graduate student , c/ o 2020 . &          3 &    0.8824 \\ \hline
                                                                                                       writer . social media wrangler . professional procrastinator . literally always on about \# thearchers . \# stillwithher &                                                                                 writer . social media wrangler . professional procrastinator . literally always on about \# thearchers . \# stillwithher \# saveaustinschools &          2 &    0.8822 \\ \hline
                                                                                  alexandria transit company ( dash ) - bus system for the city of alexandria comments ? contact customer service at dashbus@alexandriava.gov . &                                                                               alexandria transit company ( dash ) - bus system for the city of alexandria . comments ? contact customer service at dashbus@alexandriava.gov . &          1 &    0.8197 \\ \hline
                                                      professor of philosophy , religion , \& women 's studies ; christian feminist ; dog lover ; \& hack musician . \# blacklivesmatter [ rts not necessarily endorsements . ] &                                                      professor of philosophy , religion , \& women 's studies ; christian feminist ; dog lover ; hack musician . she / her \# blacklivesmatter [ rts are n't endorsements . ] &          6 &    0.8316 \\ \hline
                                                        \#fresnounified is the 4th largest school district in california , serving more than 74,000 students . preparing career ready graduates ! use : \# fresnounifediamready &                                                       \#fresnounified is the 3rd largest school district in california , serving more than 74,000 students . preparing career ready graduates ! use : \# fresnounifediamready &          1 &    0.9910 \\ \hline
                                             award - winning \#author \& \#healing \# medium . love \# positivity , laughing , \& \# baseball . good \# karma , high \#vibrations \& \#kindness always ! let there be \#light ! &                                             award - winning \#author \& \#healing \# medium . love \# positivity , laughing , \& \# baseball⚾️good \# karma , high \#vibrations \& \#kindness always ! let there be \#light ! &          3 &    0.8541 \\ \hline
                                                                    fashion \& beautyblogger♡lover of life , kisses \& hugs ♡ https://t.co/w9cve6kb23…📧stylebytina923@gmail.com \#fashionblogger \# thegirlgang \# blkcreatives &                                                                    fashion \& beautyblogger♡lover of life , kisses \& hugs ♡ https://t.co/w9cve6kb23…📧stylebytina923@gmail.com 👻tinytina923 \# fashionblogger \# blkcreatives &          2 &    0.8647 \\ \hline
                                                        comms director at @abettermn . michigan state alum . t 1d . categorize me , i defy every label . i have very important thoughts that need to be released . views=mine🇲🇽 &                                                          deputy director at @abettermn . michigan state alum . t 1d . categorize me , i defy every label . i have important thoughts that need to be released . views=mine🇲 🇽 &          4 &    0.9176 \\ \hline
                                                                                            indie author and amateur videographer . i love the outer banks nc , motorcycling , @victorinox @swissarmy knife and @zippo lighters &                                                                  indie author , haiku poet , amateur videographer , rum drinker . i love the outer banks nc , motorcycling , @victorinox @swissarmy knife and @zippo lighters &          7 &    0.8081 \\ \hline
                                                                                                              chief innovation officer of motivateme the movement 🌏 , warrior of god \#gatornation , \#heatnation \# jagsnation &                                                                                                            chief information officer of motivateme the movement 🌏 , warrior of god \#gatornation , \#heatnation \# jagsnation &          1 &    0.9347 \\ \hline
                                                   usnavy , korean war vet , married , 7 children - 17 grandchildren - 12 great - grandchildren - catholic - pro-life - love my dog \& cat conservative - bamafan . roll tide ! &                                                      usnavy , korean vet , married , 7 children - 17 grandchildren - 12 great - grandchildren - catholic - pro-life - love my dog \& cat conservative - bamafan . roll tide ! &          1 &    0.9669 \\ \hline
                                                                                                                                                                                 cooking , eating and drinking in minneapolis . &                                                                                                                                                                              cooking , eating , and drinking in minneapolis . &          1 &    0.9331 \\ \hline
                                                                                                                            cad manager \& controls designer , working with autocad since version 1.9 , acade user since 2009 . &                                                                                                   cad manager \& controls designer , working with autocad since version 1.9 , acade user since 2009 . | autodesk expert elite &          4 &    0.8560 \\ \hline
                                                                    freespirited barefoothippie treehugging natureloving paganphilosopher poetrywriting sciencenerd hopelessromantic . \#dailymonica http://www.dailymonica.com &                                                               freespirited barefoothippie treehugging natureloving spiritualphilosopher poetrywriting sciencenerd hopelessromantic . \#dailymonica http://www.dailymonica.com &          1 &    0.9735 \\ \hline
                                                                                             a midwest community synonymous with growth , named the 8th best place to live by money magazine . tweets by communications staff . &                                                           a smart , vibrant , and entrepreneurial midwest city synonymous with growth , named the 8th best place to live by money magazine . tweets by communications staff . &          7 &    0.8085 \\ \hline
                                              mom of 2 . \#houston \# texas \# blogger \& \#twitterparty host ! \# disney \# travel \# food \#entertainment \# tech \#reviews ! email : mariah@thesimpleparent.com \#disneysmmc &                                                          mom of 2 . \#houston \# texas \# blogger \& \#twitterparty host ! \# disney \# travel \# food \#entertainment \# tech \#reviews ! email : mariah@thesimpleparent.com &          1 &    0.9279 \\ \hline
                                                                                                                                       i enjoy wearing crocs for their style over their comfort . △⃒⃘ \#kday \# whitelabelradio &                                                                                                                                             i enjoy wearing crocs for their style over their comfort . △⃒⃘ \# whitelabelradio &          1 &    0.9183 \\ \hline
                                                                  pre-medicine senior , avid autodidact , voracious reader , aviator , multi-instrumentalist singer / songwriter , public health advocate , \& man of science . &                                                         pre-medicine senior , avid autodidact , voracious reader , aviator , multi-instrumentalist singer / songwriter , public health advocate , entj , and man of science . &          3 &    0.9323 \\ \hline
                                                             nyc / un correspondent : bbc : persian service . tweet in persian \& english . iran , us politics \& some canada . rt means i am endorsing u 4 president in 2016 . &                                                            nyc / un correspondent : bbc : persian service . tweet in persian \& english . iran , us politics \& some canada . rt means i am endorsing u 4 president in 2020 . &          1 &    0.8857 \\ \hline
                                                                                                                                                                                                       my son is my best friend &                                                                                                                                                                                               my son is my best friend ! 21 . &          3 &    0.8179 \\ \hline
                                                                             i am lucky to be the ... mom to two amazing kids , wife to one wonderful husband , and principal of southold elementary school ( @southoldelem ) . &                                                        i am lucky to be the ... mom to two amazing kids , wife to one wonderful husband , and principal of southold elementary school ( @southoldelem ) . \# momsasprincipals &          2 &    0.8503 \\ \hline
                                                  science , technology , history , cloud , iot , artificial intelligence / ml , cybersec news , 🏈 , us foreign policy , humor , dad life , evangelizing data science \& cylance &                                                                         technology , history , cloud , iot , artificial intelligence / ml , cybersec news , 🏈 , us foreign policy , humor , dad life and evangelizing cylance &          6 &    0.8408 \\ \hline
                                                           irs news and guidance for the public , the press and practitioners . irs does not collect comments or messages on this site . privacy policy : http://go.usa.gov/vgo &                                                              irs news and guidance for the public , press and practitioners . irs does n't collect comments or messages on this site . privacy policy : http://go.usa.gov/vgo &          2 &    0.9803 \\ \hline
                                                                               sexagenarian , terrestrial , epigeal , bipedal , bidimensional , illogical , seed bearing mammalian inhabitant of a world in perpetual turmoil . &                                                                             sexagenarian , terrestrial , epigeal , bipedal , tridimensional , illogical , seed bearing mammalian inhabitant of a world in perpetual turmoil . &          1 &    0.9021 \\ \hline
                                                                                                                                       ig : grinddontstop\_11 kik \& snapchat : tyler\_513 r.i.p aunt nikke ✨love you forever ✊ &                                                                                                                       ig : grinddontstop\_11 kik \& snapchat : tyler\_513 r.i.p aunt nikke ✨ you will always be in my heart ✊ &          7 &    0.8975 \\ \hline
                                                                                                                                           photographer - photos used only w/ permission \& full credit . licensing available . &                                                                                                                                  amateur photographer - photos used only w/ permission \& full credit . licensing available . &          1 &    0.9117 \\ \hline
                                                                                                                totally cliché wanderlust - siberian husky mom - aσa alum - pcos fighter - \# gopackgo - \# flythew - \#onegoal &                                                                                                     totally cliché wanderlust - siberian husky mom - aσa alum - pcos fighter - \# keto - \# gopackgo - \# flythew - \#onegoal &          3 &    0.9297 \\ \hline
                                                                                                                             gamer , occasional streamer , food \& animal enthusiast . mini muffin senpai . @ryuul i1 has my ❤️ &                                                                                                                  gamer , occasional streamer , food \& animal enthusiast . she / her. mini muffin senpai . @ryuuli1 has my ❤️ &          5 &    0.8839 \\ \hline
                                                                                         aspiring author of the ya novel the girl who wished to be skinny . writing to inspire youth to love themselves , one novel at a time . &                                                                                     aspiring author of the girl who wished to be skinny . writing to inspire youth to love themselves , one novel at a time . \# itgetsbetter &          5 &    0.8303 \\ \hline
                                                                                                            you might know me from @djangocon and @revsys , or from @djangogirls @djangogirlspdx @djangogirlsatx and @treehouse &                                                                                             you might know me from @djangocon and @revsys , or from @djangogirls @djangogirlspdx @djangogirlsatx and @treehouse . she / her . &          5 &    0.9031 \\ \hline
                                                                                                                                 beagle owner / whisperer ; lefty ; car aficionado ; blood donor ; self - proclaimed zen master &                                                                                                                        beagle owner / whisperer ; lefty ; car aficionado ; blood donor ; self - proclaimed zen master mcdxcii &          1 &    0.8448 \\ \hline
                                                             principal legal officer , codification division , un office of legal affairs . follow me for an unofficial curated list of un intl law activities . un ila liaison &                                                            principal legal officer , codification division , un office of legal affairs . follow me for an unofficial curated list of un intl law activities . ila un liaison &          2 &    0.9397 \\ \hline
                                                          6th gen texan ; family fought \& died at the alamo , kin to patrick henry , despise socialist democrats \& liberalism , \#nra \# txchl 66 yrs no threats , just facts &                                                     6th gen texan ; family fought \& died at the alamo , kin to patrick henry , despise socialist democrats \& liberalism , \#lifenra \# txltc 68 yrs no threats , just facts &          3 &    0.9220 \\ \hline
                                                                                  soccer ball at my feet and music in my ears . an american raised by brits . studying international relations at sacramento state university . &                                                                                soccer ball at my feet and music in my ears . an american raised by brits . graduated international relations at sacramento state university . &          1 &    0.9262 \\ \hline
                                                                                                                                                                                                \#gopackgo \# wahoowa \#vcurams &                                                                                                                                                                                \#gopackgo \# wahoowa \#vcurams \# fedexracing &          2 &    0.8172 \\ \hline
                                                                                                                                                       life is hard . it ’s harder if you ’re stupid . do n’t be stupid . \#ttp &                                                                                                                                    life is hard . it ’s harder if you ’re stupid . do n’t be stupid . all gas no brakes \#ttp &          4 &    0.8100 \\ \hline
                                                                                                          uww alum . @target leader . focused on the journey . social media junkie . lover of all things \#sportsbiz . \# tgbtg &                                                         uww alum . @target executive . focused on the journey . social media junkie . lover of all things \#sportsbiz . learn hurt , trust pain , embrace struggle . \# tgbtg &         10 &    0.8162 \\ \hline
                                                                                                     easy on the profanity , friend . 21 and only getting bolder . aspiring writer and transcendentalist . venture capitalist . &                                                                                            easy on the profanity , friend . 22 and only getting bolder . aspiring writer , transcendentalist , and young venture capitalist . &          5 &    0.8725 \\ \hline
                                                                                                   god * proud parent of a jr. competitive shooter and a jr. fastpitch softball pitcher * books * married life * conservative * &                                                                                                      god * proud parent of a jr. competitive shooter and a fastpitch softball pitcher * books * married life * conservative * &          1 &    0.9478 \\ \hline
                                                                                                       cartoonist . loves coffee and cheese . hates cults and street parking . lived in turkey , india , united states .✍🏼 ☕️ 🐙 &                                                                                                     cartoonist . loves coffee and cheese . hates cults and street parking . lived in turkey , india , united states . ✍🏼 ☕️ 🐙 &          2 &    0.9232 \\ \hline
                                                                                artist | photographer | strategic and visual communications | howard university ‘ 19 | whbc 96.3 hd3 | ακψ | ig : thekelliamirah \# byffrenchie &                                                                 artist | photographer | strategic and visual communications | howard university ‘ 19 | whbc 96.3 hd3 | ακψ | ig : thekelliamirah \# byffrenchie ( she / her ) &          5 &    0.9205 \\ \hline
                                                                                                                                                                                                    god |young boss nigga| 22 ' &                                                                                                                                                                                                   god |young boss nigga| 23 ’ &          2 &    0.8576 \\ \hline
                                                                                                                                                                                   22 ; wifey . cat mom . sinner saved by grace &                                                                                                                                                                                    23 ; wifey . mommy . sinner saved by grace &          3 &    0.8899 \\ \hline
                                                                                                              correspondent @datelinenbc , screen writer , mother of 5 beautiful girls \& marine corps wife canadian / american &                                                                                             correspondent @datelinenbc , screen writer , mother of 5 beautiful girls , newborn son \& marine corps wife . canadian / american &          4 &    0.8478 \\ \hline
                                                                            co-founder of @upwardsg , a public affairs firm focused on issue advocacy and brand engagement . proud husband , father and member of @wilshirebc . &                                                                                     co-founder of @upwardsg , a public affairs firm focused on issue advocacy and brand engagement . proud father and member of @wilshirebc . &          2 &    0.9528 \\ \hline
                                                                                                                                                                         dad , husband , history prof , sports fan , aft member &                                                                                                                                                                                       dad , husband , sports fan , aft member &          3 &    0.8538 \\ \hline
                                                                                           child of \#god • \# wife • \# mom • \#ceo • health \& wellness \# coach • fitness \#videos • recipes • facebook @alicecameronfitness &                                                                                    child of \#god • \#intercessor • \# mom • \#ceo • health \& wellness \# coach • fitness \#videos • recipes • facebook @alicecameronfitness &          2 &    0.9046 \\ \hline
                                                            lecturer @ohiostatecomm | michigan alu〽️| \#opened advocate \& author | 💖💜💙 | pr \& travel | @edsurge columnist | “ if you educate a woman , you educate a nation ” &                                                            lecturer @ohiostatecomm | michigan alu〽️| \#opened advocate \& author | 💖💜💙 | pr \& travel | @tedtalks speaker | “ if you educate a woman , you educate a nation ” &          2 &    0.9032 \\ \hline
                                                       ceo of fifteen years . focused on big data , iot , social , mobile , and cloud computing . additional decade in data warehousing , business intelligence , data mining . &                                                      ceo of sixteen years . focused on identity , iot , big data , social , mobile , \& cloud . additional decade in data warehousing , business intelligence , data mining . &          8 &    0.9100 \\ \hline
çrazy for rock music , \textbackslash{}m / metal ! my only ba\_be ' is 25 ! he loves music too . his gram still rocks ! since birth , dad called me bah . it stuck.\textasciitilde{}r.i.p \textasciitilde{}he played guitar ... & çrazy for rock music \textbackslash{}m / metal ! my only ba\_be ' is 26 ! he loves music too . his gram still rocks ! since birth , dad called me bah . it stuck.\textasciitilde{}r.i.p \textasciitilde{}he played guitar ... &          2 &    0.9529 \\ \hline
\bottomrule
\end{tabular}



==> chapter4-BiosModification/aaai21.tex <==
% \def\year{2021}\relax
%File: formatting-instructions-latex-2021.tex
%release 2021.2
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage{aaai21}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
%\nocopyright
%PDF Info Is REQUIRED.
% For /Author, add all authors within the parentheses, separated by commas. No accents or commands.
% For /Title, add Title in Mixed Case. No accents or commands. Retain the parentheses.
% \pdfinfo{
% /Title (The Power of Self-Description:\\ How Personal Biographies Inform and Evolve)
% /Author (Xingzhi Guo, Jason J. Jones, Steven Skiena)
% /TemplateVersion (2021.2)
% } %Leave this
% /Title ()
% Put your actual complete title (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case
% Leave the space between \Title and the beginning parenthesis alone
% /Author ()
% Put your actual complete list of authors (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case.
% Each author should be only by a comma. If the name contains accents, remove them. If there are any LaTeX commands,
% remove them.


% \renewcommand{\UrlFont}{\ttfamily\small}
% \usepackage{graphicx}
% \usepackage{booktabs}
% \usepackage{caption}
% \usepackage[normalem]{ulem}
% \usepackage{hyperref}
% \usepackage{float}
% \usepackage{subfig}
% \usepackage{makecell}
% \usepackage{arydshln}
% \usepackage{mathtools}
% \usepackage{amsmath}
% \usepackage{todonotes}
% \usepackage{array}
% \usepackage{adjustbox}
% \usepackage{comment}
% \usepackage{placeins}

% DISALLOWED PACKAGES
% \usepackage{authblk} -- This package is specifically forbidden
% \usepackage{balance} -- This package is specifically forbidden
% \usepackage{color (if used in text)
% \usepackage{CJK} -- This package is specifically forbidden
% \usepackage{float} -- This package is specifically forbidden
% \usepackage{flushend} -- This package is specifically forbidden
% \usepackage{fontenc} -- This package is specifically forbidden
% \usepackage{fullpage} -- This package is specifically forbidden
% \usepackage{geometry} -- This package is specifically forbidden
% \usepackage{grffile} -- This package is specifically forbidden
% \usepackage{hyperref} -- This package is specifically forbidden
% \usepackage{navigator} -- This package is specifically forbidden
% (or any other package that embeds links such as navigator or hyperref)
% \indentfirst} -- This package is specifically forbidden
% \layout} -- This package is specifically forbidden
% \multicol} -- This package is specifically forbidden
% \nameref} -- This package is specifically forbidden
% \usepackage{savetrees} -- This package is specifically forbidden
% \usepackage{setspace} -- This package is specifically forbidden
% \usepackage{stfloats} -- This package is specifically forbidden
% \usepackage{tabu} -- This package is specifically forbidden
% \usepackage{titlesec} -- This package is specifically forbidden
% \usepackage{tocbibind} -- This package is specifically forbidden
% \usepackage{ulem} -- This package is specifically forbidden
% \usepackage{wrapfig} -- This package is specifically forbidden
% DISALLOWED COMMANDS
% \nocopyright -- Your paper will not be published if you use this command
% \addtolength -- This command may not be used
% \balance -- This command may not be used
% \baselinestretch -- Your paper will not be published if you use this command
% \clearpage -- No page breaks of any kind may be used for the final version of your paper
% \columnsep -- This command may not be used
% \newpage -- No page breaks of any kind may be used for the final version of your paper
% \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% \pagestyle -- This command may not be used
% \tiny -- This is not an acceptable font size.
% \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

% \setcounter{secnumdepth}{2} %May be changed to 1 or 2 if section numbers are desired.

% The file aaai21.sty is the style file for AAAI Press
% proceedings, working notes, and technical reports.
%

% Title

% Your title must be in mixed case, not sentence case.
% That means all verbs (including short verbs like be, is, using,and go),
% nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% articles, conjunctions, and prepositions are lower case unless they
% directly follow a colon or long dash

% \title{ The Power of Self-Description: \\How Personal Biographies Inform and Evolve }
% \author {Anonymous authors}

% \author {
%     % Authors
%     Xingzhi Guo,\textsuperscript{\rm 1}
%     Jason J. Jones, \textsuperscript{\rm 2}
%     Steven Skiena \textsuperscript{\rm 1} \\
% }
% \affiliations {
%     % Affiliations
%     \textsuperscript{\rm 1} Department of Computer Science \\
%     \textsuperscript{\rm 2} Department of Sociology \\
%     Stony Brook University, New York, USA\\
%     emails
% }

% \todo{(10 pages for submission, including all. 12 pages after acceptance)}

% \begin{document}

% \maketitle

% \section{Abstract}
% \input{chapter4-BiosModification/chapter_abstract}
% \end{abstract}

%https://github.com/ytnvj2/DocumentEmbedding/blob/master/TFIDFwithEmbeddings.ipynb

\section{Introduction}
\label{introduction}
\input{chapter4-BiosModification/chapter_introduction}

\section{Related Work}
\label{related-work}
\input{chapter4-BiosModification/chapter_related_work}

\section{Ethical Considerations}
\label{ethics}
\input{chapter4-BiosModification/chapter_ethics}

\section{Biography Dataset}
\label{dataset}
\input{chapter4-BiosModification/chapter_dataset}


\section{The Predictive Power of Biography}
\label{single-bio}
\input{chapter4-BiosModification/Chapter_prediction_from_bio}

\section{Biography Evolution}
\label{biography-evolution}
\input{chapter4-BiosModification/chapter_dynamic_bio}

\section{Conclusions and Future Work}
\label{future-work}
\input{chapter4-BiosModification/chapter_conclusion}


% \bibliography{aaai21}
% \bibliographystyle{aaai21}
%\newpage

% \appendix
\section{Appendix}
\label{sec:appendix}
\input{chapter4-BiosModification/chapter_appendix}

% \end{document}


==> chapter4-BiosModification/chapter_abstract.tex <==
%People on social media reveal him/herself behind the screen via language traits in posts, replies ....
Profile biographies contain concise, yet rich, self-descriptions.
Analysis of self-descriptions provides powerful insights concerning how people see themselves and how they change.
In this paper, we analyze a longitudinal corpus recording the public, self-authored biographies of 51.18M Twitter users as they evolved over a six-year period.
First, we demonstrate that brief (160 characters) self-reported biographies have considerable predictive power on the task of inferring gender, ethnicity as well as personal interests. We estimate that the information in one bio is equivalent to 16, 8, and 2 personal tweets for the aforementioned tasks, respectively.
Second, from our temporal analysis, we discover that Twitter users usually make minor modifications (1$\sim$5 words at a time) in their bios, and most changes are in numbers and nouns, reflecting birthdays, anniversaries and career shifts. 
Furthermore, we conduct case studies of self-reported job titles within biographies, discovering occupational demographic bias and the directionality of career transitions. These results demonstrate that biographies are a rich source of data for quantitative social science. They allow unobtrusive observation of the intersections and transitions obtaining in online self-presentation.

%capture the complex aspect of society and encode interesting life transition patterns, which could be useful resources for future social studies.
% and also present a temporal analysis of self-descriptions and demonstrate that they encode interesting life transition patterns, including job promotion and graduation.

% We demonstrate that brief (160 characters) self-reported biographies have considerable predictive power on the task of gender (78.3\% acc.) and ethnicity (49.3\%) prediction, as well as categorizing users'  personal interests (64.9\%). 

%\todo{Marriage is mentioned here in the Abstract, but then never again in the body.  We should either delete this or include marriage analysis.}
%The profile description could help identify user's attributes and provide users' temporal changes for the future large scale social media analysis.
% 

==> chapter4-BiosModification/chapter_conclusion.tex <==
We demonstrated the predictive power of personal self-description (bio) on social media with the task of gender, ethnicity and personal interest classification. We empirically observe that the information encoded in a single bio is equivalent to approximately 16, 8 and 2 tweets for the tasks aforementioned, respectively.  
We also present dynamic bio studies with a new temporal bio dataset. To our best knowledge, this is the most comprehensive study of social media biography dynamics. We discover interesting life transition patterns (eg., graduation, job promotion.), and identify the directionality of occupation transitions. From our preliminary discoveries,  we envision new tasks such as training a job title embeddings and identifying recent occupation change from bio editing/ tweet posting, or more generally, future life events prediction.
%predict what occupation transition will happen in the future, 
% \begin{itemize}
%     \item Life event detection, identifying the recent life changes from the bio editing. e.g.: $man\rightarrow father, engaged\rightarrow married, promotion: director\rightarrow chair$, ...

%     \item Life event prediction: forecasting what will change in next 4 years ($student\rightarrow candidate, graduate\rightarrow engaged$, ...)

%     \item life trajectory clustering: looking for the common pattern of the life changes, cluster similar users together.
% \end{itemize}


==> chapter4-BiosModification/chapter_dataset.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.2\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_bio_length_cdf.pdf}
%     \caption{Bio length}
%     \label{fig:bio_len}
% \end{figure}

% data crawling techniques 
% raw data
To measure the predictive power of self-descriptions and conduct temporal analysis, we keep track of the 51.18 million English-language Twitter users' biographies and (re)tweets \footnote{We use the FastText language identification tool \cite{joulin2016fasttext, joulin2016bag} to filter out all non-English bios.} from Feb. 2015 to July 2021 using Twitter APIs, and detect 435.70 millions of biography changes. 
Figure \ref{fig:bio_len_summary} shows the bio length distribution, a similar observation (the peaks on two sides and one hump around 20) can be found in \cite{semertzidis2013people}. 
%\todo{JJJ: Did you filter on location? If not, then English-language Twitter users is a better term than American users.} 

\begin{figure}[htbp]
    \centering
    \subfloat[PDF (in character)\label{fig:bio_len_pdf}] {\includegraphics[width=0.45\textwidth]{Figures/fig_raw_all/figure_raw_bio_length_pdf.pdf}}\quad
    \subfloat[CDF (in character)\label{fig:bio_len}] {\includegraphics[width=0.44\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_bio_length_cdf.pdf}}
    \caption{The statistics of sampled bio length. Fig.\ref{fig:bio_len_pdf} shows two peaks, indicating people tend to either skip or write complete bios. Fig.\ref{fig:bio_len} shows that more than $\sim$80\% users have bios longer than 25 characters.}
    \label{fig:bio_len_summary}
\end{figure}

% job extractor: from all 
% prediction: long bio, person, ethnicity, personal interest.
% temporal: from all 

Demographics (e.g., gender and ethnicity) are important but sensitive features that help social scientist to understand the research population. To protect users' privacy, we follow the common practice conducted in \cite{mislove2011understanding,wood2020using,preoctiuc2015analysis} as discussed in Section \ref{ethics}. 
We inferred ethnicity and gender using name embeddings \footnote{We keep human-like names (including the modified names) by matching names in 2000 U.S. Census Data (92,600 first name and 151,671 last names):  \url{ https://github.com/rossgoodwin\/american-names};  Gender detector: \url{https://github.com/kensk8er/chicksexer}} \cite{sood2018predicting, ye2017nationality,ye2019secret} and aggregated; individual data was not stored. 

We found 7,529,400 unique names from 12,907,860 users (users may share names), and average up the distribution of demographic prediction per person over all his/her names as the proxy of their demographic characteristics. The overall statistics is presented in Figure \ref{fig:overall_demographics}. 

\begin{figure}[htbp]
    \centering
    % \subfloat[Gender distributions among users \label{fig:overall_gender}] {\includegraphics[width=0.2\textwidth]{Figures/overall_gender.pdf}}\hfill
    % \subfloat[Ethnicity distributions among users \label{fig:overall_ethnicity}] {\includegraphics[width=0.2\textwidth]{Figures/overall_ethnicity.pdf}}
    \subfloat[Gender ] {\includegraphics[width=0.45\textwidth]{Figures/overall_gender.pdf}}\quad
    \subfloat[Ethnicity] {\includegraphics[width=0.45\textwidth]{Figures/overall_ethnicity.pdf}}
    \caption{The overall demographics distribution among 12.91M users. }
    \label{fig:overall_demographics}
\end{figure}



\begin{comment}
    \begin{table}[htbp]
        \centering
        %\small
    \begin{tabular}{p{0.15\textwidth}p{0.06\textwidth}|p{0.15\textwidth}p{0.06\textwidth}}
    \toprule
                     Male &  Male\% &                      Female &   Male\% \\
    \midrule
        sport director & 100 &          makeup artist & 18.2 \\
        baseball coach & 98.5 &         literary agent & 30.6 \\
        football coach & 98.2 &          grade teacher & 34.2 \\
          sport editor & 94.8 &             life coach & 35.3 \\
         game designer & 92.7 &          social worker & 36.4 \\
    %     music producer & 0.91 &          public health & 0.38 \\
    %       sport writer & 0.91 &            facilitator & 0.38 \\
    % software developer & 0.90 &        health advocate & 0.41 \\
    %   basketball coach & 0.90 &     content strategist & 0.42 \\
    %         head coach & 0.90 &  social med. mgr. & 0.44 \\
    %  software engineer & 0.89 &            news anchor & 0.46 \\
    %       soccer coach & 0.87 &       freelance writer & 0.48 \\
    %           investor & 0.87 &          news producer & 0.49 \\
    %   assistant coach & 0.87 &        english teacher & 0.49 \\
    %      hockey player & 0.87 &      marketing manager & 0.50 \\
    %      web developer & 0.87 &     associate director & 0.55 \\
    %       videographer & 0.84 &          news reporter & 0.55 \\
        %       steeler & 0.80 &  inves. reporter & 0.56 \\
        % sport reporter & 0.79 &          news director & 0.56 \\
        %   sport anchor & 0.77 &     real estate broker & 0.57 \\
    \bottomrule
    \end{tabular}
        \caption{Top gender biased occupations}
        \label{tab:top_gender_occ_short}
    \end{table}
\end{comment}




\subsection{Case Study I: Occupational Identities in Biographies}
Biographies consist of rich occupational information \cite{semertzidis2013people}. To show the usefulness of our dataset, we extract\footnote{Job title extractor: \url{https://github.com/fluquid/find_job_titles}} and analyze the self-reported job titles. From all biographies in six years, we detected 25,033 unique occupational titles from 6,028,581 Twitter users  (11.78\% of 51.18M).  One user may have multiple job titles across time, reflecting promotion or career changes, which will be discussed in Section \ref{biography-evolution}.

\noindent \textbf{Are self-reported jobs generally prestigious? }
We observe that the most frequently mentioned job titles (e.g., \textit{director, president, etc}) are generally prestigious (high salary) occupations. 
To quantify our finding, we match\footnote{We use Rouge-L F1 score to softly align reported occupations to NY median income list, resulting in 21,946 job titles (out of 25,033) from 3,408,916 users associated with median income (General occupations like president or CEO are not listed, so we ignore them).} the mentioned occupations to the New York income list \footnote{New York's Occupational Employment Statistics:\url{https://catalog.data.gov/dataset/occupational-employment-statistics}} in Figure \ref{fig:match_job_salary}, and found most mentioned occupations have a higher income than the state's median salary.

 \begin{figure}[htbp]
    \centering
    %\includegraphics[width=0.35\textwidth, height=0.12\textheight]{Figures/occupation_figures/income_distrition.pdf}
    \includegraphics[width=0.6\textwidth]{Figures/income_twitter_job_overall.png}
    \caption{Income distribution of the mentioned occupations: The salaries are significantly higher than the overall median (\$43,431 USD) in New York, US. }
    \label{fig:match_job_salary}
\end{figure}


\noindent \textbf{Do self-reported jobs reflect actual occupational concentration of demographics?}
Table  \ref{tab:top_gender_occ_short} and \ref{tab:ethnicity_over_under_occ_short} shows the most gender-biased occupations and the over/under-represented occupations in each ethnicity group. We found certain ethnicity groups participate more in sports, academic, technology and art industry (Table \ref{tab:ethnicity_over_under_occ_long} in Appendix presents more samples).
In addition, we found males are closely related to sports, politics and technology, while females prevail in cosmetics, health and general education domain.
These results are demonstrative that bios capture complex aspects of society, and could be useful for quantitative social studies.

\begin{table}[htbp]
    \centering
    \caption{The top gender biased occupations.}
    \label{tab:top_gender_occ_short}

    \footnotesize
\begin{tabular}{p{0.3\textwidth}p{0.1\textwidth} | p{0.3\textwidth}p{0.1\textwidth}}
\toprule
                           Male &  Male\% &                  Female &  Male\% \\
\midrule
       asst. baseball coach &          0.98 &                   doula &          0.16 \\
       asst. football coach &          0.98 &             esthetician &          0.17 \\
              basketball coach &          0.98 &    kindergarten teacher &          0.18 \\
          offensive coordinator &          0.97 &    registered dietitian &          0.19 \\
                 baseball coach &          0.97 &           makeup artist &          0.20 \\
                baseball player &          0.96 &         early childhood &          0.20 \\
                    lead pastor &          0.95 &  independent consul. &          0.22 \\
                 football coach &          0.95 &            yoga teacher &          0.23 \\
            %  software architect &          0.95 &       virtual asst. &          0.24 \\
            %   golf professional &          0.93 &     instructional coach &          0.24 \\
            %      pitching coach &          0.93 &         yoga instructor &          0.25 \\
            %       ios developer &          0.93 &  occupational therapist &          0.25 \\
\bottomrule
\end{tabular}
\end{table}

%In next We use partial data from year 2020 for the prediction tasks, and leverage full data for the temporal exploration. 


\begin{table*}[hbtp]
\tiny
    \centering
    \caption{The examples of over/under-represented occupations in each ethnicity group. We normalize the raw count for each ethnicity and occupation group. The column \textit{Ratio} measures how many time the calculated value exceeds the expected value based on population prior. If ethnicity distribution of an occupation meets the prior distribution, the ratio value is 1.}
    \label{tab:ethnicity_over_under_occ_short}

\begin{tabular}{p{0.18\textwidth}p{0.03\textwidth}p{0.18\textwidth}p{0.03\textwidth}p{0.18\textwidth}p{0.03\textwidth}p{0.18\textwidth}p{0.03\textwidth}}
\toprule
                       White &     Ratio &                    Asian &     Ratio &                      Hispanic &     Ratio &                          African-American &     Ratio \\
\midrule
\multicolumn{8}{c}{Over-represented}\\
\midrule
              golf professional &                   2.12 &                research scholar &                   6.60 &             industrial engineer &                      3.48 &               performing artist &                  1.82 \\
                     golf coach &                   2.10 &            chartered accountant &                   5.76 &               volleyball player &                      2.30 &                    forex trader &                  1.81 \\
                 pitching coach &                   2.09 &               political analyst &                   4.08 &          industrial engineering &                      2.18 &            motivational speaker &                  1.79 \\
       asst. superintendent &                   2.07 &                   social worker &                   3.82 &                   soccer player &                      2.14 &               radio personality &                  1.75 \\
         social studies teacher &                   2.07 &            electronics engineer &                   3.49 &               medical assistant &                      1.74 &                    music artist &                  1.73 \\
\midrule
\multicolumn{8}{c}{Under-represented}\\
\midrule
               research scholar &                   0.84 &                  softball coach &                   0.17 &               golf professional &                      0.25 &                research scholar &                  0.74 \\
           chartered accountant &                   0.98 &        assistant football coach &                   0.18 &                  support worker &                      0.29 &             industrial engineer &                  0.76 \\
            industrial engineer &                   1.07 &        assistant baseball coach &                   0.18 &      asst. basketball coach &                      0.30 &              software architect &                  0.77 \\
           electronics engineer &                   1.12 &                  baseball coach &                   0.19 &          men's basketball coach &                      0.31 &             assistant professor &                  0.81 \\
              android developer &                   1.17 &               athletic director &                   0.20 &                      golf coach &                      0.33 &             postdoctoral fellow &                  0.83 \\
\bottomrule
\end{tabular}
\end{table*}


==> chapter4-BiosModification/chapter_dynamic_bio.tex <==
% Small Changes v.s. Big Changes
% anecdote of small changes
% add trump into bio?
% how many people totally revise the bio
% give some examples

% changes in bio v.s. changes in tweets
% compare the distribution of 
%f(tweets_old, bio_old), f(tweets_old, bio_new), 
%f(tweets_new, bio_old), f(tweets_new, bio_new), 
% find distribution 



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.25\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_edit_distance_hist.pdf}
%     \caption{Edit distance histogram: Small bio changes are more common than complete rewrite.}
%     \label{fig:news_lev_dist_hist}
% \end{figure}

%\todo{NOTE: It sounds like the analysis was run on the full dataset here rather than the filtered set used for demographics.  Is that correct? (Jason)}


%1,353,325
%From 1,353,325 twitter users' biography records across six years
%\footnote{6,082,705 pairs from any consecutive years}
Among 51.18M users, we randomly sample 1,353,325 users and acquire a subset of 2,597,550 changed pairs whose word edit distance is within 30. Figure \ref{fig:news_lev_dist_hist} shows the histogram of word-level Levenshtein distance. Most people update their bios by 1-5 words at a time.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_edit_distance_hist.pdf}
    \caption{Edit distance histogram: Small bio changes are more common than complete rewrite.}
    \label{fig:news_lev_dist_hist}
\end{figure}

In Section \ref{sec:special_case_d1}, we analyze the changed bio pairs where only one word has been substituted (89,838 pairs). 
In Section \ref{sec:general_analysis}, we extend the analysis to all pairs of arbitrary edit distance using BERTScore \cite{zhang2019bertscore} as the semantic similarity measure, and partition old/new pairs into buckets based on the nature of the changes.


\subsection{Word Substitution of Edit Distance 1}
\label{sec:special_case_d1}
For the bio pairs where only one word was substituted, we try to detect the reasons for editing through the following analysis:
% \begin{enumerate}
%     \item What is the POS tag of the changed word (Are they verbs? nouns? adjectives? or numbers?)
%     \item If changed words are numbers, are the they increased or decreased?
%     \item Are the changed words synonyms / hypernyms / hyponyms?
% \end{enumerate}



\noindent{\textbf{The POS tags of the changed words}}: we show the top-10 POS changes in Table \ref{table:d1_pos_tag_change}. The most popular POS of the  replaced words are Numbers, Nouns, X (not recognized, e.g.: random text or unrecognized abbreviation). Since Twitter biography usually does not strictly follow the English grammar, some POS transitions may be caused by the parser errors.

\begin{table}[hbtp]
    \centering
    \caption{The top POS changes: The top changes are number, reflecting age update on birthday or anniversary. Total number of replaced pairs is 89,838. }
    \label{table:d1_pos_tag_change}

    \small
    \begin{tabular}{p{0.4\textwidth}| >{\raggedleft\arraybackslash}p{0.15\textwidth}}
\toprule
POS change (before, after) & Count\  \\
\midrule
(NUM, NUM)     &       23,335 \\ \hline
(NOUN, NOUN)   &       15,850 \\ \hline
(X, X)         &       12,889 \\ \hline
(PROPN, PROPN) &        9,183 \\ \hline
(PUNCT, PUNCT) &        3,933 \\ \hline
(ADJ, ADJ)     &        2,443 \\ \hline
(NOUN, PROPN)  &        2,164 \\ \hline
% (PROPN, NOUN)  &        1,844 \\ \hline
% (VERB, VERB)   &        1,347 \\ \hline
% (NOUN, ADJ)    &        1,343 \\ \hline
% (ADJ, NOUN)    &        1274 \\ \hline
% (NOUN, X)      &         704 \\ \hline
% (PROPN, X)     &         612 \\ \hline
% (X, NUM)       &         565 \\ \hline
% (X, PROPN)     &         532 \\ \hline
\bottomrule
\end{tabular}
\end{table}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.2\textwidth]{Figures/twitter_bios_raw_chunk/figure_edit_hist_focus.pdf}
%     \caption{Number changes: Most of the number changes is increasing by one.}
%     \label{fig:d1_num_change}
% \end{figure}

\noindent{\textbf{Numerical Changes}}: we show examples of the numerical difference between the post-edited and the original bios in Table \ref{tab:d1_num_change_list}.
%\todo{In the Counts column, the last two rows have a value of 100 exactly.  Is that correct?} 
The number usually increases as the life events (e.g: age, anniversary) being updated.


\noindent{\textbf{Breakdown of Nouns:}} 
To better understand the reasons behind the word replacement, we organize the interpretable relations between changed nouns in Table \ref{tab:noun_changes}. 
We assign five categories of noun changes based on syntactic features (e.g.g: same lemma, )
Besides \textit{Others} group, most of them are minor changes (with single character change), reflecting job promotion  (e.g. \textit{vp} to \textit{svp}) or age updates. In addition, we observed many career transitions (e.g., \textit{manager} to \textit{director}, etc) in all categories, which will be addressed in Section \ref{occupation-analysis}.
%For the rest of the questions, we plot tree-like diagrams to answer the questions with a few examples in Figure.\ref{fig:new_d1_noun}-\ref{fig:new_d1_verb} for Nouns, Adjectives and Verbs, respectively.




\begin{table}[htbp]
    \centering
    \caption{Examples of top number changes: Most of them concern age and anniversary. }
    \label{tab:d1_num_change_list}

\hspace*{-0.00\textwidth}\begin{tabular}{p{0.06\textwidth} p{0.15\textwidth} p{0.25\textwidth} p{0.25\textwidth}}
    \toprule
     Diff. &  Counts &  Bio(Before) &  Bio(After)\\
    \midrule
       1 &   13,982 & 27 Year old & 28 Year old\\
       %2 &    3179 & 20 years of \#website building & 22 years of \#website building\\
       %3 &     550 & 22, NYC. & 25, NYC.\\
      -1 &     465 & Northwestern '19 & Northwestern '18\\
       5 &     345 & 170 yrs of service & 175 yrs of service\\
       %4 &     263 & I am 16 yr & I am 20 yr\\
      10 &     191 & 40-ish mom & 50-ish mom\\
      %-2 &     105 & VT ‘22 & VT ‘20\\
    1000 &     100 & wrote 3,000 poems & wrote 4,000 poems\\
     100 &     100 & 400 shows a year & 500 shows a year\\
    \bottomrule
    \end{tabular}
\end{table}


\begin{table*}[htbp]
    \small
    \centering
\caption{Breakdown of changed nouns. One pair may belong to more than one category}
\label{tab:noun_changes}

\hspace*{-0.04\textwidth}\begin{tabular}{ >{\raggedright\arraybackslash}p{0.15\textwidth} >{\raggedright\arraybackslash}p{0.05\textwidth} >{\raggedleft\arraybackslash}p{0.07\textwidth} >{\raggedright\arraybackslash}p{0.35\textwidth} >{\raggedright\arraybackslash}p{0.30\textwidth}}
\toprule
 Category & Total & \%  & \makecell[l]{Examples (Before, After, \#)} & Description \\
\midrule
 Share lemma & 693 & 4.54\% & \makecell[l]{(alumni, alumnus, 60); \\(dog, dogs, 31)\\} & The change noun shares the lemma. \\
\hline 
 Synonym & 669 & 4.38\% & \makecell[l]{(alumni, alum, 46);\\ (manager, director,41)} & The change noun is synonym. \\
\hline 
 Minor & 2327 & 15.89\% & \makecell[l]{(vp, svp, 20); \\(22yrs, 23yrs, 14)\\} & Only one character is changed (excluding same lemma pairs ) \\
\hline 
 Hyponymn  & 335 & 2.19\% & \makecell[l]{(student, graduate, 46);\\ (student, grad, 25)\\(student, alum, 15); \\(father, dad, 9)} & Become more specific\\
\hline 
 Hypernymn & 266 & 1.17\% & \makecell[l]{(teacher, educator, 17); \\(journalist, writer, 8) \\(actress, actor, 7);\\ (dad, father, 7)} & Become more general  \\
 \hline 
 Others  & 10898 & 71.36\% & \makecell[l]{(student, candidate, 104);\\ (sophomore, junior, 68)\\(coordinate, manager, 28)} & All other noun changes \\
 \bottomrule
 All & 15272 & 100\% & \makecell[l]{--} & All detected noun substitutions \\
 \bottomrule
\end{tabular}

\end{table*}



\begin{figure}[htbp]
    \centering
    \subfloat[BERTScore vs. Edit Distance.\label{fig:bertscore_lev_dist}] {\includegraphics[width=0.4\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_edit_bertscore_errorbar.pdf}}\quad
    %\subfloat[BERTScore v.s. Edit Distance: As the text changes more, they share less semantics.\label{fig:bertscore_lev_dist_dot}] {\includegraphics[width=0.2\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_edit_bertscore_hist}}\hfill
    \subfloat[The distribution of BERTScore\label{fig:bertscore_hist}] {\includegraphics[width=0.4\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_BERTScore_hist.pdf}}\hfill
    %\subfloat[The statistics of BERTScore: Roughly 80\% of the pairs is greater than 0; 40\% is greater than 0.5.\label{fig:bertscore_lev_dist}] {\includegraphics[width=0.2\textwidth]{Figures/twitter_bios_raw_chunk/figure_raw_feature_description_1_2_3_4_5_6_7_8_9_10_11_12_13_14_15_16_17_18_19_20_21_22_23_24_25_26_27_28_29_BERTScore_cdf.pdf}}\hfill
    \caption{Semantic similarity between changed bio pairs. Two peaks in \ref{fig:bertscore_hist} shows that the most common changes are minor updates and completely rewrite. }
    \label{fig:bertscore_stats}
\end{figure}
\subsection{For Arbitrary Edit Distance}
\label{sec:general_analysis}
Here we compare semantic difference in a pair of changed bios to distinguish whether it is a minor update or a completely rewrite. 
%Lexical overlap based metric like ROUGE\cite{lin2004rouge} or BLEU\cite{papineni2002bleu} score calculates the sentence similarity by comparing the surface text. 
BERT-based word alignment score -\textit{BERTScore} \cite{zhang2019bertscore}- presented a softer lexical alignment method using contextual word embeddings and the attention mechanism. It can capture the semantic similarity in two sentences of different structures and lexicons.
We extend the analysis to all changed pairs with $BERTScore_{F1}\in [-1,1]$ (Eq.\ref{eq:bertf1}) as the semantic similarity measure. The overall statistics of $BERTScore_{F1}$ is shown in Figure \ref{fig:bertscore_stats}.


%\begin{comment}
    \begin{equation}
\hspace{-0.00\textwidth}
\begin{aligned}
    &R = \frac{1}{|x|} \sum_{x_i \in x} {max_{\hat{x_j} \in \hat{x} } x_i \hat{x}_j  } ;
    P = \frac{1}{|\hat{x}|} \sum_{\hat{x_j} \in \hat{x}} {max_{x_i \in x } x_i \hat{x}_j  } \\
    &BERTScore_{F1} =  2\frac{P*R}{R+P},  
\end{aligned}
\label{eq:bertf1}
\end{equation}  where $x_i,\hat{x_i}$ denote $i^{th}$ token in two sentences $x,\hat{x}$.

%\end{comment}

% show similarity score calculation 

% \begin{itemize}
%     \item \textbf{Semantic Similarity}: Lexical overlap based metric like ROUGE\cite{lin2004rouge} or BLEU\cite{papineni2002bleu} score compares the surface text in two sentences, and calculates the similarity score. Recently, BERT-based word alignment score (\textit{BERTScore}\cite{zhang2019bertscore}) was presented for the same purpose but results in more soft lexical alignment with the help of the contextual word embeddings and the attention mechanism (e.g.: capture the similarity of a denotation (semantic concept) in two differently structured sentences). We use BERTScore-F1 score $\in [-1,1]$ as the semantic similarity measure. The overall statistics of BERTScore-F1 is shown in Figure.\ref{fig:bertscore_stats}.
    
%     \item \textbf{Syntactic Similarity}: The word-level edit distance can be a proxy metric of the sentence structure difference. The more words changed, the more dissimilar the sentence structure would be. A better syntactic representation metric could be found in the future \footnote{probably Tree distance}.
    
%     %\item \textbf{Sentiment Similarity}:
% \end{itemize}




%With the attention mechanism, BERTScore is quite insensitive to pure syntactic changes where the relative word order varies but semantics holds still. So we could roughly decompose the changes into the separate semantic and syntactic axis.

%In order to capture the different change categories (e.g.: large syntactic changes but small semantic changes, ...), we plot the semantic similarity (BERTScore) against word-level levenshtein distance in Figure. \ref{fig:bertscore_lev_dist} and Figure.\ref{fig:bertscore_lev_dist_dot}.



Figure \ref{fig:bertscore_lev_dist} shows the semantic similarity (BERTScore) against word-level levenshtein distance. Within our expectation, semantic similarity keeps decreasing as more edits are applied.  Figure \ref{fig:bertscore_hist} shows the distribution of BERTScore, the humps centered at 0 tells that a significant fraction of people completely rewrite their bios, while the hump at 0.8 shows another large group of people minorly edit their bios (e.g: age or occupation updates as mentioned before).


%However, in Figure.\ref{fig:bertscore_lev_dist_dot} we observed that a portion of highly edited sentences (edit distance $>10$) still retain the original semantics with BERTScore greater than 0.6.  We show some examples from A,B,C,D areas in Table.\ref{table:Text_Area_A}-\ref{table:Text_Area_D} in appendix.

%in Table.\ref{table:Text_Area_A},Table.\ref{table:Text_Area_B},Table.\ref{table:Text_Area_C},Table.\ref{table:Text_Area_D} with pre/post-edited sentences, word-level edit distance and BERTScore.


\subsection{Case Study II: Dynamics in Occupational Identity }
\label{occupation-analysis}
To better understand the changes of occupational identities in bios, we analyze how the self-reported occupations change in the bios, and detect the occupational (job) transitions as people update their bio. 

\noindent \textbf{Represent transitions as a graph}: We formulate occupational transitions as a directed weighted graph $G(V, E)$, as shown in Figure \ref{fig:job_trans_graph}, where $V$ contains all unique job titles, $E$ contains all job title transitions $e_{i,j}$ from $v_i$ to $v_j$ with an edge weight $w_{i,j}$, representing the total number of the observed transitions from i to j.

Specifically, we insert a dummy node ("none") representing no job was detected, and define a transition from the detected job title set $ s_{t-1}, s_{t} $ at time $t-1$ to $t$ as $S_{\delta(t-1,t1)} \in \{ {e_{i,j}=(v_i, v_j) | v_k \in V, |v_k|=1, i \neq j \} }$,  where $v^{t-1}_i \in s_{t-1} \setminus s_{t}$, and $v^{t}_i \in S_{t} \setminus S_{t-1}$. For example: 

$S_{t-1} \in $ \{\textit{Student, Volunteer}\} , 
$S_{t} \in $ \{\textit{Software Engineer, Volunteer}\},

$S_{\delta(t-1,t1)} \in$ \{ \textit{(Student, Software Engineer)} \}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/figure_job_transition_graph.pdf}
    \caption{Examples of job transitions in the graph. Darker edges represent more observed transitions. }
    \label{fig:job_trans_graph}
\end{figure}

The final graph has 25,033 nodes, 287,425 edges, consisting of 7 weakly-connected components. The largest component contains 25,021 nodes (99.95\% of all).
%job_one_waytransition_freq


%\begin{equation}
%    v^{t-1}_i = s_{t-1} \setminus s_{t} , v^t_j = s_{t1} \setminus s_{t-1} \\
%\end{equation}

%$S_{\delta(t-1,t1)} = S_{Job}^{t}S_{Job}^{t-1} \ \in{\{(v_i, v_j) | v_i \in V, i \neq j \}}$ and $|S_{\delta(t-1,t1)}| = 1$. 

%$S_{Job}^{t}$ and $S_{Job}^{t-1}$ (e.g., from \textit{Student} $\rightarrow$ \textit{Software Engineer}).  


%\textbf{Occupation title changes}:
%  To better understand the bio changes, we analyze how the self-reported occupations change in the bios. We extract the job titles \footnote{Job title extractor: \url{https://github.com/fluquid/find_job_titles}} from changed biography pairs, and construct a directed graph (e.g., \textit{Student} $\rightarrow$ \textit{Software Engineer}). 
% Another interesting observation is that we could sample paths from the graph as simulated path (career path). For example, we start off as a \textbf{student}, and end up as a \textbf{Associate Professor}, the sampled path (with max length 3) from the graph can be:

% \begin{itemize}
%     \item 'Student', 'Adjunct Professor', 'Associate Professor'
%     \item 'Student', 'Assistant Professor', 'Associate Professor'
%     \item 'Student', 'Director', Associate Professor'
%     %\item 'Student', 'Founder', Associate Professor'
%     %\item 'Student', 'Political Scientist', Associate Professor'
%     %\item ...
% \end{itemize}


%By extracting the largest weakly connected components from the constructed directed graph, we have final graph of 1,085 nodes (77.8\%) and 1,833 directed edges.

% Table\ref{table:job_transition_freq} shows the top transitions. Figure.\ref{figure:12_job_trans} shows an example of the transitions between 12 titles.

% \begin{figure}[htbp]
%     \centering
%     %\includegraphics[width=0.3\textwidth]{Figures/figre_twitter_bios_job_transition.png}
%     \includegraphics[width=0.4\textwidth]{Figures/twitter_bios_raw_chunk/figre_twitter_bios_job_transition.png}
%     \caption{Transition graph of 12 job titles}
%     \label{figure:12_job_trans}
% \end{figure}


% \begin{table}[htbp]
%     \centering
% \begin{tabular}{lrr}
% \toprule
%                  Title &    \# &         Salary (USD) \\
% \midrule
%               student & 2587 &       N/A \\
%               director & 2336 &   90,791 \\
%               %founder & 1277 &       N/A \\
%                  %owner & 1030 &       N/A \\
%             % co-founder &  782 &       N/A \\
%              president &  702 &       N/A \\
%             %   partner &  446 &       N/A \\
%       graphic designer &  354 &  50,665 \\
%       %managing editor &  312 &  59276.36 \\
%     %  software engineer &  287 &       N/A \\
%   %assistant professor &  271 &       N/A \\
%             %  associate &  267 &       N/A \\
%     % executive director &  262 &       N/A \\
%     %   freelance writer &  238 &       N/A \\
%     %   graduate student &  232 &       N/A \\
%         %   staff writer &  229 &       N/A \\
%         % sport reporter &  226 &       N/A \\
%         % vice president &  226 &       N/A \\
%     %      web developer &  210 &       N/A \\
%     %  creative director &  206 &       N/A \\
%         %   board member &  198 &       N/A \\
%     %   basketball coach &  193 &       N/A \\
%              scientist &  183 &  71,934 \\
%         %   videographer &  182 &       N/A \\
%         %  correspondent &  178 &       N/A \\
%         %   sport editor &  177 &  59276.36 \\
%         %  senior editor &  177 &  59276.36 \\
% %     executive producer &  176 &       N/A \\
% %  social medium manager &  174 &       N/A \\
% % communication director &  171 &       N/A \\
% %               investor &  170 &       N/A \\
% %             head coach &  167 &       N/A \\
% %     assistant director &  164 &       N/A \\
% %     software developer &  164 &       N/A \\
%      marketing manager &  162 & 152,304 \\
%             %  collector &  161 &       N/A \\
%         %   news editor &  161 &  59276.36 \\
%         %      cofounder &  158 &       N/A \\
%         %   sport writer &  155 &       N/A \\
%     %   associate editor &  153 &  59276.36 \\
%             %   counsel &  149 &       N/A \\
%     %      news reporter &  147 &       N/A \\
%     %   assistant coach &  146 &       N/A \\
%         % football coach &  145 &       N/A \\
%     %   assistant editor &  141 &  59276.36 \\
%     %  community manager &  132 &       N/A \\
%     %   public relation &  130 &  61518.18 \\
%         %         prover &  125 &       N/A \\
%         %   sport anchor &  122 &       N/A \\
%         % music producer &  118 &       N/A \\

% \bottomrule
% \end{tabular}
%     \caption{The top mentioned occupation titles are common (e.g.,\textit{student, graphic designer}) and prestigious (e.g.,\textit{director, president, etc}). \textit{N/A} indicates no salary record is matched.}
%     \label{tab:title_mention_time}
% \end{table}



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/occupation_figures/income_distrition.pdf}
%     \caption{Income distribution of the mentioned occupations: The salaries are significantly higher than the overall median (\$43,431 USD) in New York, US. }
%     \label{fig:match_job_salary}
% \end{figure}

%\ref{table:job_transition_freq}
We identify the most common title transitions (in either direction) in the section \textit{Top Mentioned Transitions} in Table \ref{table:job_transition_big}, and find that the most transitions are related to job promotion or title revision.  
We also defined the transition directionality, a fraction of directed transitions from $v_i$ to $v_j$ (e.g., owner to founder):
\begin{equation}
    dir_{i,j} =\frac{w_{i,j}}{w_{i,j} + w_{j,i}} \in [0,1],
\end{equation}

Furthermore, we sort the transitions by  $dir_{i,j}$ in the section of \textit{Highly Directed Transitions} in Table \ref{table:job_transition_big}, where we discover that the top transitions are related to job promotion and reflect a significant role change (eg., \textit{"student to nurse"} or \textit{"postdoc. to professor"}). 
However, in the section of \textit{Less Directed Transitions}, most of the job titles are interchangeable with subtle difference in specificity (\textit{scientist} to \textit{neuroscientist}) and generality.

\noindent \textbf{Community of Occupational Identities}: The job transition graph has an appealing property - clusterness, which could measure the proximity between occupational titles. For example, "rooted" from \textit{Student} in Figure \ref{fig:job_trans_graph}, roles of academia are naturally clustered on the left-hand side, while industrial roles of IT are intertwined on the right-hand part. 


Graph partition \cite{clauset2004finding} is well studied for community detection. We partition the simple job graph (unweighted, undirected) based on modularity, discovering densely intra-connected communities with varying resolution $\gamma \in \{ 1, 2, 4 ,..., 512 \}$.  As Figure \ref{fig:group_gamma} shows, a larger $\gamma$ usually leads to discover more and finer communities. Figure \ref{fig:groupsize_gamma} shows that most clusters have less than 100 nodes when\footnote{We show examples when $\gamma=8$ since it's close to the changing point in Figure \ref{fig:group_gamma}. Though there could be finer sub-groups in clusters, we left it for future work. } $\gamma=8$.

\begin{figure}[htbp]
    \centering
    \subfloat[\#Groups vs Gamma \label{fig:group_gamma}] {\includegraphics[width=0.45\textwidth]{Figures/figure_job_transition_graph_cluster_gamma.pdf}}\hfill
    \subfloat[Group nodes size ($\gamma=8$) \label{fig:groupsize_gamma}] {\includegraphics[width=0.45\textwidth]{Figures/figure_job_transition_graph_partition_size.pdf}}\hfill
    \caption{\textit{Left}: More fine-grained communities are discovered as $\gamma$ increases. \textit{Right}: The histogram of \#nodes in each job community after graph partition ($\gamma=8$). Most of the community has less than 100 job titles}
    \label{fig:job_trans_graph_community}
\end{figure}

We also present the job titles in sampled groups, from small to large clusters, in Table \ref{table:job_title_community}. 
The related job titles are correctly assigned to the same cluster\footnote{Cluster size: The number of nodes in the clusters. E.g.: There are 95 clusters of size 2 in all 350 discovered clusters.}
, some of them share straightforward text pattern (e.g., \textit{"hadoop developer"} and \textit{"hadoop architect"}), while others are inherently related without significant text overlap (e.g., \textit{"highway maintenance worker"} and \textit{"bridge inspector"}). Those detected transitions and clusters can provide more context to better understand personal social dynamics.



\begin{table}[hb]
    \centering
    \small
    \caption{The detected occupation transition pairs: generally the transition reflects promotion, graduation or just rephrasing. The dummy node is ignored. }
    \label{table:job_transition_big}
\begin{tabular}{p{0.3\textwidth}p{0.3\textwidth}p{0.1\textwidth} p{0.1\textwidth}}
\toprule
                 Title A &                 Title B  &  \#  & $dir_{A,B}$\\
\midrule
\multicolumn{4}{c}{Top Mentioned Transitions}\\
\midrule
    %   founder &     co-founder &        10149 &         0.46 \\
    co-founder &        founder &        10149 &         0.54 \\
           ceo &        founder &         8577 &         0.57 \\
%       founder &            ceo &         8577 &         0.43 \\
    %   founder &          owner &         7384 &         0.41 \\
        owner &        founder &         7384 &         0.59 \\
        %   ceo &          owner &         5917 &         0.47 \\
        owner &            ceo &         5917 &         0.53 \\
 founder \& ceo &        founder &         3290 &         0.51 \\
%       founder &  founder \& ceo &         3290 &         0.49 \\
      director &        founder &         2987 &         0.57 \\
%       founder &       director &         2987 &         0.43 \\
vice president &             vp &         2734 &         0.66 \\
%            vp & vice president &         2734 &         0.34 \\
vice president &      president &         2545 &         0.76 \\
\midrule
\multicolumn{4}{c}{Highly Directed Transitions}\\
\midrule
           student nurse &         staff nurse &          109 &         0.99 \\
                %  student &      medical intern &          196 &         0.99 \\
         nursing student &    registered nurse &          217 &         0.98 \\
     assistant professor & associate professor &         2154 &         0.97 \\
     postdoctoral fellow & assistant professor &          136 &         0.96 \\
         account manager &    account director &          163 &         0.96 \\
  Sr. account manager &    account director &          105 &         0.96 \\
     editorial assistant &    assistant editor &          163 &         0.94 \\
    %  instructional coach & assistant principal &          154 &         0.94 \\
    %       student nurse &    registered nurse &          122 &         0.93 \\
%      marketing assistant & marketing exec. &          106 &         0.93 \\
%                  student &       private pilot &          145 &         0.93 \\
%         associate editor &       senior editor &          174 &         0.92 \\
%         assistant editor &    associate editor &          264 &         0.91 \\
% Sr. account exec. &     account manager &          102 &         0.91 \\
\midrule
\multicolumn{4}{c}{Less Directed Transitions}\\
\midrule
                    director &            business director &          142 &         0.50 \\
        %   business director &                     director &          142 &         0.50 \\
                   scientist &               neuroscientist &          126 &         0.50 \\
            %   neuroscientist &                    scientist &          126 &         0.50 \\
            %  assistant coach &   asst. basketball coach &          110 &         0.50 \\
            % graphic designer &                 video editor &          110 &         0.50 \\
                % video editor &             graphic designer &          110 &         0.50 \\
%   asst. basketball coach &              assistant coach &          110 &         0.50 \\
                         cto &                        owner &          110 &         0.50 \\
%                       owner &                          cto &          110 &         0.50 \\
          software developer &                ios developer &          102 &         0.50 \\
%               ios developer &           software developer &          102 &         0.50 \\
            % digital marketer & digital marketing spec. &          102 &         0.50 \\
% digital marketing spec. &             digital marketer &          102 &         0.50 \\
\bottomrule
\end{tabular}
\end{table}
%Table \ref{table:job_transition_full} in Appendix presents more samples. 

%The histogram of \#nodes in each community is shown Figure . Many of 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/figure_job_transition_graph_partition_size.pdf}
%     \caption{The histogram of \#nodes in each job community after graph partition. Most of the community has less than 10 job titles.}
%     \label{fig:job_trans_graph_community}
% \end{figure}

\begin{table}[htbp]
    \centering
    \small
    \caption{Each cluster (row) contains various highly-related job titles (manually rendered in colors) . }
    \label{table:job_title_community}

\begin{tabular}{p{1.0\textwidth}}
\toprule
 \centering\arraybackslash \textbf{Sampled Titles in Job Clusters} (350 discovered clusters, $\gamma=8$) \\ \hline
\midrule
 \centering\arraybackslash Cluster size : 2 (95/350) \\ 
\midrule
\textcolor{red}{health information director, health information technician} \\ \hline
% \textcolor{red}{certified registered locksmith, certified master locksmith} \\ \hline
\textcolor{red}{consumer lending manager, secondary market manager} \\ \hline
\textcolor{red}{loader operator, front end loader operator} \\ \hline
\midrule
 \centering\arraybackslash Cluster size: 3 - 30 (101/350)\\ 
\midrule
\textcolor{red}{regional sales coordinator, district sales coordinator, special projects coordinator },
\textcolor{blue}{highway maintenance worker, bridge inspector, traffic worker, toll collector, highway inspector}
\\ \hline
\textcolor{red}{privacy director, privacy analyst algorithm developer}, 
\textcolor{blue}{hadoop developer, hadoop architect, linux architect, windows server administrator, web systems developer, mainframe systems administrator}
\\ \hline
% \textcolor{red}{university administrator, university president, graduate school dean, director of campus recreation},
% \textcolor{blue}{senior strategy manager, program analyst, business system consultant, senior program analyst }
% \\ \hline

\textcolor{red}{occupational safety specialist, safety and health manager, safety trainer},
\textcolor{blue}{family worker, community board member, community engagement coordinator},
\textcolor{purple}{professor of early childhood education, peer educator, speech language pathologist assistant},
% \textcolor{pink}{asp developer, digital product specialist, tool builder, code official, electrician}
\\ \hline
\midrule
 \centering\arraybackslash Cluster size: 31 - 60 (71/350)\\ 
\midrule
\textcolor{red}{clinical assistant, clinic assistant, clinical associate, psychiatric assistant}
\textcolor{blue}{communication instructor, language specialist, public speaking teacher}
\textcolor{purple}{software development leader, information director}
\\ \hline

\textcolor{red}{building consultant,  building surveyor},
\textcolor{blue}{topographical surveyor, survey analyst, survey manager, survey director}
\textcolor{purple}{project management manager, senior project manager, e-business project manager}
\\ 
\hline

% \textcolor{red}{vice president of advertising, channel director, vice president of news, associate publisher}
% \textcolor{blue}{director of reimbursement, group managing director, business director}
% \\ \hline
\textcolor{red}{customer logistics manager, import manager, export sales manager, export specialist, poultry buyer,}
\textcolor{blue}{dairy nutritionist, dairy consultant }
\\ \hline

\bottomrule
\end{tabular}
\end{table}



% the min-cut, job community. What's the fraction of people move between communities.
% the most in-degree job title
% the most out-degree job title


%Although the current detected transitions are limited due to the performance of job title extractor, these



% Names represent a person as his/her most common identity. The changes in name over time reflect many social aspects. We observed that ...

% who changed last name.



==> chapter4-BiosModification/chapter_ethics.tex <==
% current 
Although Twitter data is public and often falls under public data exemptions in IRB consideration, sensitive information such as users' gender, ethnicity, health, political affiliation or beliefs should be used with caution.  
Inference on the individual level is a restricted use cases per the Twitter Developer Agreement, however: \footnote{ More about restricted uses of the Twitter APIs: \url{https://developer.twitter.com/en/developer-terms/more-on-restricted-use-cases}}
\begin{quote}
    Aggregate analysis of Twitter content that does not store any personal data (for example, user IDs, usernames, and other identifiers) is permitted, ...
\end{quote}
All of our results are at aggregate level, so that no individual identifier or original content can be traced back or reconstructed from our results. 
All the possibly identifiable examples shown in our results were artificially modified to enforce privacy protection.
We only share data regarding population-level analysis, not any analysis of individual users that may be abused.  The IRB of our institution has affirmed that use of public information does not constitute human subjects research, in accordance with regulations from the US Department of Health and Human Services.
%\todo{Do we need add IRB process we have gone through?}
%Our agreement restricts these tools to population-level analyses3 and not the analysis of individual users. We exclude certain applications, such as targeting of individuals based on race or ethnicity. Any future research that makes demographically-contextualized conclusions from classifier predictions must explicitly consider ethical trade-offs specific to its application.








==> chapter4-BiosModification/chapter_introduction.tex <==
% social media analysis needs user profile.
The concise personal biography is a feature of many social media platforms and provides an outlet for users to report their current self-identity.  On Twitter, the biography is part of every user's public profile, and research has explored the various and changing aspects of identity users choose to mention \cite{semertzidis2013people, rogers2021using, guo2024evolution}. 
% bio represent user states 
% add more bio related... More clean, more accurate, less noisy
Although users differ in the extent of what they disclose about themselves, many social media biographies express relational identity (\textit{e.g. father/mother of, alumni of}), demographics, occupations and political polarity. 
For example, the biography:
\begin{quote}
    29. cameraman. black man. Films. "We are guardians of the image \& that's how I see our role as DP's"
    %- Geoff Boyle \#ReleasetheSnyderCut }
\end{quote}
contains information about age (\textit{29-year old}), occupation (\textit{cameraman}), ethnicity (\textit{black}), gender (\textit{man}) and interests (\textit{films}). 
Other biographies are more lyrical and less explicit, but still revealing with respect to personality or life attitudes, e.g.:
\begin{quote}
    happiness can be found even in the darkest times if one only remembers to turn on the lights.
\end{quote}

% how NLP people leverage bio...
%People on social media reveal themselves behind the screen via the language they emit.  
The language within social media streams is frequently used to make inferences about users.  For instance, NLP analysis of social media posts to assess psychological state \cite{ schwartz2013personality}, gender \cite{burger2011discriminating}, and user sentiment \cite{neri2012sentiment} are well-studied problems. 
%The resulted text may perverse information about users' gender, personal interests and political stance over different period of time. 
%But this data is not generally available due to privacy settings, whereas user profiles that include self-description are often relatively open.
But some inferred information is hiding in plain sight - it is explicitly mentioned in public biographies.
%
%In order to better understand the user behavior, 
%NLP techniques for user profiling \cite{ikeda2013twitter, rangel2017overview, lynn2019tweet} traditionally aggregate text from hundreds of the user's tweets as a personal document for user modeling, sometimes with demographics and self-description. 

%\todo{NOTE: I am not sure what the previous sentence adds.  Is it redundant? (Jason)} 
%(biography)
%
%As almost every social media platform gives space for personal bio to introduce him/herself, only a few study has discussed how biography alone is useful for user profiling\cite{priante2016whoami}. 

In this paper, we investigate how self-descriptions provide user information and how self-descriptions evolve over time.
Prior works \cite{conover2011predicting, lynn2019tweet, sap2014developing} generally leverage
tweets together with bios as a supplementary feature for better user profiling accuracy.
Here we argue that these short self-descriptions provide more concise predictive power than tweets, and focus on quantifying how many tweets is equivalent to one bio in term of predictive power. 
%Here we argue that these short self-descriptions provide concise information with the predictive power of many tweets on the task of gender, ethnicity and user's personal interest classification. 
Additionally, we explore the dynamic nature of self-identity.  Bio text, serving as a proxy for self-identity, allows analysis of changing self-conception over the lifecourse. For example: the self-identity may change from \textit{student} to \textit{engineer} on graduation.  We analyze bio modifications with the detailed breakdown of change categories. 
Finally, we present a large-scale analysis of self-reported occupations among Twitter users, together with a dynamic analysis of job title transitions.

%Finally, (?)we present a datasets containing million-scale twitter user across five years for future social media temporal analysis.

The primary contributions of this paper include:
\begin{itemize}
    \item {\em Temporal Self-Description Data Set} -- We have assembled a longitudinal corpus of self-reported biographies as they evolve annually over the period 2015-2021, with 50.18 million American users whose biographies changed at least once over this period.
    With this rich dataset, we present a case study of occupational identity among Twitter users, identifying the most gender/race-biased occupations.
    %\todo{NOTE: It is not necessarily true that every user history contains at least one change.  We should check the data if we want to make that claim.  It is true that all of the users tweeted at least once each year, which provides us annual snapshots of their bio in every year. (Jason)} 
    Currently we share the full occupational graph and embeddings of bios (from 1.35M users across six years) rather than raw text due to privacy concerns.  Our dataset provides a unique resource for studying changes in self-identity, and will be made available on publication. 
    %\todo{JJJ: We should not share any dataset with user IDs in it. I don't think we should promise a dataset at all.} \todo{Twitter TOS: can only share 1,500,000 Tweet IDs within 30 days }
    
    \item {\em The Power of Self-Description} -- We demonstrate that brief (160 character) self-reported biographies have considerable predictive power on the task of gender (78.0\%) and ethnicity (49.3\%) prediction, as well as categorizing users’ personal interests (64.9\%). We estimate that one bio is worth approximately 16 tweets when predicting gender and 8 tweets when predicting ethnicity.
    %\todo{We need a better description of the final results.}
    %
    \item {\em The Evolution of Identity} --
    We present a temporal analysis explaining how and why self-descriptions change, distinguishing life events (e.g. job promotion, graduation, etc) and quantitative changes from minor changes and complete rewrites. From the case study of transitions of occupation identity, we discover the inherent directionality on certain job transitions (e.g., from \textit{assistant professor} to \textit{associate professor}). %error corrections .. job title transition records over six years and

%\todo{need a punchline based on results.}
\end{itemize}
% demonstrate the overlooked power of biography in large scale analysis
% discover dynamic biography changes

This paper is organized as follows.  Section \ref{related-work} describes previous work in analysis of self-identity, particularly for social media.
Section \ref{dataset} describes our Twitter biography data set, design choices and a case study of occupations among Twitter users.
Section \ref{single-bio} presents our results for user classification based on analysis of single biographies.
We study the changes in user biographies over time in Section \ref{biography-evolution}.
Finally we present our conclusions and future work in Section \ref{future-work}.

==> chapter4-BiosModification/chapter_related_work.tex <==

% Self-identity detection from essay, psychology 
Social media users often present their self-identities in bios. \citet{semertzidis2013people} investigated how people express themselves in twitter profile bios and found users frequently describe interests (e.g., music, food) and profession (e.g., marketing, writer).  Further, they categorized the bio content into six groups together with average word fraction as follows: Occupation (7.5\%), Interests/Preferences/Hobbies(4.6\%),  Personal Info (2.6\%), Social Nets/Internet (2.3\%), Community (1.5\%) and General. 
Another related research line is social media user profiling, which aims at predicting user's attributes from text on social media. \citet{bhattacharya2014inferring} tried to infer users' interests from the topical labels of who they subscribe to (e.g., following Barack Obama may give the labels \textit{Politics}). They also use interests explicitly declared in the bios as ground-truth to evaluate their inferred results. \citet{burger2011discriminating,preoctiuc2018user, lynn2017human, lynn2019tweet,lynn2020hierarchical} tried to predict user's demographics or personalities from user's document (tweets) and non-document attributes (location, profile photo), leveraging language features (n-gram, POS tags, word embeddings) and various classifiers like SVM, LSTMs or BERT-based deep models. They use personal bios as a supplement feature for accuracy improvement, while we incline to believe a single bio tells more than a single tweet, and try to quantify how many tweets can achieve the same predictive power of one bio on various tasks. 

Users differ in which aspects of their self they emphasize in their bios, however, many indicate their occupational identity. \citet{preoctiuc2015analysis,pan2019twitter} extracted Twitter users' occupations from bios, tweets and social network structure, and framed the task of occupational class prediction. \citet{vainio2017highly} did a detailed word co-occurrence analysis of bios from academic Twitter users, finding that users tweeting academic articles emphasize occupational expertise rather than personal interests. In our case studies, we investigate the demographic concentrations in 26.92K unique jobs from 6.02 million users who mentioned occupations in their bios. 

Personal biographies are dynamic, reflecting the life or mind changes in a person over time. \citet{shima2017users} analyzed the timing and reasons for Twitter bio changes and found that English users most frequently make changes on their birthday. \cite{rogers2021using} discovered that Americans defined themselves more politically by integrating more political words in their Twitter bios over recent years. In our temporal analysis, we examine the reasons behind modifications and discover interesting bio transitions for graduation, anniversaries and career shifts. To our best knowledge, this is also the largest resource for studies of occupation dynamics.




%Similar to the tweets, it can reveal information about the user interests and identity, and it is interesting to understand it further.

%\textbf{User Document Embedding} reveals ....
%\cite{volkova2015inferring} infer user latent representation.

% 1. Tweets, gender revealing lexicon 
% 2. Predicting the Political Alignment of Twitter Users
% 3. Document embeddings: For fair comparison, we try different methods to extract embedding for tweets. 1. TF-IDF 2. Weighted Embeddings 3.
% 4. BERT Tweets is the first public large-scale language model pre-trained for English Tweets. BERTweet is trained based on the RoBERTa pre-training procedure
%Tweet Classification without the Tweet: An Empirical Examination of User versus Document Attributes


%\textbf{When people change}: \cite{shima2017users} when people change
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8258287&tag=1

%\textbf{Name} tells a lot about person's gender and ethnicity. Name embeddings \cite{nameprism} (e.g. NamePrism) effectively perverse the personal traits by modeling homophily in names and relations on social networks. 
% Gender, Ethnicity from name


% BERT Score

% Dynamic Analysis of twitter bio transition (jason's paper)

% https://raphaelb.org/posts/freezing-bert/

